Higher dimensional Jordan curves

We address the question of what is the correct higher dimensional analogue of Jordan curves from the point of view of quantitative rectifiability. More precisely, we show that 'topologically stable' sets can be used as covering objects in Analyst's Travelling Salesman Theorem-type theorems: if $E$ is lower $d$-regular (in a certain suitable sense), then we show that there exists a topologically stable surface $\Gamma$ so that $E \subset \Gamma$ and $$ \mathrm{diam}(E)^d + \beta^d(E) \approx \mathcal{H}^d(\Gamma), $$ where $\beta^d$ is a term quantifying the curvature of $E$. A corollary of the main result of this paper and a construction by Hyde, is a higher dimensional analogue of Peter Jones TST, valid for \textit{any} subset of Euclidean space.

==> 01-2-Intro.tex <==
\section{Introduction}
This paper was motivated by three questions, which we introduce below.

\subsection{Higher dimensional `curves' for the analyst's traveling salesman theorem}
Let $E$ be a subset of $\R^n$ and suppose that $E$ has Hausdorff dimension larger than one. The first motivating question is the following: what simple geometric or topological condition should we impose on $E$ so that $E$ `is like a Jordan curve'? Let us explain what is the context of this question (and thus what this question really mean).

We begin by recalling the Travelling Salesman Problem (TSP). Given a finite set of points, it asks to find the shortest path that goes through each one of them. Motivated by problems in harmonic measure, Peter Jones posed the following variant of the TSP: given a general set $E$ in the plane, can we find the length of the shortest curve (up to a constant multiple) passing through it? This makes sense whenever we can actually cover $E$ with a rectifiable curve (that is, a curve of finite length). Hence a restatement of Jones' question is: give a characterisation of subsets $E$ of rectifiable curves in the plane. This problem came to be known as the Analyst's TSP. Note that if we know from the start that $E$ is contained in a line $L$, then we are immediately done: the shortest curve $\Gamma$ will be the appropriate line segment, and it's length will be exactly equal to the diameter of $E$. However, if $E$ presents some curvature, then the length of the covering curve will necessarily increase; to quantify this increment, one needs to quantify how much $E$ deviates from being a line, that is, we need a measurement of its curvature.
%\begin{figure}[hbt!]\label{f:curvature}
 %\centering
 %\includegraphics[scale=0.5]{tst-curvature.png}
 %\caption{The increment of the curve in the second figure will be comparable to $h^2/\diam(E)$.}
%\end{figure}
Hence it makes sense to measure how much $E$ deviates from lines at all points and scales: so Jones defined what came to be known as the Jones $\beta$ numbers; for a dyadic square $Q$, set 
\begin{align} \label{e:beta-inf}
    \beta_{E, \infty}(Q):= \inf_{L \text{ a line}} \sup_{z \in E \cap 3Q} \frac{\dist(z, L)}{\ell(Q)},
\end{align}
where $\ell(Q)$ denotes the side length of $Q$, the infimum is taken over all (affine) lines in $\Complex$ and $\dist(z, L)$ is the usual Hausdorff distance given by $\inf_{l \in L}|z-l|$. Note that this quantity measure exactly what was mentioned above, i.e. how much $E$ deviates from a line ($Q$ determines the scale and location at which we make the measurement). Jones in \cite{jones90} then proved that $E$ is a subset of a curve $\Gamma$ and $\Gamma$ is rectifiable if and only if 
\begin{align}\label{e:jones-function}
   \beta^2_\infty(E):=  \sum_{Q \text{ dyadic }} \beta_{E, \infty}^2(Q) \ell(Q)\, < \, \infty,
\end{align}
where the sum is taken over all dyadic cubes. Moreover, this statement is quantitative, that is, let $\Gamma_0$ denotes the shortest curve containing $E$; there exists a universal constant $C_0$ such that for all $E$ we have
\begin{align}\label{e:TST}
    C_0^{-1} \leq \frac{ \text{diameter}(E)+ \beta_\infty^2(E)}{\mathcal{H}^1(\Gamma_0)} \leq C_0.
\end{align}
Here $\mathcal{H}^1$ denotes the $1$-dimensional Hausdorff measure, and so $\mathcal{H}^1(\Gamma_0)$ is the length of $\Gamma_0$. See also \cite{jones91} for a more thorough introduction to the Analyst's TSP and some indication of why it is relevant in the theory of harmonic measure. The same characterisation was later generalised to curves in arbitrary euclidean space by K. Okikiolu in \cite{oki92} and to curves in Hilbert space by 
R. Schul in \cite{schul07}. 
The question on whether a similar theorem could be proved for higher dimensional sets was completely open until very recently. In \cite{azzam-schul18} J. Azzam and R. Schul proved a version of Jones' theorem for sets of dimension larger than one in Euclidean space. It is in this context that the initial question makes perhaps a little more sense. If in the plane we characterise subsets of rectifiable curves, subsets of what type of geometric object do we want to consider now? Or, in other words, what sort of sets in $\R^n$ should play the role that curves played in the plane? One could legitimately think about, for example, topological spheres; see Figure \ref{f:octopus} for why this would not be a good candidate. 
\begin{figure}[hbt!]\label{f:octopus}
 \centering
 \includegraphics{octopus.png}
 \caption{Given the $2$-dimensional  8-corner Cantor set in $\R^3$, one can construct a $2$-dimensional surface with finite measure, so that the closure of this surface will contain the Cantor set and will be homeomorphic to the $2$-sphere.}
\end{figure}

Azzam and Schul decided for a slightly different approach to that of Jones. They chose to focus on obtaining a quantitative result of type \eqref{e:TST} for a set $E$ lying in $\R^n$ by imposing a certain size condition directly on $E$. This size condition is the following:
we say that a set $E \subset \R^n$ is \textit{lower content} $d$-\textit{regular} with constant $c_0 <1$ if 
\begin{align} \label{e:LCR}
    \hd_\infty(B(x,r) \cap E) \geq c_0 r^d
\end{align}
for all $(x, r) \in E \times (0, \diam(E))$; here $\hdc$ is the Hausdorff content, see P. Mattila's book \cite{mattila}, Chapter 4, for definitions and properties. Note in particular that a curve is lower content $1$-regular; hence $E$ is, in this respect, `similar' to a curve (it is at the same time true that there are no assumption on $E$ in Jones' theorem: some questions remain unanswered). 
Azzam and Schul also had to think of a new variant of the $\beta$ numbers; indeed, in any situation where one is dealing with sets of dimension larger than one, the $\beta$ coefficients as defined in \eqref{e:beta-inf} become rather useless: in his PhD thesis, X. Fang constructed a Lipschitz graph $K$ with $\beta_{\infty}^2(K)=\infty$, see \cite{fang}. Shortly after, David and Semmes in \cite{david-semmes91} introduced an averaged (or `$L^p$') version of these coefficients, defined as
\begin{align}\label{e:beta-p}
    \beta_{E,p}^d(x,r):= \inf_{L} \ps{\frac{1}{r^d} \int_{B(x,r)} \ps{\frac{\dist(y, L)}{r}}^p \, d \hd|_{E}(y) }^{\frac{1}{p}},
\end{align}
where the infimum is taken over all affine $d$-dimensional planes in $\R^n$.
David and Semmes were dealing with Ahlfors $d$-regular sets, i.e. sets satisfying 
\begin{align}\label{e:ADR}
    C^{-1} r^d \leq \hd(E \cap B(x,r)) \leq C r^d \mbox{ for } x \in E \mbox{ and } 0 \leq r \leq \diam(E). 
\end{align}
Clearly with this assumption on $E$, \eqref{e:beta-p} makes sense.
Note however that the assumption on lower content $d$-regularity does not exclude that $E$ may be of dimension larger that $d$. If that was the case, $\hd|_{E}$ would not be a locally finite measure, and thus \eqref{e:beta-p} would not have any meaning at all. This is the reason why Azzam and Schul introduce the following variant of the $L^p$-type $\beta$ coefficients. They put
\begin{align} \label{e:beta-p-cont}
\beta_E^{d,p} (x,r) = \inf_L \left( \frac{1}{r^d} \int_0^1 \hdc (\{y \in B(x,r)\cap E \,|\, \dist(y,L)> tr\}) t^{p-1} \, dt \right)^{\frac{1}{p}},
\end{align}
where the infimum is taken over all affine $d$-planes $L$ in $\R^n$. The integral on the right hand side of \eqref{e:beta-p-cont} is a Choquet integral. 
With these Jones coefficients and with the assumption of lower content regularity (i.e. \eqref{e:LCR}) on $E$, Azzam and Schul proved an estimate of the type \eqref{e:TST}, with a difference, however: rather than having only the $d$-dimensional Hausdorff measure of $E$ at the denominator (as in \eqref{e:TST}), they had $\hd(E)$ \textit{plus} a term, $\textrm{BWGL}(E)$, which quantify the amount of `holes' present in $E$; that is, they proved an estimate like 
\begin{align} \label{e:TSTdTheta}
     C^{-1} \leq \frac{ \text{diameter}(E)^d+ \beta_E^{d,p}(E)^2}{\mathcal{H}^d(E) + \textrm{BWGL}(E)} \leq C,
\end{align}
where $\beta^{d,p}(E)^2$ is defined as in \eqref{e:jones-function}, but using the content $\beta$ numbers. We will define precisely $\text{BWGL}(E)$ later; for the moment, let us say that its presence is somewhat natural: in Jones's theorem, we had at the numerator the length of the minimal curve covering $E$; now, a curve has no holes. However, $E$ may very well be quite broken (even while being lower content regular). Thus, if we imagine our set $E$ being covered by `a higher dimensional curve' $\Gamma$, we would have $\hd(\Gamma) \sim \hd(E) + \text{BWGL}(E)$, where $\text{BWGL}(E) \sim \hd( \Gamma \setminus E)$.  

%\begin{figure}[hbt!]\label{f:holes}
% \centering
% \includegraphics{holes.png}
% \caption{The measure of the holes is measured by BWGL(E).}
%\end{figure}

We will state all this more precisely later; but for now, let us go back to our initial question: recall that we asked for conditions on $E$ so that $E$ `looks like a curve'. In view of the correspondance between \eqref{e:TST} and \eqref{e:TSTdTheta}, we can make our question more precise: what conditions on a set $E$ guarantee an estimate of the type \eqref{e:TST} \textit{without} the term $\text{BWGL}(E)$? The main result of this paper is an answer to this question. We put on $E$ a topological condition (TC) which guarantees precisely this: an estimate of the type \eqref{e:TST}, or, in other words, \eqref{e:TSTdTheta} without the $\text{BWGL}(E)$ term. This condition in introduced below, see Subsection \ref{ss:TC}. 

\subsection{Topological non-degeneracy of sets and geometric complexity} \label{ss:Topo-ND}
In \cite{semmes}, Semmes stated the following guiding principle to understand the relation between the topology of some set, and its `mass' distribution. 

\textit{`Suitable topological condition on a space in combination with upper bounds on the mass often implies serious restriction on the geometric complexity of the space.'}

In the monograph \cite{david-semmes00}, David and Semmes made this principle into the following theorem | to avoid introducing extra notation, we state it in a somewhat imprecise manner. 
\begin{theorem}[\cite{david-semmes00}, Theorem 0.10] \label{t:DS-quasi}
Let $E$ be a compact subset of $\R^n$ and let $A$ be a union of dyadic cubes in $\R^n$ containing $E$. If $\hd(E)< + \infty$ and if, given a constant $\theta>0$,  $\hd(f(E)) > \theta$ for every continuous mapping $f: E \to A$ which is homotopic to the identity through mappings from $E$ to $A$, then the following holds. For any$ \tau>0$, there is a compact set $Z\subset \R^n$ such that
\begin{itemize}
    \item $Z$ is Ahlfors regular, uniformly rectifiable and contains big pieces of Lipschitz graphs;
    \item $\hd(Z)> \theta'$, where $\theta'$ depends on $n$ and $A$, but not on $\tau$.
    \item $\hd(Z \setminus E) \leq \tau \hd(E)$.
\end{itemize}
\end{theorem}

Here, we will give a result which is similar to Theorem \ref{t:DS-quasi}; however the initial assumptions are somewhat different: in particular, we will be looking at deformations which are only Lipschitz.

\subsection{Uniformly non-flat sets and their Hausdorff dimension}
The third question which motivates this paper stems from a result of Bishop and Jones, \cite{bishop-jones97}. Here, they proved that if a connected compact subset of the plane is uniformly non-flat, then its dimension is strictly larger than one. For definitions and the precise statement of this, see Section \ref{s:non-flat}. Moreover, their theorem showed explicitly how the non-flatness of the set affects the lower bound on its dimension. In \cite{david04}, David gave a corresponding result for higher dimensional sets, which however is qualitative in nature, i.e. it doesn't present how the non-flatness of $E$ affect the dimensionality of $E$. Here, as a further application of our main result, we give an exact analogue of Bishop and Jones's result. 


\subsection{The topological condition on $E$} \label{ss:TC}
Let us now define precisely the topological condition mentioned above. 
Let $E$ be a subset of $\R^n$. 
\begin{definition}[Allowed Lipschitz deformations with parameter $\alpha_0$] Fix a constant $0< \alpha_0 <1$.
Consider a one parameter family of Lipschitz maps $\{\varphi_t\}$, $0 \leq t \leq 1$ and defined on $\R^n$. We say that $\{\vp_t\}_{0\leq t \leq 1}$ is an \textit{allowed Lipschitz deformation} with parameter $\alpha_0$, or an $\alpha_0$-ALD, if it satisfies the following four conditions: 
\begin{align}
    & \vp_t(\bar B(x,r) )\subset \bar B(x,r) \mbox{ for each } t \in [0,1]; \label{e:vp1}\\
    & \mbox{ for each } y \in \R^n, t \mapsto \vp_t(y) \mbox{ is a continuous function on } [0,1]; \label{e:vp2}\\
    & \vp_0 (y) = y \mbox{ and } \vp_{t}(y) = y \mbox{ for } t \in [0,1] \mbox{ whenever }  y \in \R^n \setminus B(x,r); \label{e:vp3}\\
    & \dist(\vp_t(y), E) \leq \alpha_0 r \mbox{ for } t \in [0,1] \mbox{ and } y \in E \cap B(x,r), \mbox{ where } 0<\alpha_0<1. \label{e:vp4}
\end{align}
\end{definition}

The topological condition that we impose on $E$ is the following. 
\begin{definition}[Topological Condition] \label{d:TC}
Fix four parameters:
\begin{align}
    & r_0, \mbox{ the scale parameter}, \label{e:r_0}\\
    & \alpha_0, \mbox{ the distance parameter}, \label{e:alpha_0}\\
    & \delta_0, \mbox{ the lower regularity parameter, } \label{e:delta_0} \\
    & \eta_0, \mbox{ the boundary parameter.} \label{e:eta_0}
\end{align}
We say that a subset $E \subset \R^n$ satisfies the topological condition with parameters $r_0, \alpha_0, \delta_0$ and $\eta_0$, or the $(r_0, \alpha_0, \delta_0, \eta_0)$-(TC), or just (TC), if for all $\alpha_0$-ALD $\{\vp_t\}$, and for all $x_0 \in E$ and $0< r < r_0$, we have
  \begin{align}\label{e:TC} \tag{TC}
    \hd\ps{B(x, (1-\eta_0)r) \cap \vp_1(E) } \geq \delta_0 r^d. 
\end{align}
\end{definition}
 We may refer to a set $E$ satisfying the topological condition above as a \textit{topologically stable} $d$-surface, or, for short, TS $d$-surface.
\begin{remark}
Let us remark once more that this condition is not new. As stated it was introduced by G. David in \cite{david04}, where he proved that a set $E$ endowed with such a condition and so that its $\beta$ numbers are large, then it must have dimension strictly larger than $d$. 
\end{remark}

%\begin{figure}[hbt!]\label{f:TC}
 %\centering
 %\includegraphics[scale=0.7]{TC.png}
 %\caption{On the left, a ball satisfying the topological condition. On the right, one failing it.}
%\end{figure}

\subsection{Statement of the main result and some consequences}

Let $\dD(E)=\dD$ denote the family of Christ-David cubes relative to $E$ (see Theorem \ref{t:Christ} for definitions). 
Our main result in the following.
\begin{theorem}\label{t:main}
	Let $E \subset \R^n$ and let $0<\eta_0, \delta_0, \alpha_0<1$ and $r_0>0$. If $E$ satisfies the $(r_0, \alpha_0, \delta_0, \eta_0)$-\eqref{e:TC}, then, for any $R \in \dD$ such that
	\begin{align} \label{e:locality}
	    \ell(R) < r_0,
	\end{align}
	and any $C_0 \geq 1$,
	\begin{align}\label{e:main}
	   \diam(R)^d+ \sum_{\substack{Q \in \dD \\ Q \subset R  }}\beta_E^{p,d} (C_0 Q)^2 \ell(Q)^d  \leq C  \hd(R),
	\end{align}
	where the constant $C$ depends on $\alpha_0$, $\delta_0$ and $\eta_0$.
\end{theorem}
\begin{remark}
The assumption \eqref{e:locality} is a natural one and cannot be avoided. Assuming the topological condition from a certain scale, i.e. from $r_0$, means that at larger scale there could be holes. This would make the term $\text{BWGL}(E)$ come back.
\end{remark}

Theorem \ref{t:main} together with the main result from \cite{azzam-schul18}, see Theorem \ref{t:AS} below, gives the following corollary. 

\begin{corollary}\label{cor:main}
Let $E \subset \R^n$. If there are parameters $\eta_0, \delta_0, \alpha_0$ and $r_0$ so that $E$ satisfies the topological condition \eqref{e:TC}, 
then with $1\leq p<p(d)$, where
\begin{equation}
\label{e:pd}
p(d):= \left\{ \begin{array}{cl} \frac{2d}{d-2} & \mbox{if } d>2 \\
 \infty & \mbox{if } d\leq 2\end{array}\right. ,
 \end{equation}
 and $C_0$ sufficiently large (depending only on $n$), we have
\begin{align} \label{e:TST1}
    \diam(R)^d + \sum_{\substack{Q \in \dD \\ Q \subset R}}\beta_E^{p,d}(C_0 Q)^2 \ell(Q)^d \sim \hd(R),
\end{align}
where $R \in \dD$ is so that $\ell(R)<r_0$, and
where the constant behind the symbol $\sim$ depends on $C_0, n, p$, the parameters coming from the topological condition, and the parameters behind the constants appearing in Theorem \ref{t:AS} (see below). 
\end{corollary}



In some cases, the estimate \eqref{e:TST1} was already known: for $\ve$-Reifenberg flat (see Definition \ref{d:reif}), for example. Another known case was for $n=d-1$ and $E$ is satisfying Condition B (for definitions, see \cite{azzam-schul18} and the references therein). We will see below that both Reifenberg flatness and Condition B imply the topological condition that we introduced above. 

%Another consequence of Theorem \ref{t:main} and of the techniques coming from \cite{azzam-villa19}, is the following. See Section \ref{s:Sigma}.
%\begin{theorem}\label{t:SigmaIntro}
%Let $E \subset\R^n$ be a lower content $d$-regular set with constant $c_0$ and let $Q_0 \in \dD$. Given two parameters $0< \ve, \kappa< 1$, there exists a set $\Sigma= \Sigma(\ve, \kappa, Q_0)$ such that
%\begin{enumerate}
 %   \item $Q_0 \subset \Sigma$.
 %   \item $\Sigma$ is a TC surface with constant $r_0= \diam(Q_0)/2$, $0<\eta_0<1/100$, and $\alpha_0$ and $\delta_0$ sufficiently small with respect to $\kappa$ and $\ve$. 
 %   \item We have the estimate
 %   \begin{align*}
 %       \beta(Q_0)^2 + \diam(Q_0)^d \sim_{c_0, n, d, \ve} \hd(\Sigma). 
  %  \end{align*}
%\end{enumerate}
%Moreover, if $\hd(\Sigma)< +\infty$, then $E$ is $d$-rectifiable. 
%\end{theorem}
%That is, given any lower content regular set, we can cover it with a topologically stable $d$-surface. If this surface has finite measure, the set will be rectifiable. This is basically what happens in the original analyst's TST by Peter Jones. 

Concerning the type of questions raised in Subsection \ref{ss:Topo-ND}, we have the following corollary, which pops out immediately from Theorem \ref{t:main} and the theory of uniformly rectifiable sets (see \cite{david-semmes93}).

\begin{theorem}
Let $E$ be a topologically stable $d$-surface. If $E$ is upper Ahlfors $d$-regular, then $E$ is uniformly rectifiable. 
\end{theorem}

Finally, concerning the Hausdorff dimension of uniformly non-flat sets (see Section \ref{s:non-flat} for precise definitions), we have the following theorem. 

\begin{theorem} \label{t:high-dim-intro}
Let $E \subset \R^n$ be a topologically stable $d$-surface. Let $R \in \dD$ be such that, for any $Q \in \dD(R)$, we have that
\begin{align}
    \beta_E^{p,d}(C_0 Q)^2 > \beta_0 >0.
\end{align}
Then
\begin{align}
    \dim(R) > d + c \beta_0^2. 
\end{align}
\end{theorem}
See Section \ref{s:non-flat} for a sketch of proof of this. 

\subsection{Acknowledgement}
I would like to thank Jonas Azzam, my supervisor, for suggesting the problem, for his help and support. I would also like to thank PCMI/IAS and the organisers of the graduate school of 2018 on Harmonic Analysis: it was here that I learned many tools used in this paper, as explained by Guy David (whom I also thank for the clear explanations). 

==> 01-2-IntroNew.tex <==
\section{Introduction}
\subsection{The Analyst's Travelling Salesman Problem}
We begin by recalling the Travelling Salesman Problem (TSP)\footnote{The reader familiar with the area is encouraged to skip the first few paragraphs of the introduction: this story has become part of the narrative identity of a mathematical community and as such has been repeated many times over.}. Given a finite set of points, the TSP asks to find the shortest path that goes through each one of them. In the late eighties, Jones posed the following variant of the TSP: given a general set $E$ in the plane, can we find the length of the shortest curve  passing through it? This makes sense whenever we can actually cover $E$ with a \textit{rectifiable} curve (i.e. a curve of finite length). Hence a restatement of Jones' question is: give a characterisation of subsets $E$ of rectifiable curves in the plane. This problem came to be known as the Analyst's TSP. Note that if we know from the start that $E$ is contained in a line $L$, then we are immediately done: the shortest curve $\Gamma$ will be the appropriate line segment, and it's length will be exactly equal to the diameter of $E$. However, if $E$ presents some curvature, then the length of the covering curve will necessarily increase; to quantify this increment, one needs to quantify how much $E$ deviates from being a line, that is, we need a measurement of its curvature.
%\begin{figure}[hbt!]\label{f:curvature}
 %\centering
 %\includegraphics[scale=0.5]{tst-curvature.png}
 %\caption{The increment of the curve in the second figure will be comparable to $h^2/\diam(E)$.}
%\end{figure}
Hence it makes sense to measure how much $E$ deviates from lines at all points and scales: so Jones defined what came to be known as the Jones $\beta$ numbers; for a dyadic square $I$, set 
\begin{align} \label{e:beta-inf}
    \beta_{E, \infty}(I):= \inf_{L \text{ a line}} \sup_{z \in E \cap 3I} \frac{\dist(z, L)}{\ell(I)},
\end{align}
where $\ell(I)$ denotes the side length of $I$, the infimum is taken over all (affine) lines in $\Complex$ and $\dist(z, L)$ is the usual Hausdorff distance given by $\inf_{l \in L}|z-l|$. Note that this quantity measures exactly what was mentioned above, i.e. how much $E$ deviates from a line ($I$ determines the scale and location at which we make the measurement). Jones in \cite{jones90} then proved the following. 

\begin{theorem}\label{t:Jones-TST}
$E$ is a subset of a curve $\Gamma$ and $\Gamma$ is rectifiable if and only if 
\begin{align}\label{e:jones-function}
   \textup{\jones}_\infty(E)^2:=  \sum_{I \text{ dyadic }} \beta_{E, \infty}^2(I) \ell(I)\, < \, \infty,
\end{align}
where the sum is taken over all dyadic cubes. Moreover let $\Gamma_0$ denote the shortest curve containing $E$. There exists a universal constant $C_0$ such that\footnote{By $a \approx_{C} b$ we mean that $C^{-1} \leq \frac{a}{b} \leq C$. See also Section \ref{s:prel}.} for all $E$ we have
\begin{align}\label{e:TST}
     \textup{diameter}(E)+ \textup{\jones}_\infty^2(E) \approx_{C_0} \mathcal{H}^1(\Gamma_0).
\end{align}
\end{theorem}
\begin{figure}
\begin{minipage}[l]{0.45\linewidth}
        \centering
        \includegraphics[scale=0.3]{flat.png}
\end{minipage}
\begin{minipage}[l]{0.45\linewidth}
        \centering
        \includegraphics[scale=0.3]{curvature.png}
\end{minipage}
\caption{\small{The heuristics behind Jones' TST (Theorem \ref{t:Jones-TST}): in the first case (left), the set $E$ is flat, hence the length of the shortest curve is equal to the diameter of $E$. In the second case (right), the length of the covering curve $\Gamma$ needs to account for the curvature, and thus we have $\mathrm{length}(\Gamma) \approx h^2 + \mathrm{diameter}(E)$. }} 
\end{figure}   
\michele{Add some details to the caption.}
\noindent
Jones' result turned out to be incredibly influential. His work \cite{jones90}, together with that of David and Semmes (\cite{david-semmes91}, \cite{david-semmes93}), initiated a whole new area of research, referred to sometimes as \textit{quantitative rectifiability}. Techniques developed in this context helped solving long standing problems in complex and harmonic analysis (\cite{david98}, \cite{tolsa03}, \cite{ntv}) (some of which motivated Jones\footnote{See also \cite{jones1991} for an overview of the problems and questions behind Jones' theorem.}, David and Semmes to start with), and found applications beyond these fields: harmonic measure (\cite{azzam2016rectifiability}), boundary value problems (\cite{ahmmt}, \cite{orponen2020sub}), rectifiability (\cite{azzam2015characterization}), free boundary problems (\cite{focardi2018measure}).
\\
\\
\noindent
To complete the Analyst's TSP story, the same characterisation was later generalised to curves in arbitrary euclidean space by K. Okikiolu in \cite{oki92} and to curves in Hilbert space by 
R. Schul in \cite{schul2007}. \michele{Add more reference on works in metric space, etc etc - Badger, Schul, Li, GC David etc.}
The question on whether a similar theorem could be proved for `higher dimensional'\footnote{We will shortly make precise obscure expressions such as `higher dimensional'.} sets was completely open until very recently. There are two reasons for this.

\begin{itemize}[leftmargin=.5cm]
    \item The first issue, which is also the most fundamental one, is the following: if in the plane we characterise subsets of rectifiable curves, subsets of what type of geometric object do we want to consider now? Or, in other words, what sort of `$d$-dimensional' sets\footnote{Throughout the paper, $d \in \N$ will denote the dimension of the set $E$ which is being studied, while $n$ will denote the dimension of the Euclidean ambient space. Clearly we will always have $d<n$.} in $\R^n$ should play the role that curves played in the plane? One could legitimately think about, for example, topological spheres; see Figure \ref{f:octopus} for why this would not be a good candidate.
    \item The second issue is  technical in nature: in any situation where one is dealing with sets of dimension larger than one, Jones' $\beta_{E, \infty}$ coefficients (as in \eqref{e:beta-inf}) become rather useless: in his PhD thesis, X. Fang constructed a codimension one Lipschitz graph $G$ in $\R^3$ with $\beta_{\infty}^2(G)=\infty$, see \cite{fang1990} or Example 1.16 in \cite{azzam2018analyst}.
    A further version of Jones' coefficients was introduced by David and Semmes in \cite{david-semmes91}. We will define them later on; for the moment it will suffice to say this: David and Semmes' coefficients make sense for `higher dimensional' sets, as long as such sets are \textit{a priori} \textit{Ahlfors regular}. Ahlfors regularity is a size condition\footnote{It is not a regularity condition: the four corner Cantor set is Ahlfors $1$-regular and purely unrectifiable.}  which impose a certain relationship between the diameter of a portion of the set and its mass.
 However, Jones's theorem does not assume this; indeed, $E$ need not to have \textit{a priori} finite $d$-dimensional measure, let alone be Ahlfors regular. Thus, a new type of coefficient measuring flatness is needed. 

\end{itemize}
\begin{figure}[hbt!]\label{f:octopus}
 \centering
 \includegraphics[scale=0.5]{octopus.png}
 \caption{Given the $2$-dimensional  8-corner Cantor set in $\R^3$, one can construct a $2$-dimensional surface with finite measure, so that the closure of this surface will contain the Cantor set and will be homeomorphic to the $2$-sphere.}
\end{figure}

\subsection{An Analyst's TST for higher dimensional sets}
Notwithstanding these difficulties, a few of years ago, J. Azzam and R. Schul proved in \cite{azzam2018analyst} a version of Jones' theorem for sets of dimension larger than one in Euclidean space. 
\begin{itemize}[leftmargin=0.5cm]
    \item To deal with the first difficulty,
Azzam and Schul decided to focus on obtaining a quantitative result of type \eqref{e:TST} directly for a set $E$ lying in $\R^n$, without trying to find a `covering object'. To be able to make some progress, they imposed on $E$ a size condition called \textit{lower content regularity}. 
\begin{definition}
We say that a set $E \subset \R^n$ is \textit{lower content} $d$-\textit{regular} with constant $\cc_1 \leq1$, or lower content $(d, \cc_1)$-regular, if 
\begin{align} \label{e:LCR}
    \hd_\infty(B(x,r) \cap E) \geq \cc_1 r^d
\end{align}
for all $(x, r) \in E \times (0, \diam(E))$.
\end{definition}
The symbol $\hdc$ represents Hausdorff content, which will be defined in \eqref{e:hdc} below.
Roughly speaking, lower content regularity prevents a set $E$ to concentrate around objects of dimension smaller than $d$. It is a natural assumption to impose on $E$, and it appears, in a form or another, in works on harmonic measure for example (see \cite{akman2019absolute}, \cite{akman2019rectifiability}, \cite{azzam2019harmonic})\footnote{Lack of lower bounds on the mass of a set (whether measured with a measure or a content) is highly problematic, as it becomes hard to say anything about its geometry.}. 

\item To deal with the second difficulty, Azzam and Schul introduced the following variant of the $L^p$-type $\beta$ coefficients\footnote{The $L^p$ $\beta$-coefficients are the ones that David and Semmes came up with.}. For a set\footnote{This set will usually be a ball or a cube. In this case $\diam(B)$ will be substituted by the radius of the ball or the side length of the cube.} $B \subset \R^n$
\begin{align} \label{e:beta-p-cont}
\beta_E^{d,p} (B) := \inf_L \left( \frac{1}{r^d} \int_0^1 \hdc (\{y \in B\cap E \,|\, \dist(y,L)> t \, \diam(B)\}) t^{p-1} \, dt \right)^{\frac{1}{p}},
\end{align}
where the infimum is taken over all affine $d$-planes $L$ in $\R^n$. The integral on the right hand side of \eqref{e:beta-p-cont} is a Choquet integral. Azzam and Schul chose $\hdc$ to define their $\beta$ coefficients because $\hdc$ \textit{does not blowup}. Indeed, for any set $E$, we always have that $\hdc(E)\lesssim \diam(E)^d$, even when the Hausdorff dimension of $E$ is larger than $d$. We refer the reader to Examples 1.14, 1.15 and 1.16 in \cite{azzam2018analyst} for some examples which motivate their choice of $\beta$-coefficients.
\end{itemize}

 \noindent
With these two adjustments, Azzam and Schul prove an estimate of the type \eqref{e:TST}, \textit{with a difference}: rather than having only the $d$-dimensional Hausdorff measure of $E$ in the RHS (as in \eqref{e:TST}), they have $\hd(E)$ \textit{plus} a term, $\textrm{BWGL}(E)$, which quantifies the amount of `holes' present in $E$; that is, they proved an estimate like\footnote{We will recall their theorem precisely in Section \ref{s:actual-theorems}, see Theorem \ref{t:AS-real}.}
\begin{align} \label{e:TSTdTheta}
    \text{diameter}(E)^d+ \jones_{p,d}(E)^2 \approx \mathcal{H}^d(E) + \textrm{BWGL}(E)
\end{align}
where $\beta_{d,p}(E)^2$ is defined as in \eqref{e:jones-function}, but using the content $\beta$ numbers \eqref{e:beta-p-cont}. The presence of $\rm BWGL(E)$ is natural: in Jones's theorem the RHS only contains the length of the covering curve; now, a curve has no holes\footnote{Sherlock, personal communication.}. However, $E$ may very well be quite broken (even while being lower content regular). Thus, if we imagine our set $E$ being covered by `a higher dimensional curve' $\Gamma$, we would have $\hd(\Gamma) \approx \hd(E) + \text{BWGL}(E)$, where $\text{BWGL}(E) \approx \hd( \Gamma \setminus E)$ (see Figure \ref{f:bwgl}).

\begin{figure}[h]
\begin{minipage}[l]{0.45\linewidth}
        \centering
        \includegraphics[scale=0.4]{bewgl2.png}
\end{minipage}
\begin{minipage}[l]{0.45\linewidth}
\centering 
\includegraphics[scale=0.4]{bwgl.png}
\end{minipage}
\caption{A covering curve picks up the holes in the set (left). In the absence of a `higher dimensional curve', the term BWGL accounts for the holes (right).} \label{f:bwgl}
\end{figure}


\subsection{Main result: topologically stable surfaces as higher dimensional curves}
The story of the Analyst's TST has left an issue open: what should a `higher diemensional' curve be? Another way to formulate this question is: what conditions on  $E$ guarantee an estimate of the type \eqref{e:TSTdTheta} \textit{without} the term $\mathrm{BWGL}(E)$, that is, for what higher dimensional sets does Jones' TST hold in its original form \eqref{e:TST}?
\textit{The main result of this paper is an answer to this question}.
We show that if we put on $E$ a certain \textit{topological condition} (firstly appeared in \cite{david2004hausdorff}), then $E$ will satisfy an estimate precisely of the type \eqref{e:TST}. We will define this condition further on, see Section \ref{s:actual-theorems}. For the moment, call a $d$-dimensional set $E$ satisfying such a condition a \textit{stable $d$-surface}. We state our main theorem in a somewhat sloppy manner, postponing the more precise (but less readable) statement to Section \ref{s:actual-theorems}. 
\begin{MainOne}[Sloppy version]\label{t:main-sloppy}
Let $E \subset \R^n$ be $d$-stable.
Then we have\footnote{Recall once more that $\jones_{p,d}(E)^2:= \sum_{Q \in \dD(E)} \beta_E^{p,d}(Q)^2 \ell(Q)^d$, where $\beta_E^{p,d}$ is this case is the content $\beta$-coefficients as defined in \eqref{e:beta-p-cont}, while $\dD$ is the family of \textit{Christ-David} cubes which we introduce in Section \ref{s:prel}, Theorem \ref{t:Christ}. For the moment, the reader may imagine them simply as dyadic cubes. The choice of $p$ in the theorem will be made explicit in Section \ref{s:actual-theorems}.}
\begin{align*} %\label{e:TST1}
    {\rm diameter}(E)^d + \textup{\jones}_{p,d}(E)^2  \approx \hd(E),
\end{align*}
where the constant behind the symbol $\approx$ depends on $d, n$, the parameters coming from the topological condition, and the parameters behind the constants appearing in the main result of \cite{azzam2018analyst}, Theorem \ref{t:AS}. 
\end{MainOne}

\noindent A first application of Theorem \ref{t:main-sloppy} is an Analyst's TST for sets which are lower content regular  and with stable $d$-surfaces as curves. In words, we show
that \textit{for any set $E$ which is lower content regular, there exists a stable $d$-surface $\Sigma$ such that}
\begin{align*}
    \diam(E)^d + \textup{\jones}_{p,d}(E)^2 \approx \hd(\Sigma).
\end{align*}
The reader will find the precise statement in Theorem \ref{c:TST-lcr-stable}, Section \ref{s:actual-theorems}. Now,
in the very recent work \cite{hyde2020TST}, Hyde shows that for a general set $E$ one can always construct a lower content $d$-regular set $F$ containing it and such that\footnote{The $\beta$ coefficients used by Hyde are not precisely the same as the ones introduced by Azzam and Schul, i.e. as in \eqref{e:beta-p-cont}. See Section \ref{s:actual-theorems} for more details and a precise statement of \eqref{e:H-sloppy} (which can be found as Theorems \ref{t:TST-H1} and \ref{t:TST-H2}).} 
\begin{align}\label{e:H-sloppy}
    \jones_{p,d}(E)^2 \approx \jones_{p,d}(F)^2.
\end{align}
Hence, the series of papers \cite{azzam2018analyst}, \cite{azzam2019quantitative}, \cite{hyde2020TST} together with the present article give \textit{a full Analyst's Travelling Salesman Theorem for sets of any dimension in Euclidean space}. See also Corollary 1.14 in \cite{hyde2020TST}.
\begin{CorMainOne}[Sloppy version]\label{c:TST-end-sloppy}
Let $E$ be a set in $\R^n$. Then there exists a stable $d$-surface $\Sigma$ such that
\begin{align*}
    {\rm diameter}(E)^d + \textup{\jones}_{p,d}(E)^2 \approx \hd(\Sigma). 
\end{align*}
\end{CorMainOne}

\subsection{Relevance and more applications}
The reader may understandably wonder whether Theorem \ref{t:main-sloppy} is at all interesting or useful. 
I think it is interesting in the sense that, behind it, there is a natural question: what should a `higher dimensional curve' be? Although as stated such a question is imprecise and open to very many answer, if we add `\textit{from the point of view of the Analyst's TST}', it takes a decidedly more precise meaning. 
\noindent
As for the usefulness of the result, we provide a few more applications (with the hope that more will come). Once again, we state the results rather imprecisely, to convey some ideas. We postpone details and precision to Section \ref{s:applications}. 

\begin{itemize}[leftmargin=0.5cm]
    \item We will call a set uniformly non $d$-flat if the $d$-dimensional $\beta$-coefficients (as defined in \eqref{e:beta-p-cont}) are large at all scales\footnote{We postopone the precise definition to Section \ref{s:actual-theorems}.}. As first application of our main result, we show that \textit{if $E$ is $d$-stable and uniformly non $d$-flat, then it must have Hausdorff dimension larger than $d$.} This result was proven in by David in \cite{david2004hausdorff}. We provide a quantitative strengthening of David's result which gives a precise dependence between  $\beta$-coefficients and dimension. See Theorem \ref{t:non-flat} below. 
    \item In \cite{semmes1995finding}, Semmes stated the following guiding principle to understand the relation between the topology of some set, and its `mass' distribution: \textit{`Suitable topological conditions on a space in combination with upper bounds on the mass often implies serious restrictions on the geometric complexity of the space.'} 
As a second application, we give a result that makes this principle precise. This result is similar to the main result in \cite{david2000uniform}. \michele{Add precise references to theorems}
\end{itemize}


\subsection{Sketch of the proof}
We give a brief idea of the proof. As a first step, we apply a construction from \cite{azzam2019quantitative} which gives a \textit{coronisation} of a $d$-stable surface $E$ by Ahlfors $d$-regular sets. One should imagine such a construction as a dyadic approximation of $E$ at certain scales. Next, following ideas coming from the proofs in \cite{david2004hausdorff}, we show that, first, the topological condition transfers from $E$ to the approximating sets. The fundamental observation is this: because the approximating sets are Ahlforse regular and satisfy the topological condition, they turn out to have large intersection with \textit{quasiminimal sets}. By the main result in \cite{david2000uniform}, sets of this type are (locally) \textit{uniformly rectifiable}. This will give certain estimates on the $\beta$-coefficients, which will then be transferred back to $E$, to obtain one direction of Theorem \ref{t:main-sloppy}. The other direction follows from the main result in \cite{azzam2018analyst}.


\subsection{Structure of the paper}
In Section \ref{s:prel} we gather some notation which will be used throughout the paper. In Section \ref{s:actual-theorems} we state precisely the main result (Theorem \ref{t:main-prec}) and the definition of the topological condition (Definition \ref{d:TC}). We give the precise statements of the two applications mentioned  above (Theorem \ref{t:main-app1} and Theorem \ref{t:main-app2}) together with the relevant definitions in Section \ref{s:applications}.  In
Section \ref{s:remarks} we give some remarks on the choice of the topological condition and show that some perhaps better known types of surfaces falls withing this category. In Section \ref{s:reductions} we start the proof in earnest with some preliminary reductions and by applying the corona construction of \cite{azzam2019quantitative}. In Section \ref{s:STC} we define a variant of the topological condition and show that it is `inherited' from $E$ by the approximating sets coming from \cite{azzam2019quantitative}. Section \ref{s:FFproj} introduces a fundamental tool, Federer-Fleming projections. In Section \ref{s:TC-STC} we show that the above mentioned `inheritance' effectively happens. Section \ref{s:E-rho-STC} presents a further family of approximating sets. 
In Section \ref{s:STC-UR} we show that the approximating sets lie close to a uniformly rectifiable set. Section \ref{s:beta} concludes the proof via some $\beta$-coefficients estimates. In Section \ref{s:app1} we give a proof of the first application mentioned above, while Section \ref{s:app2} contains the second one. 

\subsection{Acknowledgments}

==> 03-2-remarks.tex <==
\section{Some remarks on the topological condition \eqref{e:TC}}
We want to motivate a little the topological condition \eqref{e:TC}. 
\begin{definition}
A Semmes $d$-surface is a set $E\subseteq \R^{n}$ so that the following holds. For all points $x_0 \in E$ and $r>0$, we can find an affine subspace $W$ of dimension $n-d$ and a sphere $S$ of dimension $n-d-1$ which is contained in $W$ and so that
\begin{align}
    & S \subset B(x_0, r) \tag{GSS 1} \label{eq:GSS1} \\
    & \dist(S, E) \geq C_0^{-1} r \tag{GSS 2} \label{eq:GSS2}\\
    & S \mbox{ links } E. \tag{GSS 3} \label{eq:GSS3}
\end{align}
Let us explain what we mean by $S$ links $E$; we say that $S$ and $E$ are linked if it is not possible to find an homotopy $F(t, x)$ defined and continuous for all $(t, x) \in [0,1] \times \R^n$ such that

\end{definition}



==> 04-2-constructionER.tex <==
\section{First reductions and the construction of approximating skeleta}\label{s:first-red}
Sections \ref{s:first-red} to \ref{s:beta-end} will be devoted to the proof of Theorem \ref{t:topo-main}. We will first prove the following inequality (the converse being an immediate consequence of Azzam and Schul's result Theorem \ref{t:AS-real}, as we will see in Section \ref{s:beta-end}).   
\begin{proposition} \label{p:main-one-dir}
Assume that $1 \leq d < n$. Let $E \subset \R^n$ be a stable $d$-surface with parameters $r_0, \alpha_0, \delta_0$ and $\eta_0$ and let $\dD$ be its Christ-David cubes. Let $Q_0 \in \dD$ be an arbitrary cube satisfying $\ell(Q_0)< r_0$ and let $\aA>1$. Take $1 \leq p < p(d)$ with 
\begin{align*}
p(d):= \left\{ \begin{array}{cl} \frac{2d}{d-2} & \mbox{if } d>2 \\
 \infty & \mbox{if } d\leq 2\end{array}\right. 
 \end{align*}
 Then it holds that
\begin{align}\label{e:main}
    {\rm diameter}(Q_0)^d + {\rm BETA }(Q_0) \lesssim \hd(Q_0),
\end{align}
where 
\begin{align}\label{e:BETA}
    {\rm BETA}(Q_0) = {\rm BETA}_{E, \aA, p, d} (Q_0): = \sum_{Q \in \dD(Q_0)} \beta_E^{d,p} (\aA B_Q)^2 \ell(Q)^d,
\end{align}
and where the constant behind the symbol $\lesssim$ depends on the parameters of $\eqref{e:TC}$ \textup{(}$\alpha_0, \delta_0, r_0, \eta_0$\textup{)}, on $\aA$, on $p$, and on the dimensional parameters \textup{(}$d$, $n$\textup{)}.
\end{proposition}

\subsection{First reductions}
Let us get started with the proof of Theorem \ref{t:main}. Fix a top cube $R \in \dD$. First, we see that if $\hd(R) = \infty$, then there is nothing to prove. Thus, we may assume that
\begin{align} \label{e:hdE}
    \hd(R)< + \infty
\end{align}

We will use the following lemma. 
\begin{lemma}[\cite{azzam-schul18} Lemma 2.13] \label{lemma:betaincreasep}
Let $1 \leq p < \infty$, $E \subset \R^n$ a closed subset and $B$ a ball centered on $E$ with $\hdc(B \cap E) > 0$. Then 
\begin{align*}
\betae{1}(B) \lesssim_n \betae{p}(B).
\end{align*}
\end{lemma}

\begin{remark}
From Lemma \ref{lemma:betaincreasep}, we see that it is enough to show \eqref{e:main} for $\betae{p}$, with $p \geq 2$. 
\end{remark}

\subsection{Construction of the approximating skeleta $E_R$} \label{s:ER}
In this subsection we introduce a construction from \cite{azzam-villa19}; this is a corona decomposition of a lower regular set $E$ (in the sense of \eqref{e:LCR}) in terms of Ahlfors regular sets $E_R$ (as in \eqref{e:ADR}). The following lemma from \cite{azzam-villa19} makes this precise. 
\begin{lemma}[\cite{azzam-villa19}, Main Lemma]\label{l:corona}
Let $k_0>0$, $\tau>0$, $d>0$ and $E$ be a set that is $(c_0,d)$-lower content regular. Let $Q_{0} \in \dD_{0}$ and $\dD(k_0)=\bigcup_{k=0}^{k_0}\{Q\in \dD_{k}|Q\subseteq Q_0\}$. Then we may partition $\dD(k_{0})$ into stopping-time regions $Tree(R)$ for $R$ from some collection $Top(k_{0})\subseteq \dD(k_{0})$ with the following properties: 
\begin{enumerate}
\item We have 
\begin{equation}
\label{e:ADR-packing}
\sum_{R \in Top(k_{0})} \ell(R)^{d} \lec_{c_0,d} \cH^{d}(Q_0).
\end{equation}

\item Given $R\in \Top(k_{0})$ and a stopping-time region $\cT(Q) \subseteq \Tree(R)$ with maximal cube $Q$, let  $\cF(Q)$ denote the minimal cubes of $\cT(Q)$ and 
\begin{align}\label{e:d_F}
    d_{\cF(Q)}(x) = \inf_{P \in \cF(Q)} \ps{ \ell(P) + \dist(x,P)}
\end{align}
For $C_{1}>4$ and $\tau>0$, there is a collection  $\cC_Q$ of disjoint dyadic cubes covering $C_{1}B_{Q}\cap E$ so that 
if 
\[
E_{\cT(Q)}=\bigcup_{I\in \cC_Q} \d_{d} I,\]
where $\d_{d}I$ denotes the $d$-dimensional skeleton of $I$, then the following hold:
\begin{enumerate}
\item $E_{\cT_Q}$ is Ahlfors regular with constants depending on $C_{1},\tau,d$ and $c_0$.
\item We have the containment
\begin{equation}
\label{e:contains}
C_{1}B_{Q}\cap E \subseteq \bigcup_{I\in \cC_Q} I\subseteq 2C_{1}B_{Q}.
\end{equation}

%
%Let $\cC_{\cF}$ denote the maximal dyadic cubes $I$ for which $\ell(I)<\tau \inf_{x\in I}d_{\cF}(x)$, let $C_{0}>4$, and set 
%\[E_{\cT}=\bigcup_{I\in \cC_{\cF} \atop I\cap C_{0}B_{T}\neq\emptyset} \d_{d} I\] 
%where $\d_{d}I$ denotes the $d$-dimensional skeleton of $I$. Then $E(\cT)$ is Ahlfors $d$-regular,
\item $E$ is close to $E_{\cT(Q)}$ in $C_{1}B_{Q}$ in the sense that
\begin{equation}
\label{e:adr-corona}
\dist(x,E_{\cT(Q)}) \lec  \tau d_{\cF(Q)}(x) \;\; \mbox{ for all }x\in E\cap C_{1}B_{Q}.
\end{equation}
\item The cubes in $\cC_Q$ satisfy
\begin{equation}
\label{e:whitney-like}
\ell(I)\sim \tau \inf_{x\in I} d_{\cF(Q)}(x) \mbox{ for all }I\in \cC_Q.
\end{equation}
\end{enumerate}
\end{enumerate}
\end{lemma}

For the sake of completeness and notation, we give a short sketch of the proof of Lemma \ref{l:corona}; for details, we refer the reader to \cite{azzam-villa19}. The idea is akin to Frostmann's Lemma and its proof (both can be found in \cite{mattila}, Chapter 8, from page 112). 

Assume without loss of generality that $Q_0 \subset [0,1]^n$; let us fix some notation:
\begin{align*}
    & \Delta_{j}(Q_0) := \ck{I \in \Delta_{j} \, |\, Q_0 \cap I \neq \emptyset };\\
    & \Delta(Q_0) := \bigcup_{j \geq 0} \Delta_{j}(Q_0).
\end{align*}
We also set
\begin{align*}
    V_{j}(Q_0):= \bigcup_{I \in \Delta_{j}(Q_0) } I.
\end{align*}
We are going to iteratively define a measure on the set the approximating set $V_{j}$; we then put all those dyadic cubes where this measure is too large is a family called $\Badsh{}$, to then perform a stopping time algorithm on the David-Christ cubes of $Q_0\subset E$, stopping whenever a David-Christ cubes hits a dyadic cubes in $\Badsh{}$ with comparable side length, and restarting after skipping one generation of cubes. Through this stopping time procedure we obtain the decomposition of $\dD(k_0)$ mentioned in Lemma \ref{l:corona}.

Let us define the measure mentioned above. For $m \in \N$  
\begin{align*}
    \mu_{m}^m := \mathcal{H}^n|_{V_{m}} 2^{(n-d)m}.
\end{align*}
 Note that then, if $I \in \Delta_{m}(Q_0)$, 
\begin{align*}
    \mu_{m}^m (I) = \ell(I)^d.
\end{align*}
We now define a family of cubes $\Badsh{}(m)$ as follows. First, we immediately impose that
\begin{align*}
    \Delta_{m}(Q_0) \subset \Badsh{}(m).
\end{align*}
Next, we look at the cubes one level up, that is, at the cubes in $\Delta_{m-1}(Q_0)$. If for one such cube $J$, we have
\begin{align*}
    \mu_{m}^m(J) > 2 \ell(J)^d,
\end{align*}
the we put $J$ in $\Badsh{}(m)$ and define
\begin{align*}
    \mu_{m}^{m-1}|_J := \ell(J)^d \frac{\mu_{m}^m|_J}{\mu_{m}^m(J)} < \frac{1}{2} \mu_{m}^m|_J.
\end{align*}
Otherwise, we set
\begin{align*}
    \mu_{m}^{m-1}|_J := \mu_{m}^m|_{J}.
\end{align*}
Note that in this way, it is always true that, for a cube $I \in \Delta_{m-1}(Q_0)$, $\mu_{m}^{m-1}(I) \leq 2 \ell(I)^d$. Continuing inductively in this fashion, we define $\mu_{m}^{m-2}$, $\mu_{m}^{m-3}$ and so on; suppose we defined $\mu_{m}^{k}$, for $1\leq k\leq m$. We consider the cubes $I \in \Delta_{k-1}$: if 
\begin{align*}
    \mu_{m}^{k}(I) > 2 \ell(I)^d, 
\end{align*}
then we put $I \in \Badsh{}(m)$ and set 
\begin{align*}
    \mu_{m}^{k-1}|_I := \ell(I)^d \frac{\mu_{m}^{k}|_I}{\mu_{m}^{k}(I)} < \frac{1}{2}\mu_{m}^k.
\end{align*}
Otherwise, we set
\begin{align*}
    \mu_{m}^{k-1}|_I:= \mu_{m}^{k}|_I.
\end{align*}
We stop when we reach $k=1$ (and so $\mu_{m}^0$ is defined). 
One can then show the packing condition
\begin{align} \label{e:Bad-est}
    \sum_{I \in \Badsh{}(m) } \ell(I)^d \leq C(n,d) \hd(Q_0),    
\end{align}
which is independent of $m \in \N$.
For a proof of this, see \cite{azzam-villa19}, in particular equation (3.5). 

Let now $k_0>0$ be an arbitrary integer number, $M>1$ a constant to be fixed later and $C_0>1$ the inflation constant for the $\beta$ numbers (see Constant \eqref{i:C0}). We now perform the stopping time mentioned above. We start with putting $Q_0 \in  \Tree(Q_0)$. If there exists a cube $Q \in \Child(Q_0)$ such that
\begin{align} \label{e:ST-cond}
    & MB_Q \cap I \neq \emptyset \enskip \enskip \enskip \mbox{ and}\\
    & \lambda \ell(I) \leq \ell(Q) \leq \ell(I),
\end{align}
where $\lambda$ is as in Theorem \ref{t:Christ},
then we stop. Otherwise we put all the cubes $Q \in \Child(Q_0)$ in $\Tree(Q_0)$; next we scan $\Child(Q_0)$ to see if any cube here has a child satisfying \eqref{e:ST-cond}. We proceed recursively in this fashion; the process will eventually terminate because we stopped at all cubes, or because we reached the bottom of $\dD(k_0)$. Furthermore, we consider all cubes $Q$ of the same generation of $Q_0$, so that
\begin{align*}
    2C_0 Q_0 \cap Q \neq \emptyset.
\end{align*}
We denote this family by $\dN(Q_0)$. 
On each of these cubes, we perform the same stopping time, so to construct the relative $\Tree(Q)$. Finally we put 
\begin{align} \label{e:forest}
    \Forest(Q_0) := \bigcup_{Q \in \dN (Q_0)} \Tree(Q),
\end{align}
and also
\begin{align*}
    \Stop(Q_0) := \ck{ Q \in \dD(k_0) \, |\, Q \mbox{ is minimal in } \Forest(Q_0)}.
\end{align*}
Next, we put
\begin{align*}
    \Next(Q_0) := \bigcup_{Q \in \Stop(Q_0)} \Child(Q).
\end{align*}
We now repeat the stopping time on each $R \in \Next(Q_0)$. Thus, if we set $\Top_0(k_0) :=\{Q_0\}$, then $\Top_1(k_0) := \Next(Q_0)$; proceeding inductively, supposed that $\Top_m(k_0)$ has been defined, for $m \in \N$: we put
\begin{align*}
    \Top_{m+1}(k_0) := \bigcup_{R \in \Top_m(k_0)} \Next(R).
\end{align*}
Finally, we set
\begin{align}
    \Top(k_0) = \bigcup_{k=0}^\infty \Top_k
\end{align}
Hence, to each element $R \in \Top$, there correspond a forest $\Forest(R)$ and a family of minimal cubes $\Stop(R)$. Now, for each $R \in \Top$, let us define
\begin{align}
    & d_{R}(x) := \inf_{Q \in \Stop(R)} \ps{ \ell(Q) + \dist(x, Q)}, \mbox{ and } \\
    & d_R(I) := \inf_{x \in I} d_{R}(x), \mbox{ whenever } I \in \Delta.
\end{align}
This is a now standard smoothing procedure which goes back to David and Semmes' \cite{david-semmes91}. 
Hence, for a parameter $\tau>0$, we put
\begin{align} \label{e:CR}
    \cC_R := \ck{ \mbox{ maximal } I \in \Delta \, |\, I\cap 2C_0 R \neq \emptyset \mbox{ and } \ell(I) < \tau d_R(I)}. 
\end{align}
Finally we set
\begin{align*}
    \wt E_R := \bigcup_{I \in \cC_R} \partial_d I.
\end{align*}
Thus $\wt E_R$ is the union of $d$-dimensional skeleta (see \eqref{e:skeleta}) of cubes belonging to $\wt E_R$. 

\begin{lemma}[\cite{azzam-villa19}, Lemma 3.6]
The set $\wt E_R$ is Ahlfors $d$-regular. 
\end{lemma}
\begin{remark}
The constant $M>1$ is fixed here: it has to be sufficiently large (depending on $\tau$). See the proof of Lemma 3.6 in \cite{azzam-villa19}.
\end{remark}

Let us state a couple of standard technical lemmas which will come handy later on in the paper. We add their proof in the appendix for the sake of completeness.
\begin{lemma} \label{l:meta1} Let $S$ be a cube in $\wt \Stop(Q)$ for some $Q \in \Next(R)$, $R \in \Top(k_0)$. Then there exists a dyadic cube $I_S := I \in \cC_{Q}$ so that $I_S \subset \frac{1}{2}B_S$ and $\ell(I_S) \sim \tau \ell(S)$.
\end{lemma}

\begin{lemma}\label{l:I-QI}
Let $I \in \cC_Q$ for $Q \in \Next(R)$, $R \in \Top(k_0)$. Then there exists a cube $Q_I \in \wt \Tree(Q)$ so that 
\begin{align*}
    & \ell(I) \leq \ell(Q_I) \leq c \tau^{-1} \ell(I); \\
    & \dist(I, Q_I) \leq c \tau^{-1} \ell(I). 
\end{align*}
\end{lemma}


We want to apply Lemma \ref{l:corona}, to obtain a corona decomposition of our set $E$, endowed with the topological condition \eqref{e:TC}. To do so, however, we first need to show that $E$ is lower content $d$- regular. 
\begin{lemma} \label{l:TP-LCR}
Let $E \subset \R^n$ be compact subset which satisfies the topological condition \eqref{e:TC} with parameters $r_0, \alpha_0, \delta_0$ and $\eta_0$. Then $E$ satisfies
\begin{align*}
    \hdc(E \cap B(x,r)) \gtrsim c_0 r^d
\end{align*}
for all $x \in E$ and $r< r_0$; the lower regularity constant $c_0$ will depend on $\delta_0$ and $\eta_0$. 
\end{lemma}
This fact is essentially present in Chapter 12 of \cite{david-semmes00}, although in a somewhat different form. We give a proof for this reason. 
We will first prove the following Sublemma, which will imply Lemma \ref{l:TP-LCR}.
\begin{sublemma} \label{sl:hdc-sl}
Let $E$ be a compact subset of $\R^n$ and let $(x, r) \in E \times \R_+$ be a pair so that
\begin{align} \label{e:small-content}
    \hdc(B(x,r) \cap E) < \mu \nu \, \delta_0 r^d
\end{align}
for a parameter $\nu$ \textup{(}sufficiently small depending on $\eta_0$\textup{)} and a number $\mu>0$ which depend  only on $\eta_0$ and $\delta_0$ \textup{(}as in Lemma \ref{l:TP-LCR}\textup{)}. Then there exists a one parameter family of Lipschitz mappings $\{\vp_t\}$ which satisfies \eqref{e:vp1}-\eqref{e:vp4} and so that $\vp_1$ maps $B(x,(1-\eta_0)r) \cap E$ into the $(d-1)$-dimensional skeleton of cubes from $\Delta_{j}$, where $j=j(\rho) \in \N$ is such that $2^{-j} \sim \rho$, and  $\rho = (\nu \delta_0)^{1/d} r$. 
\end{sublemma}
The proof of this Sublemma will follow quickly if we use the following Proposition from \cite{david-semmes00}.
\begin{proposition}[{\cite{david-semmes00}, Proposition 12.61}]\label{p:content} 
Let $A$ be a union of dyadic cubes from $\Delta_j$, where $j$ is some integer. There is a possibly small constant $c>0$ so that if $\theta \sim c\, 2^{-j}$, the following is true. Let $F$ be a compact subset of $A$ such that
\begin{align} \label{e:theta-small}
    \hdc(F \cap Q) < \theta \mbox{ for all } Q \in \Delta_{j}.
\end{align}
Then there is a Lipschitz mapping $\phi: F \to A$ so that $\phi(F) \subset \dS_{j, d-1}$ and $\phi(F \cap Q) \subset Q$ for all $Q \in \Delta_j$. Also, $\phi$ is homotopic to the identity through mappings from $F$ to $A$.  
\end{proposition}
%\michele{Sorry, maybe it's confusing, but here I'm proving the sublemma, not the proposition.}
\begin{proof}[Proof of Sublemma \ref{sl:hdc-sl}]
Let $\rho>0$ and $j(\rho) \in \N$ be as in the statement of the Sublemma, and let $\mu>0$, $\nu>0$ two possibly small parameteres to be fixed soon. Set
\begin{align} 
    & A^1:= \bigcup \ck{ I \in \Delta_{j(\rho)} \, |\, I \cap B\ps{x,(1-\mu)r} \neq \emptyset}, \label{e:A1}\\
    & A^2 := \bigcup \ck{ I \in \Delta_{j(\rho)} \, |\, I \cap A^1 \neq \emptyset}. \label{e:A2}
\end{align}
We want $\mu$ and $\nu$ to be so that
\begin{align}\label{e:mu-nu}
    \eta_0 > 10 \, \mu > 2(\nu \,  \delta_0)^d.
\end{align}
This choice then implies that
\begin{align}\label{e:A1subA2}
    E \cap B(x,(1-\eta_0) r) \subset E\cap B(x,(1-\mu)r) \subset E \cap A^1 \subset E \cap A^2 \subset B(x,r) \cap E,
\end{align}
Now, by the hypothesis \eqref{e:small-content}, we see that for any $I \in \Delta_{j(\rho)}$ which is also contained in $A^2$ we have 
\begin{align*}
    \hdc\ps{ I \cap (E \cap A^1) } < \mu\, \nu\, \delta_0 \,r^d = \mu\, \rho^d.
\end{align*}
Adjusting the choice of $\mu$ and $\nu$ if needed, we see that this implies \eqref{e:theta-small} to hold for all $I \in \Delta_{j(\rho)}$ which also lie in $A^2$ with $F= E \cap A^1$. Moreover, with this $F$, \eqref{e:theta-small} holds trivially for any other $I \in \Delta_{j(\rho)}$. Hence we apply Proposition \ref{p:content} with $j= j(\rho)$ (i.e. so that $2^{-j} \sim \rho$), $A=A^2$ as defined in \eqref{e:A2} and $F = A^1 \cap E$, as defined in \eqref{e:A1}. We obtain a Lipschitz mapping $\phi$ which sends $E \cap A^1$ into $\dS_{j(\rho), d-1}$ and all the properties listed in the proposition. Note in particular that with the choice \eqref{e:mu-nu} of $\mu$ and $\nu$ and the fact that $\phi(E\cap I) \subset I$ for any $I \in \Delta_{j(\rho)}$, we have that
\begin{align} \label{e:containment1}
    B\ps{x, (1-\eta_0)r} \cap \phi(E) = B\ps{ x, (1-\eta_0)r} \cap \phi(E \cap A^1) \subset \phi(E \cap A^1).
\end{align}

Now we can extend $\phi$ to be the identity outside of $A^2$. Setting 
\begin{align}
    \vp_t(y)= t\phi(y) + (1-t) y \mbox{ for } t \in [0,1],
\end{align}
it is easy to check that $\vp_t$ satisfies \eqref{e:vp1}-\eqref{e:vp4}.
\end{proof}

\begin{proof}[Proof of Lemma \ref{l:TP-LCR}]
For the sake of contradiction, suppose that for $x \in E$, and $r<r_0$, the inequality \eqref{e:small-content} holds. Then, using the definition of topological condition \eqref{e:TC} (which can be applied since $r<r_0$), we obtain
\begin{align*}
    \delta_0 r^d &
    < \hd\ps{B(x,(1-\eta_0)r) \cap \vp_1(E)}\\
    & = \hd\ps{B(x,(1-\eta_0)r) \cap \phi(E)} \\
    & \leqt{\eqref{e:containment1}} \hd\ps{\phi(E \cap A^1)} = 0.
\end{align*}
Thus we must have that for any such a pair $(x,r) \in E \times \R_+$, \eqref{e:small-content} cannot hold. This implies the lower content $d$-regularity of $E$ (for scales smaller than $r_0$), with constant $c_0$ depending only on $\delta_0$ and $\eta_0$. 
\end{proof}
\begin{remark}
Because all our statements are local, we will be ignoring the fact that our set is lower regular only for (possibly) small scales. In fact, we could assume without loss of generality that $r_0=1$. 
\end{remark}

We now see that whenever $E$ satisfies the topological condition \eqref{e:TC}, then it is also lower content $d$-regular. We therefore can apply Lemma \ref{l:corona} to $E$ and obtain a decomposition $\Top$ and for each $R\in \Top$, an Ahlfors regular set $\wt E_R$ wich approximate $E$ at a specific scale and location. Recall that the decomposition $\Top$ depends on the integer $k_0$: if we want to underline this, we may write $\Top(k_0)$. 

\subsection{Modification of $\wt E_R$}
In this subsection, we modify slightly the construction of $\wt E_R$; we need to do so to construct a coherent Federer-Fleming projection in the next section. 

Fix $R \in \Top$; recall the definition of $\cC_R$ in \eqref{e:CR}.
 Take a cube $I \in \cC_R$. Consider one of its $(n-1)$-dimensional faces, and denote it by $T_I$. Set 
\begin{align*}
    & \Adj^{n-1} (T_I) \\
    & := \ck{ J \in \cC_R \, |\, \ell(J) \leq \ell(I), \, J \cap T_I \mbox{ is an } (n-1) \mbox{-face of } J \mbox{ and } J \cap T_I \subset \Int(T_I) }
\end{align*}
We order the cubes in $\cC_R$ from the largest to the smallest one, and we label them as $I_0,....,I_N$, for some $N \in \N$. This is true because the cardinality of $\cC_R$ is finite (depending on $k_0$). 
Let us start our construction with $I_0 \in \cC_R$ (thus $I_0$ is the largest cube in $\cC_R$). We look at one of its $(n-1)$-dimensional faces, let us denote it by $T_{I_0}$. 
Now, let $I$ be a cube of minimal side length contained in $\Adj^{n-1}(T_{I_0})$; let $n(I) \in \N$ be such that $\ell(I) = 2^{-n(I)}$. We consider the family of cubes in $\Delta_{n(I)}$ such that they have an $(n-1)$-dimensional face contained in $T_{I_0}$. We call this family  $\Delta_{n(I)}(T_{I_0})$. Let us denote by
\begin{align} \label{e:tiles}
    \cD^{n-1}(T_{I_0})
\end{align}
the family of $(n-1)$-dimensional faces of the same side length of $I$, such that they are both an $(n-1)$-dimensional face of a cube $J \in \Delta_{n(I)}(T_{I_0})$ and also they are contained in $T_{I_0}$. We may refer to this family as the \textit{tiles} of $T_{I_0}$. 
%\michele{I think I need to improve the wording here.}
We repeat the same procedure for $I_1,...,I_N$; we don't do anything if $\Adj^{n-1}(T_{I_j})= \emptyset$ for some face $T_{I_j}$ of $I_j$, $1 \leq j \leq N$. Note that the definition of $\Adj^{n-1}(T_I)$ imposes the following: if two cubes $I$ and $I'$ are so that, say, $\ell(I)> \ell(I')$ and $I' \in \Adj^{n-1}(T_I)$, then the tiles constructed on $T_I$ will be the same one that we have on the face $T_{I'} \subset T_I$. The construction of tiles on the other $(n-1)$-faces of $I'$ will not change the ones already present in $T_{I'}$. 
This procedure terminates since $\cC_R$ is finite. 

Once we constructed $(n-1)$-dimensional tiles on all the $(n-1)$-dimensional faces of all cubes in $\cC_R$, we rest. After, we proceed as follows. 
Denote by 
\begin{align} \label{e:cF}
    \cF^{n-1}
\end{align}
the family of $(n-1)$-dimensional faces belonging to some cube in $\cC_R$. If $T \in \cF^{n-1}$ and $\cD^{n-1}(T) \neq \emptyset$, the put the elements of $\cD^{n-1}(T)$ in $\cF^{n-1}$ and take $T$ away. If $\cD^{n-1}(T) = \emptyset$, then leave $T$ in $\cF^{n-1}$.

%\begin{figure}[hbt!]
 %\centering
 %\includegraphics[scale=0.5]{Adj2.png}
 %\caption{The construction of the family of $(n-2)$ dimensional faces $\Adj^{n-2}(F_{T_0})$.}
%\end{figure}

Next, we repeat the previous construction: order the elements of $\cF^{n-1}$ in decreasing order with respect to side length and consider $T_0$ (the largest face in $\cF^{n-1}$). For each $(n-2)$-dimensional face $F_{T_0}$ of $T_0$ we set
\begin{align*}
    & \Adj^{n-2}(F_{T_0})\\
    & := \ck{ T \in \cF^{n-1} \, |\, \ell(T) < \ell(T_0), \, T \cap F_{T_0} \mbox{ is an } (n-2)-\mbox{face of } T \mbox{ and } T \cap F_{T_0} \subset F_{T_0} }. 
\end{align*}
We now look for the minimal element of $\Adj^{n-2}(F_{T_0})$, and call it $T$. Let $n(T) \in \Z$ so that $\ell(T) = 2^{n(T)}$; we now tessellate $F_{T_0}$ with tiles of side length $2^{n(T)}$; by tessellate here we mean the obvious thing, i.e. we substitute $F_{T_0}$ with its children of size $2^{n(T)}$. 
Let us denote the tiles so constructed by
\begin{align*}
    \cD^{n-2}(F_{T_0}). 
\end{align*}
We repeat the same procedure for $T_1,...,T_{N'} \in \cF^{n-1}$. Again, the construction of $(n-2)$-dimensional tiles for smaller $(n-2)$-dimensional faces does not affect the previously constructed tiles for larger faces. 
This procedure terminates since $\cF^{n-1}$ is finite, which follows trivially from $\cC_R$ being finite. 
Next, we set 
\begin{align*}
    \cF^{n-2} 
\end{align*}
to be the family of $(n-2)$-dimensional faces coming from elements of $\cF^{n-1}$, and we immediately modify it as above: if $\cD^{n-2}(F_T) \neq \emptyset $, for $T \in \cF^{n-1}$, we substitute $F_T$ with the corresponding family of tiles. 

We continue this construction: we obtain $\cF^{n-3}$ from $\cF^{n-2}$, $\cF^{n-4}$ from $\cF^{n-3}$, and so on, until we construct $\cF^d$. We stop at this point and we set 
\begin{align} \label{e:newER}
   E_R := \wt E_R \cup \ps{\bigcup_{F \in \cF^d} F}.
\end{align}
\begin{lemma}
The set $E_R$ is Ahlfors $d$-regular. 
\end{lemma}
\begin{proof}
Lower regularity follows immediately from the definition and the lower regularity of $\wt E_R$. On the other hand, note that for any cube $I \in \cC_R$, any smaller neighbouring cube $I' \in \cC_R$ will satisfy $\ell(I')> \tau \ell(I)$. If we envelope $I$ in cubes of side length $\ell(I) \tau$ and we consider the $d$-dimensional skeleton of this family of cubes, we see that the overall additional mass will not exceed a constant times $\ell(I)^d$, where such a constant depends on $n$, $d$ and $\tau$. Thus upper regularity is also preserved.
\end{proof}

\begin{notation} \label{n:C3}
From now on, we fix the notation for the regularity constant of $E_R$: it will be denoted by $C_3$.
\end{notation}

==> 06-2-FFproj.tex <==
\section{Federer-Fleming projections}
In this section we will construct a Federer-Fleming projection of $E$ onto a subset of $E_R$; we will use these projections in the next section to prove that the topological condition \eqref{e:TC} on $E$ implies the condition STC on the approximating skeleta.  Our construction will mimic the one in \cite{david2004hausdorff}, which in turn comes from \cite{david2000uniform}. The difference here is that we are dealing with a skeleton of faces coming from cubes of different sizes.
\\
\\
\noindent
Let $B(x,r)$ be a ball centered on the set $E$ (the construction below will be applied to the ball $B(x_2,r_2)$ as in the definition of STC, Definition \ref{d:TND}). Set
\begin{align}
    & \cC_R(x,r) := \left\{ I \in \cC_R \, |\, I \cap B(x,r) \neq \emptyset\right\}; \label{e:C_R(x,t)}\\
    & \cF^{m}(x,r) := \ck{ T \in \cF^{m} \, |\, T \cap B(x,r) \neq \emptyset } \mbox{ for } d \leq m \leq n-1; \label{e:F(x,r)} \\
    & D_R(x,r) := \bigcup_{I \in \cC_R(x,r)} I. \label{e:D-R}
\end{align}
Furthermore, we set $\cC_R^2(x,r)$ to be the family of dyadic cubes composed by $\cC_R(x,r)$ together with a maximal subfamily of cubes 
$J \in \Delta\setminus \cC_R$ so that 
\begin{align}
    & \Int(J) \subset \ps{ \bigcup_{I \in \cC_R(x,r)} I}^c; \label{e:C2a}\\
    & \mbox{there exists a dyadic cube } I \in \cC_R(x,r) \st I \cap J \neq \emptyset, \label{e:C2b}
\end{align}
and moreover, if we 
    let  
\begin{align*}
    \dN(J)  \mbox{ be the family of cubes in } \cC_R(x,r) \mbox{ which intersect  } J,
\end{align*}
we ask that
\begin{align} \label{e:C2c}
    \min\ck{\ell(I) \, |\, I \in  \dN (J)} \leq \ell(J) \leq \max\ck{\ell(I) \, |\, I \in  \dN(J)}.
\end{align}
The family $\cC^2_R(x,r) \setminus \cC_R(x,r)$ forms a sheath for $\cC_R(x,r)$ (imagine the plastic covering of some Minecraft electrical wires). Finally we define
\begin{align} \label{e:D-R-2}
    D_R^2(x,r):= \bigcup_{I \in \cC_R^2(x,r)} I.
\end{align} 
%\begin{figure}[hbt!]
% \centering
% \includegraphics[scale=0.6]{DR.png}
% \caption{The sets $D_R(x,r)$ and $D_R^2(x,r)$.}
%\end{figure}

Recall the definition of $E_R$ as in \eqref{e:newER}. The following lemma is similar to Proposition 3.1 in \cite{david2000uniform}, and so is the proof. The only difference is that we are working with a non-uniform grid of cubes. 
\begin{lemma}\label{l:FF}
Given $(x,r) \in E\times \R_+$, there exists a Lipschitz map $\pi : \R^n \to \R^n$ such that 
\begin{align}
    & \pi(y)=y \mbox{ whenever } x \in \R^n \setminus D_R^2(x,r); \label{e:pi1}\\
    & \pi(I) \subset I \mbox{ if } I \in \cC_R^2(x,r); \label{e:pi2}\\
    & \pi(E) \cap I \subset E_R \cap I \mbox{ for any } I \in \cC_R(x,r). \label{e:pi3}
\end{align}
\end{lemma}
We will obtain our Federer-Fleming projection as the composition of a finite number of maps which we will define inductively. 
We start by defining a map, let us call it $\pi_1$, that will send points in $D_R^2(x,r) \cap E$ into $(n-1)$-dimensional faces. We define $\pi_1$ on each individual cube $I \in \cC_R^2(x,r)$ as follows. Pick a point $c_I \in I$ such that $c_I \notin E$. This is possible since $\hd(E)<\infty$ (recall \eqref{e:hdE}) and thus, in particular, $\dim_H(E) < d+1$; a standard argument then shows that $E$ is porous, and thus such a point $c_I$ must exist. Then for $y \in E \cap \Int(I)$, we set 
\begin{align}\label{e:pi1-a}
    \pi_1(y) \mbox{ to be the point where the line passing through } y  \mbox{ and } c_I \mbox{ meets } \partial I;
\end{align} 
note that, then, $\pi_1(y)$ belong to some $(n-1)$ dimensional face of $I$. On the other hand, if $y \in E\cap \partial I$, we set 
\begin{align} \label{e:pi1-b}
    \pi_1(y)=y.
\end{align}
We then 
\begin{align} \label{e:pi1-c}
    \mbox{extend } \pi_1 \mbox{ on the whole of } I  \mbox{ such that } \pi_1(I) \subset I \mbox{ and } \pi_1 \mbox{ is Lipschitz on } I.
\end{align} 
(This can be done via standard extension results, see for example \cite{heinonen}).
Note that this definition is coherent, in the sense that one can glue together the definition of $\pi_1$ on each $I \in \cC_R^2(x,r)$  into a unique map $\pi_1$ defined on the whole of $D^2_R(x,r)$. Indeed, if $I, I' \in \cC_R^2(x,r)$ are so that $I \cap I' \neq \emptyset$, then the definition of $\pi_1$ on $I'\cap I$ must agree, since $I \cap I'$ is contained in $\partial I$ and $\partial I'$. Furthermore, we extend the definition of $\pi_1$ to $\R^n \setminus D_R^2(x,r)$ by setting \begin{align}\label{e:pi1-d}
    \pi_1(y)=y
\end{align}
there. Thus \eqref{e:pi1-a}-\eqref{e:pi1-d} give a coherent definition of $\pi_1$ on the whole of $\R^n$. 

\begin{figure}[hbt!]
 \centering
 \includegraphics[scale=0.4]{FF-proj2.png}
 \caption{The first step in the construction of Federer-Fleming projections.}
\end{figure}

Now, if $d=n-1$, we stop here and we set $\vp := \pi_1$. Otherwise, we continue as follows. We want to send points on the $(n-1)$-dimensional faces of cubes in $\cC_R(x,r)$ to the boundaries of these faces, which are, in turn, $(n-2)$-dimensional faces. To do this, we proceed, as above, by defining the map we need on each individual face.
Recall the definition of $\cF^{n-1}$ in \eqref{e:cF}. Let us start by defining $\pi_2$ on each $\partial T \cup (\pi_1(E) \cap T)$, where $T \in \cF^{n-1}$: we repeat the construction above. Namely, 
\begin{align} \label{e:pi2a}
    \mbox{we find a point } c_T \in \Int(T) \setminus \pi_1(E) \mbox{ and then project radially } \pi_1(E)\cap T \mbox{ onto } \partial T;
\end{align} 
once again, this definition leave unchanged those points which already belong to $\partial T$. Next, 
\begin{align} \label{e:pi2b}
    & \mbox{we extend } \pi_2 \mbox{ to the whole of } D_R(x,r)  \mbox{ by requiring that } \nonumber \\
    & \pi_2(I) \subset I \mbox{ for any } I \in \cC_R(x,r).
\end{align}
Let us say a few words on how to construct such an extension. Given $I \in \cC_R(x,r)$, let $T$ be one of its $(n-1)$-dimensional faces. We know $\pi_2$ on $T \cap \pi_1(E)$ and on $\partial T$. We can then extend $\pi_2$ as a Lipschitx map from $T$ to $T$ via standard extension results. We now want to extend $\pi_2$ from $\partial I$, to the whole of $I$, with the requirement that $\pi_2(I) \subset I$. To do so, let $c_I$ be the center of $I$. We set $\pi_2(c_I):= x^*$, where $x^*$ is any point in $\pi_2(\partial I)$. Then for any point $y \in \partial I$, and a point $x = t c_I + (1-t) y$, $t \in [0,1]$, (so that $x$ belongs to the line segment from $c_I$ to $y$), we set
\begin{align*}
    \pi_2 (x) = t \pi_2(c_I) + (1-t) \pi_2(y).
\end{align*}
Note that, because both $\pi_2(c_I)$ and $\pi_2(y)$ belong to $\partial I$, and $I$ is convex, then $\pi_2(x) \in I$. 
Let us check that $\pi_2$ so defined is Lipschitz on $I$. Take any two points $x_1, x_2 \in I$ and write them as
\begin{align}
    & x_1= t c_I + (1-t) y_1, \, \, t \in [0,1] \mbox{ and } y_1 \in \partial I;\label{e:x1}\\
    & x_2= s c_I + (1-s) y_2,\, \, s \in [0,1] \mbox{ and } y_2 \in \partial I. \label{e:x2}
\end{align}
Assume first that $t=s$. We can assume that $t=s<1$, for otherwise $x_1=x_2$. In this case, we have that
\begin{align*}
    |\pi_2(x_1) - \pi_2(x_2)| & = |(1-t)(\pi_2(y_1)-\pi_2(y_2))| \\
    & \leq C \, |(1-t)(y_1-y_2)| \\
    & = |x_1-x_2|.
\end{align*}
Here the constant $C$ is the Lipschitz constant of $\pi_2$ as function defined on $\partial I$.

Next, let us suppose that for $x_1$ and $x_2$ as in \eqref{e:x1} and \eqref{e:x2}, we have that $y_1=y_2$, hence they lie on the same line segment from $c_I$ to $\partial I$. We first note that (assuming without loss of generality that $t>s$), 
\begin{align*}
|x_1 - x_2| = |(t-s) (c_I - y_1)| \geq (t-s) \ell(I).  
\end{align*}
On the other hand, we have that
\begin{align*}
    |\pi_2(x_1) - \pi_2(x_2)|= |(t-s)(\pi_2(c_I) - \pi_2(y_1))| \leq \sqrt{n}\, (t-s) \ell(I).
\end{align*}
Thus $|\pi_2(x_1) - \pi_2(x_2)| \leq \sqrt{n}|x_1-x_2|$. Finally, for  any two points $x_1, x_2 \in I$ as in \eqref{e:x1} and  \eqref{e:x2}, put
\begin{align*}
    x_2':= t\, c_I + (1-t)y_2.
\end{align*}
Note that there exists a constant, depending only on $n$, so that
\begin{align}
|x_2 - x_2'| \leq C \, |x_1 - x_2|,    
\end{align}
%\michele{Should I prove this?}
But then, by the triangle inequality, we also have that
\begin{align*}
    |x_1-x_2'| \leq C |x_1-x_2|. 
\end{align*}
This give us the following:
\begin{align*}
    |\pi_2(x_1) - \pi_2(x_2)| &  \leq |\pi_2(x_1) - \pi_2(x_2')| + |\pi_2(x_2') - \pi_2(x_2)| \\
    & \leq C \ps{ |x_1- x_2'| + |x_2'-x_2|} \\
    & \leq C' |x_1-x_2|. 
\end{align*}
This proves that the extension of $\pi_2$ to the whole of $I$ is indeed Lipschitz, with a Lipschitz constant comparable to that of $\pi_2$ as defined on $\partial I$. Now we let $\pi_2$ on $D(x,r)$ to be piecewise defined on each $I$ of $\cC_R(x,r)$. 

Let us see why this definition is coherent. If $T, T' \in \cF^{n-1}$, $T \cap T' \neq \emptyset$ and let us assume without loss of generality that $\ell(T') < \ell(T)$, then either 
\begin{align}\label{e:pi2-case1}
    T' \subset T,
\end{align}
or
\begin{align} \label{e:pi2-case2}
    T \cap T' \subset \ps{\partial T} \cup \ps{\partial T'}.
\end{align}
If \eqref{e:pi2-case2} holds, than we immediately see that the definition of $\pi_2$ is coherent, since we defined to be the identity on both $\partial T$ and $\partial T'$. 
We divert a moment from the main construction to show that the former case does not happen.
\begin{lemma}
The case \eqref{e:pi2-case1} does not occur.
\end{lemma}
\begin{proof}
Let $T \in \cF^{n-1}(x,r)$, and assume first that $T$ is an $(n-1)$-dimensional face (as opposed to a tile) of a cube $I \in \cC_R(x,r)$. Suppose that there exists an element $T'$ of $\cF^{n-1}(x,r)$ such that $T' \subset T$. If $T'$ is an $(n-1)$-dimensional face of a cube $I' \in \cC_R(x,r)$, then, by construction of $\cF^{n-1}(x,r)$, we must have that
$I' \in \Adj^{n-1}(T)$. But then $F$ cannot possibly belong to $\cF^{n-1}$. On the other hand, if $T'$ is a tile, then also in this case $T$ cannot be in $\cF^{n-1}$, since it should have been tessellated into tiles of the same size of $T'$. 

Suppose now that $T$ is a tile itself. But by construction, we cannot have two tiles of different sizes lying on the same $(n-1)$-dimensional face. Thus $T' \subset T$ has to really be $T' = T$, which contradicts the fact that $\ell(T')< \ell(T)$.
\end{proof}
Thus the definition of $\pi_2$ is coherent.
Let us now define $\pi_2$ on those $(n-1)$-dimensional faces $T'$  of cubes in $\cC_R^2(x,r)$ such that $\Int(T') \nsubseteq \Int(D_R(x,r))$ (recall the definition of $D_R(x,r)$, \eqref{e:D-R}). 
These are the faces which form the external boundary of the sheath $\cC_R^2(x,r) \setminus \cC_R(x,r)$. For these faces we leave everything unchanged, i.e. we let
\begin{align}\label{e:pi2c}
    \pi_2(y) = y  &\mbox{ for any } y \in T, \\
    & \mbox{ where } T \mbox{ is a } (n-1)\mbox{-dimensional face } T \mbox{ with } T \nsubseteq D_R(x,r).
\end{align}\label{e:pi2d}
Finally, we extend $\pi_2$ to the whole of $D^2_R(x,r) \setminus D_R(x,r)$ by requiring that 
\begin{align}
    & \pi_2(I) \subset I \mbox{ for } I \in \cC^2_R(x,r)\setminus \cC_R(x,r) \nonumber \\
    & \pi_2(y) = y \mbox{ whenever } y \in \partial D_R^2(x,r).
\end{align}
(This can be done in the same fashion as for \eqref{e:pi2b}).
We finally set 
\begin{align}\label{e:pi2e}
    \pi_2(y)=y \mbox{ whenever } y \in \R^n \setminus D_R^2(x,r).
\end{align}
Hence \eqref{e:pi2a}-\eqref{e:pi2e} give us a Lipschitz map $\pi_2$ defined on the whole of $\R^n$.
Now, if $d=n-2$, then we can set $\vp = \pi_2 \circ \pi_1$, otherwise we continue projecting. To do so, we define a third map $\pi_3$. We follow the procedure above: first, if $F$ is an $(n-2)$-dimensional element of $\cF^{n-2}(x,r)$, then we set $\pi_3$ to be the radial projection from some point $c_F \in \Int(F) \setminus \pi_2 \circ \pi_1(E)$ defined on $\partial F \cup \ps{\pi_1 \circ \pi_2 (E) \cap F}$. In particular, $\pi_3(y)=y$ if $y \in \partial F$. Next, we extend $\pi_3$ to the whole of $T$, by requiring that $\pi_3(T) \subset T$; if there is an element $F$ of $\cF^{n-2}$ such that $(\pi_2 \circ \pi_1) (E) \cap F = \emptyset$, we set $\pi_3(y)=y$ on such an element. Note that this definition is coherent by construction of $\cF^{n-2}(x,r)$, as in the definition of $\pi_2$. Next, we extend the definition of $\pi_3$ to the faces $T$ of dimension $(n-1)$, requiring that for any such a face, we have $\pi_3(T) \subset T$ and $\pi_3(\Int(T)) \subset \Int(T)$; we also require that $\pi_3(y) = y$ on those faces $T$ such that $T \cap D_R(x,r) = \emptyset$. Finally, we extend $\pi_3$ to the whole cubes $I$, requiring again that $\pi_3(I) \subset I$. At this point, note that for $y \in E$, we have 
\begin{itemize}
    \item  
    either $\pi_3 \circ \pi_2 \circ \pi_1 (y)\in \R^n \setminus D^2_R(x,r)$ if $ y \in E \setminus D^2_R(x,r)$;
    \item 
    or $\pi_3 \circ \pi_2 \circ \pi_1 (y) \in T$, where $T$ is a $(n-1)$-dimensional face of a cube in  $\cC_R^2(x,r) \st T \nsubseteq D_R(x,r)$; 
    \item
    or  $\pi_3 \circ \pi_2 \circ \pi_1 (y) \in F$,  where $F \in \cF^{n-3}$.
\end{itemize}
\begin{remark}
The second possibility only occurs for those $y \in E$ so that 
\begin{align*}
    y \in \bigcup_{I \in \cC^2(x,r) \setminus \cC(x,r)} I \subset \R^n \setminus B(x,r).
\end{align*}
\end{remark}
We continue constructing projections in this fashion until reaching the $d$-dimensional skeleton.
At each step, we construct $\pi_m$, for $n-d \leq m \leq n$, first on the elements of $\cF^m(x,r)$ as a radial projection, and second we extend this definition to faces (or tiles) of increasing dimension, asking (if $F'$ represents on such face or tile) that $\pi_m (F') \subset F'$. 
We stop once $\pi_{n-d}$ has been defined. If $y \in E $, then, setting
\begin{align} \label{e:def-pi}
    \pi:= \pi_{n-d} \circ \cdots \circ \pi_1,
\end{align}
we see that
\begin{itemize}
    \item either $\pi(y)\in \R^n \setminus D_R^2(x,r)$, if $y \in E \setminus D^2_R(x,r);$
    \item or $\pi(y) \in T$, where $T$ is an $(n-1)$-dimensional face of a cube in $\cC_R^2(x,r)$ such that  $T \nsubseteq D_R(x,r)$;
    \item or $\pi(y) \in F$, where $F \in \cF^{d}(x,r)$.
\end{itemize}
Note that the definition of $\pi$ is coherent for the same reasons that $\pi_3$ and $\pi_2$ were coherent. In particular, $\pi$ is Lipschitz (with possible a very large Lipschitz constant, but we do not mind this). Moreover, it follows from the construction that the properties \eqref{e:pi1}, \eqref{e:pi2} and \eqref{e:pi3} are satisfied; this concludes the proof of Lemma \ref{l:FF}

==> 07-2-TP-TND.tex <==
\section{Topological stability of $E$ implies topological stability of the approximating set} \label{s:TC-STC}
In this section, we will prove that the topological condition \eqref{e:TC}, imposed on $E$, implies the condition
STC on the approximating sets $E_R$ (see in Definition \ref{d:TND}, see \eqref{e:TND-constants}-\eqref{e:TND5}).
Our proof follows that of David's, with a few tweaks. See \cite{david2004hausdorff}.
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{tc-stc.png}
    \caption{The topological condition on $E$ implies the skeletal topological condition on $E_R$.}
    \label{fig:tc-stc}
\end{figure}
\begin{lemma}\label{l:TC-STC}
Let $E \subset \R^n$ be such that $0<\hd(E)<\infty$. Suppose moreover that $E$ satisfies the $(r_0, \alpha_0, \delta_0, \eta_0)$-\eqref{e:TC}, for some given parameteres $r_0, \alpha_0, \delta_0, \eta_0$ and let $Q_0 \in \dD(E)$ be such that $\ell(Q_0)< r_0$. For some $k_0 \in \N$, apply Lemma \ref{l:corona} to $Q_0$ to obtain a corona decomposition $\Top(k_0)=\Top(Q_0, k_0)$ and a family of sets $\{E_R\}_{R \in \Top(k_0)}$ with parameter $\tau$. Then we can find parameters $r_1, \alpha_1, \delta_1$ and $\eta_1$, so that the family $\{E_R\}_{R \in \Top(k_0)}$ satisfies the $C_2$-\textup{(STC)} for $C_2$ sufficiently large. 
\end{lemma}
We will prove this lemma through a few lemmata below. 
%\michele{This $C_2$ will have to be larger than $C_1$, i.e. the ADR constant of $E_R$; how is this determined?}

Set 
\begin{align} \label{e:tau}
    \tau < \frac{1}{100} \min\{\alpha_0, \eta_0\}.
\end{align}

Now, let $\Top= \Top(k_0)$; recall that for a large constant $C_2$, we want to prove the existence of parameters $r_1$, $\alpha_1<1$ and $\delta_1$ (as in \eqref{e:TND-constants}) so that for all $x_1 \in E$, $R \in \Top$ and $Q \in \Tree(R)$ with $x_1 \in Q$, as in \eqref{e:TND-x1}-\eqref{e:TND-R}, for which \eqref{e:TND-upper} holds, we have the lower bound \eqref{e:TND4}. Let us immediately choose the parameters in \eqref{e:TND-constants} (our choice is that of David in \cite{david04}).
We set
\begin{align}
    & r_1 = r_0, \mbox{ where } r_0 \mbox{ is the one given by } \eqref{e:TC}; \label{e:r_0b} \\
    & \alpha_1 = C \min(\eta_0, \alpha_0); \label{e:alpha} \\
    & \eta_1 = C \frac{\delta_0}{C_2}; \label{e:eta} \\
    & \delta_1 = C \delta_0. \label{e:delta}
\end{align}
We will fix the various absolute constants $C$ as we go along. They will only depend on $n$.
Let $x_1$, $R$ and $Q$ as in \eqref{e:TND-x1}, \eqref{e:TND-R} and \eqref{e:TND-Q}. We now want to find a ball $B(x_2, r_2)$ with the required properties. We choose
\begin{align}
    & x_2= x_1 \mbox{ and } \label{e:TND-x}\\
    & r_2 \st \frac{\ell(Q)}{3} \leq r_2 \leq \frac{2\ell(Q)}{3}. \label{e:TND-r_2}
\end{align}
We would also like the quantity $\hd\ps{E_R \cap A_{\eta_1 \ell(Q)}(x_2,r_2)}$ to be small. Indeed, if we had that, for some choice of $r_2$, it held
\begin{align} \label{e:TP-TNDb}
    \hd\ps{E_R \cap A_{\eta_1 \ell(Q)} (x_2,r_2)} \lesssim \delta_1 \ell(Q)^d,
\end{align}
then in order to verify \eqref{e:TND4} (adjusting the constant in the definition of $\delta_1$), we would only have to check that 
\begin{align}\label{e:TP-TNDa}
\hd\ps{ \vp_1(E_R \cap B(x_2,r_2))} \geq \delta_1 \ell(Q)^d.     
\end{align}
Let us show that such a choice of $r_2$ is indeed possible. Let $s_1,...,s_N$ be a family of radii such that each one of them satisfies \eqref{e:TND-r_2} and $\ck{A_{\eta_1 \ell(Q)}(x_2, s_k)}_{k=1}^N$ is a pairwise disjoint family of (concentric) annuli. By the definition of $A_{\eta_1\ell(Q)} (x_2,r_2)$, we have that 
\begin{align*}
    N \gtrsim \frac{1}{\eta_1}.
\end{align*} 
Moreover, because these annuli are pairwise disjoint, we see that
\begin{align*}
    \sum_{k=1}^N \hd(E_R \cap A_{\eta_1 \ell(Q)} (x_2,s_k)) \leq \hd\ps{E_R \cap B(x_2, \ell(Q))} \leqt{\eqref{e:TND-upper}}  C_2 \ell(Q)^d. 
\end{align*}
Then by the pigeonhole principle and \eqref{e:eta} and \eqref{e:delta}, we must have that for some $1\leq k \leq N$, \eqref{e:TP-TNDb} holds putting $r_2=s_k$.
\begin{lemma} \label{l:IandQ}
Let $I \in \cC_R(x_2, r_2)$, where $\cC_R(x,r)$ is defined in \eqref{e:C_R(x,t)}; also, here $x_2=x_1 \in Q$, for some $Q \in \Tree(R)$, and $r_2$ is as in \eqref{e:TND-r_2}. Then 
\begin{align}
    \ell(I) \leq C\, \tau\, \ell(Q). 
\end{align}
\end{lemma}
\begin{proof}
It suffices to prove the lemma for $Q \in \Stop(R)$.
If $I \in \cC_R$, then we know that $\ell(I) \lesssim \tau d_R(I)$ (recall that $\tau$ depends on $\alpha_0$ and $\eta_0$ and was fixed in \eqref{e:tau}). Moreover, $d_R(\cdot)$ is 1-Lipschitz. Then if $y \in I \cap B(x_2, r_2)$, we have that
\begin{align*}
    d_R(I) \leq d_R(y) \leq |y-x_2| + d_R(x_2).
\end{align*}
Because $r_2 \sim \ell(Q)$, $|x_2-y| \leq \ell(Q)$. On the other hand, we see that $d_R(x_2) = \inf_{P \in \Stop(R)} \ps{ \ell(P) + \dist(x_2, P)} \leq \ell(Q)$. 
\end{proof}
\begin{remark}
Note that the same holds for any $I \in \cC_R^2(x_2,r_2)$, by definition of $\cC_R^2(x_2,r_2)$ (as defined in \eqref{e:C2a}, \eqref{e:C2b} and \eqref{e:C2c}). 
\end{remark}

\begin{lemma} \label{l:TND}
Let  $(x_2,r_2)$ to be as chosen in \eqref{e:TND-x} and \eqref{e:TND-r_2}. For any one parameter family of Lipschitz deformations $\ck{\vp_t}_{0\leq t \leq 1}$ satisfying \eqref{e:vp1}, \eqref{e:vp2}, \eqref{e:vp3} and \eqref{e:TND3} \textup{(}relative to $(x_2,r_2)$\textup{)}, the property \eqref{e:TP-TNDa} holds, that is, we have
\begin{align*}
    \hd(\vp_1(E_R \cap B(x_2, r_2))) \geq \delta_1 \ell(Q)^d. 
\end{align*}
\end{lemma}
\begin{proof}
We have two ingredients we want to put together to achieve \eqref{e:TP-TNDa}: on one hand, we know that something similar holds for $E$ (i.e. TC); on the other hand, we know that $E$ is locally well approximated by $E_R$, and we have a continuous (actually Lipschitz) way to move from $E$ to $E_R$ (i.e. the Federer-Fleming projection we constructed in the previous section). The idea is therefore the following: pick the one parameter family $\vp_t$ for which we want to show \eqref{e:TP-TNDa}, and pick $\pi$ as in Lemma \ref{l:FF}. We will construct from these a deformation $f$ which satisfies conditions \eqref{e:vp1}-\eqref{e:vp4}; hence from \eqref{e:TC}, we will deduce \eqref{e:TP-TNDa}.

Set 
\begin{align}
    \pi_t (y) := t\, y + (1-t)\, \pi(y).
\end{align}
Note that
\begin{align*}
    |\pi_t(y) - y |\leq t|\pi(y)-y| \leq n^{1/2} \ell(I), 
\end{align*}
if $y \in D_R^2(x_2,r_2)$; otherwise this quantity is equal to zero. By Lemma \ref{l:IandQ} we have that
\begin{align}
    \ell(I) \lesssim \tau d_R(y) \leq \tau \ps{|y-x_2| + d_R(x_2)} \lesssim \tau \ell(Q).
\end{align}
Thus we have 
\begin{align} \label{e:TP-TNDg}
    |\pi(y) - y| \lesssim \tau \ell(Q) \mbox{ for all } y \in \R^n.
\end{align} 
Let us now define $\{f_t\}_{0\leq t \leq 1}$. We set
\begin{align}
    f_t (y) := \begin{cases}
    \pi_{2t}(y) & \mbox{ if } 0 \leq t \leq \frac{1}{2};\\
    \vp_{2t-1} (\pi(y)) & \mbox{ if } \frac{1}{2}\leq  t \leq 1.
\end{cases}
\end{align}
We claim that $\{f_t\}$ satisfies the conditions \eqref{e:vp1}-\eqref{e:vp4} applied to the larger ball \begin{align}\label{e:TND-wt-r}
    B(x_2, \wt r) \mbox{ where } \wt r:= (1+ \eta_0)r_2. 
\end{align}
We verify these conditions one by one. It is immediate from the definition that each $f_t$ is Lipschitz. 

\underline{Claim.}
We have that $f_t(B(x,\wt r)) \subset \overline{B}(x, \wt r)$, i.e. \eqref{e:vp1} holds for $f_t$. 

Note that
\begin{align} \label{e:TP-TNDd}
    B(x_2,r_2) \cap E \subset D_R(x_2,r_2) \subset D_R^2(x_2,r_2),
\end{align}
where $D_R(x_2,r_2)$ and $D^2_R(x_2,r_2)$ were defined in \eqref{e:D-R} and \eqref{e:D-R-2}; indeed \eqref{e:TP-TNDd} follows immediately from the definitions. Moreover, using Lemma \ref{l:IandQ}, we see that
any cube which was added to $\cC_R^2(x_2,r_2) \setminus \cC_R(x_2,r_2)$, must have side length at most $C \tau \ell(Q)$ (recall that $Q$ satisfies \eqref{e:TND-Q}). Thus $D_R^2(x_2,r_2) \subset B(x_2,r_2+ C \tau \ell(Q))$ and also, since
\begin{align*}
    \tau \ell(Q) \leqt{\eqref{e:tau}} \frac{1}{100} \eta_0 \ell(Q) \leqt{\eqref{e:TND-r_2}} \eta_0 r_2,
\end{align*}
(where we used \eqref{e:tau} and \eqref{e:TND-r_2}),
we have that
\begin{align}
    D^2_R(x_2, r_2) \subset B(x_2, r_2+ \tau \ell(Q)) \subset   B(x_2, (1 + \eta_0) r) \subset B(x_2, \wt r), 
\end{align}
Let us consider a few cases separately.
\begin{itemize}
    \item 
If $y \in D^2_R(x_2,r_2)$, then $\pi_t(y) \in D^2_R(x_2,r_2)$ for all $0\leq t \leq 1$ (by Lemma \ref{l:FF}), and so 
\begin{align*} 
    f_s(y) \in B(x_2, \wt r) \mbox{ for } s \leq \frac{1}{2} \mbox{ whenever } y \in D_R^2(x_2,r_2).
\end{align*} 
Now, recall that \eqref{e:vp1} holds for $\vp_t$ (relative to $B(x_2,r_2)$); hence 
if, together with $y \in D_R^2(x_2,r_2)$, we also have that $\pi(y) \in B(x_2,r_2)$, we then conclude that $f_s(y) \in \overline{B}(x_2,r_2)$ for $\frac{1}{2} \leq s \leq 1$. Also \eqref{e:vp3} holds for $\vp_t$: if $\pi(y) \notin B(x_2,r_2)$, then, for $\frac{1}{2} \leq s \leq 1$ and recalling \eqref{e:TP-TNDd}, $f_s(y)= \pi(y) \in D_R^2(x_2,r_2)$. We obtain then that
\begin{align} \label{e:TP-TNDc}
    f_s(y) \in B(x_2, \wt r) \mbox{ whenever } y \in D_R^2(x_2,r_2).
\end{align}
Suppose now that $y \in B(x_2,\wt r) \setminus D_R^2(x_2,r_2)$; by construction $\pi(y)=y$ whenever $y \in \R^n \setminus D_R^2(x_2,r_2)$, hence $\pi_t(y) = y$ for $t \in [0,1]$, and thus
\begin{align} \label{e:TP-TNDe}
    f_s(y)=y \mbox{ for } s \leq \frac{1}{2} \mbox{ whenever } y \in B(x_2, \wt r) \setminus D_R^2(x_2,r_2).
\end{align} 
\item If $\pi(y) \in B(x_2,r_2) \setminus D_R^2(x_2,r_2)$, then $\vp_t(\pi(y)) \in \overline{B}(x_2,r_2)$ by \eqref{e:vp1} for $\vp_t$; if $\pi(y) \in B(x_2, \wt r) \setminus \ps{ B(x_2,r_2) \cup D_R^2(x_2,r_2)}$, then $\vp_t(\pi(y))=\pi(y)=y$. Thus we obtain that
\begin{align}\label{e:TP-TNDf}
    f_s(y) \in B(x_2, \wt r) \mbox{ for } \frac{1}{2} \leq s \leq 1 \mbox{ whenever  } y \in B(x_2, \wt r) \setminus D_R^2(x_2,r_2).
\end{align}
Now \eqref{e:TP-TNDc}, \eqref{e:TP-TNDe} and \eqref{e:TP-TNDf} give us the property \eqref{e:vp1} for $\{f_s\}$ relative to $B(x_2,\wt r)$. 
\end{itemize}

\underline{Claim.}
 \eqref{e:vp2} holds for $f_t$, that is, the path $s \mapsto f_s(y)$ is continuous. But this is clear, since $t \mapsto \pi_t(y)$ is continuous; moreover, $\pi_1(y)=\pi(y) = \vp_0(\pi(y))= f_{\frac{1}{2}}(y)$, and $t \mapsto \vp_{2t-1}(\pi(y))$ is also continuous.

\underline{Claim.}
Condition \eqref{e:vp3} holds. 

Indeed, $f_0(y)= \pi_0(y)=y$; if $y \in \R^n \setminus B(x_2,\wt r)$, we have seen above that $f_t(y)=y$. Thus \eqref{e:vp3} holds for $\{f_s\}$ in $B(x_2, \wt r)$. 

We now verify that also \eqref{e:vp4} holds, i.e. we need to show that $\dist(f_s(y), E) \leq \alpha_0 \wt r$ for $s \in [0,1]$ and $y \in E \cap B(x_2, \wt r)$. First, consider $0 \leq s \leq \frac{1}{2}$; let $y\in E \cap B(x_2,\wt r)$; then we have
\begin{align*}
    & \dist(f_s(y), E) = \dist(\pi_{2s}(y), E) \leq |\pi_{2s}(y)- y|\\
    & \leqt{\eqref{e:TP-TNDg}} n^{\frac{1}{2}} \tau \ell(Q) \leqt{\eqref{e:tau}} \frac{1}{3} \alpha_0 \ell(Q) \leqt{\eqref{e:TND-r_2}, \eqref{e:TND-wt-r}} \alpha_0 \wt r.
\end{align*}
Now suppose that $s> \frac{1}{2}$. If $y \in B(x_2, \wt r) \cap E$, then 
\begin{align}
    & \mbox{either } y \in D_R^2(x_2,r_2) \label{e:TP-TNDh} \\
    & \mbox{or } y \notin D^2_R(x_2,r_2) \cup B(x_2,r_2). \label{e:TP-TNDi}
\end{align}
If $y$ is so that \eqref{e:TP-TNDi} holds, then $\pi(y) =y$, and moreover, from \eqref{e:vp3} for $\vp_t$ relative to $B(x_2,r_2)$, we see that $\vp_{2s-1}(\pi(y))= \vp_{2s-1}(y) = y$. Hence \eqref{e:vp4} holds in this case. 
On the other hand, suppose that \eqref{e:TP-TNDh} holds. Then 
\begin{align}
    & \mbox{either } \pi(y) \in E_R \label{e:TP-TNDl}, \\
    & \mbox{or } \pi(y) \in T, \mbox{ where } T \mbox{ is an } (n-1)\mbox{-face with } T \nsubseteq D_R(x_2,r_2). \label{e:TP-TNDm}
\end{align}
If \eqref{e:TP-TNDl} holds, then $\dist(\vp_{2s-1}(\pi(y),E) \leq \alpha_1 \ell(Q)$ by \eqref{e:TND3} applied to $\vp_t$; this immediately implies $\dist(f_s(y), E) \leq \alpha_0 \wt r$ for $s> \frac{1}{2}$ by the choice of $\alpha_1$ in \eqref{e:alpha}. 
On the other hand, if \eqref{e:TP-TNDm} holds, we must have $\pi(y) \notin B(x_2,r_2)$ (by construction of $\pi$), and therefore $\vp_{2s-1}(\pi(y))= \pi(y)$. Now $\pi(y)$ belongs to a cube in $\cC_R^2(x_2,r_2)$ with side length at most $\tau \ell(R)$ and touching $E$, hence we retrieve $\dist(f_s(y), E)\leq \alpha \ell(R) \leq \alpha_0 \wt r$. Together with the previous estimates, we obtain that $\{f_s\}$ satisfies \eqref{e:vp4} for all $s \in [0,1]$. That is to say, we have that by the TC
\begin{align}\label{e:TP-TNDo}
    \hd\ps{ B(x_2,(1-\eta_0)\wt r) \cap f_1(E) } \geq \delta_0 \wt r^d.
\end{align}
Since $B(x_2, r_2) \supset B(x_2, (1-\eta_0) \wt r)$, \eqref{e:TP-TNDo} implies that
\begin{align}\label{e:TP-TNDp}
    \hd\ps{B(x_2,r_2) \cap f_1(E)} \geq \delta_0 (1+\eta_0)^d \,r_2^d.
\end{align}
Recall from above that if $y \in E$ and it is such that $y \notin D_R(x_2,r_2)$, then $f_1(y) \notin B(x_2,r_2)$. Thus, 
\begin{align*}
    B(x_2,r_2) \cap f_1(E) \subset f_1(D_R(x_2,r_2)\cap E).
\end{align*}
Note also that $\pi(E \cap D_R(x_2,r_2)) \subset E_R$. Thus we obtain, using \eqref{e:TP-TNDp}, \eqref{e:TP-TNDb} and \eqref{e:delta},
%\michele{Expand a little upon the last inequality.}
\begin{align*}
    \hd\ps{\vp_1(E_R) \cap B(x_2,r_2)} \geq 2 \delta_1 \ell(Q)^d. 
\end{align*}
This concludes the proof of Lemma \ref{l:TND}.
\end{proof}

Lemma \ref{l:TND} and the considerations given above \eqref{e:TP-TNDa} prove Lemma \ref{l:TC-STC}.

==> 08-2-AlmgrenQM.tex <==
\section{A further approximating set}\label{s:E-rho-STC}
We now construct a dyadic approximation of $E_R$. We will then show that this approximation satisfies the STC; in the next section, we will show that this implies that this dyadic approximation has large intersection with a uniformly rectifiable set. 
\\
\\
\noindent
Let $\rho$ be a small parameter (which we will fix later, and can be assumed to be of the form $2^{-k}, k \in \N$). We write
\begin{align*}
    \Delta_\rho := \Delta_{j(\rho)},
\end{align*}
where $j(\rho)$ is an integer so that $2^{-j(\rho)} = \rho.$
We set
\begin{align}
    & \cC_{R, \rho} := \ck{ I \in \Delta_{\rho} \, |\, I \cap E_R \neq \emptyset}; \label{e:cC-R-rho}\\
    & E_{\rho}= E_{R,\rho} := \bigcup_{I \in \cC_{R, \rho}} \partial_d I. \label{e:E-rho}
\end{align}

\begin{figure}[hbt!]
 \centering
 \includegraphics[scale=1.2]{Erho.png}
 \caption{The red set represents $E$. The black squares represents $E_R$. The blue smaller squares represent $E_{R, \rho}$.}
\end{figure}

\begin{lemma} \label{l:Erho-ADR}
Let $I_*$ be the smallest cube in $\cC_R$ (which exists since $\cC_R$ is finite). Then for all $\rho< \ell(I_*)$, $ E_\rho$ is Ahlfors regular, with the same regularity constant as $E_R$. 
\end{lemma}
\begin{proof}
Let $T$ be a $d$-dimensional face of some cube $J \in \cC_R$. Denote by $\cF^{d}_\rho$ the collection of $d$-dimensional faces from cubes in $\cC_{R, \rho}$. Then we can cover $T$ with a disjoint subcollection of $\cF^{d}_\rho$. If we denote such a collection by $\cF^{d}_\rho(T)$, then it is obvious that
\begin{align*}
    \hd(T) =\sum_{F \in \cF^d_{\rho}} \hd(F). 
\end{align*}
To each such a face $F \in \cF^d_{\rho}$, there corresponds a bounded number of cubes so that $F \subset I \in \cC_{R,\rho}$. This bounded number depends only on $n$ and $d$. Moreover, each of these cubes has a bounded number of other $d$-dimensional faces, and, again, this number depends only on $n$ and $d$. Thus, if we denote by $\Delta_\rho(T)$ the family of cubes in $\Delta_\rho$ which also meet $T$, we see that
\begin{align*}
   \sum_{I \in \Delta_\rho(T)} \hd(I) \leq C(n, d) \sum_{F \in \cF^{d}_\rho} \hd(F) = C(n,d)\, \hd(T).
\end{align*}
Then, we see that
\begin{align*}
    \hd\ps{ E_\rho \cap B(x,r)} & \leq \sum_{\substack{I \in \cC_{R,\rho}\\ I \cap B(x,r) \neq \emptyset}} \hd(I) \\
    & \leq \sum_{J \in \cC_{R}(x,r)} \sum_{T \,\text{face of } J} \sum_{I \in \cF^d_\rho(T)} \hd(I) \\
    & \leq C(n,d) \sum_{J \in \cC_{R}(x,r)} \hd(J) \\
    & \leq C_3 r^d.
\end{align*}
Lower regularity is even easier since we are adding mass. 
\end{proof}

\begin{lemma}
The set $E_\rho$ satisfies the condition STC relative to the scale of $R$ with the same constants as $E_R$.
\end{lemma}
\begin{proof}
Let $C_2$ be a constant sufficiently large (in particular, we need it to be larger than $C_3$, the regularity constant of $E_R$ and $E_\rho$). We know from Section \ref{s:TC-STC}, that $E_R$ satisfies the STC with a choice of constants as in \eqref{e:r_0b} - \eqref{e:delta}. Let $(x_2,r_2)$ as in \eqref{e:TND-x} and \eqref{e:TND-r_2}. %\michele{Make it clear that you are using STC at scale $R$}
We now add to the constraint on $\rho$ given in the statement of Lemma \ref{l:Erho-ADR}, the following one: we ask that
\begin{align} \label{e:rho}
    \rho < \frac{1}{1000\sqrt{n}} \min \ck{\eta_1, \alpha_1} \ell(R).
\end{align}
Note that because $E_\rho$ is Ahlfors regular independently of $\rho$, this does not cause any trouble. 

Note that $E_\rho \cap B(x_2,r_2) \supset E_R\cap B(x_2,r_2)$, simply because $E_R \subset E_\rho$. Thus, also $\vp_1(E_\rho \cap B(x_2,r_2)) \supset \vp_1(E_R\cap B(x_2,r_2))$, and therefore
\begin{align*}
    \hd(\vp_1(E_\rho \cap B(x_2, r_2))) & \geq \hd\ps{\vp_1(E_R \cap B(x_2,r_2))} \\
    &\geq \delta_1 \ell(R)^d + \hd(E_R \cap A_{\eta_1 \ell(R)}(x_2,r_2)).
\end{align*}
But now note that if we choose a parameter $c>0$ sufficiently small, and we put $\wt \eta_1 = c \eta_1$, then we see that
\begin{align*}
    \hd(E_R \cap A_{\eta_1 \ell(R)}(x_2, r_2)) \geq \hd(E_\rho \cap A_{\wt \eta_1 \ell(R)}(x_2, r_2)). 
\end{align*}
Note that $c$ only depends on $n$ and $d$. Hence we obtain that 
\begin{align} \label{e:STC-E-rho}
    \hd(\vp_1(E_\rho \cap B(x_2, r_2))) \geq \delta_1 \ell(R)^d + \hd(E_\rho \cap A_{\wt \eta_1 \ell(R)}(x_2, r_2)),
\end{align}
and the lemma is proven. 
\end{proof}


\section{STC implies that $E_\rho$ has large intersections with some uniformly rectifiable set}
In this section, we show that the topological condition STC imposed on $E_R$ (and thus on $E_\rho$) tells us that $E_\rho$ has a large intersection (large with respect to the scale of $R$) with a uniformly $d$-rectifiable set. The idea is to define a functional whose minimizer $F$ has large intersection with $E_\rho$. In turn $F$, by virtue of being a minimiser of such a functional, will turn out to be a quasiminimiser (in the sense of \cite{david-semmes00}), and thus uniformly rectifiable.

\begin{remark}
Once again, we follow David in \cite{david04} and we adapt his proof to our current situation.
\end{remark}

\subsection{Definition of a functional $J$.}
Let $C_2$ be a large constant and $k_0$ a suffciently large integer. Then STC gives us  constants $r_1$, $\alpha_1<1$, $\eta$ and $\delta_1$ (as in \eqref{e:TND-constants}) such that for every choice of $x_1 \in E$ and $R \in \Top(k_0)$ as in \eqref{e:TND-x1} \and \eqref{e:TND-R} (here we are applying STC with the cube $Q$ to be equal to $R$ itself), so that $\hd(E_R \cap B(x_1, \ell(R))) \leq C_2 \ell(R)^d$ holds, we can find a ball $B(x_2,r_2) \subset B(x_1, \ell(R))$ for which, given an appropriate one-parameter family of Lipschitz deformations $\{\vp_t\}$, we have the lower bound \eqref{e:TND4}. From the previous section, we see that this holds (at this specific scale $\ell(R)$) for both $E_\rho$ and $E_R$.

To implement the idea described above, we first need a functional: to define a functional, we need to clarify upon which type of sets it will act, and where these sets may be. In other words, we need to determine an appropriate class of subsets as domain of definition of such a functional. To simplify the notation, we put
\begin{align}
    & r:= r_2;\\
    & x := x_2.
\end{align}
For later use, let us set
\begin{align}\label{e:Bj}
    B_j:= B\ps{x, r - \eta_1 \ell(R) + \frac{j \eta_1 \ell(R)}{10}} \mbox{ for } 0 \leq j \leq 10.
\end{align}
Note that $B_{10}= B(x,r)$ and $B_{10}\setminus B_0 =A_{\eta_1 \ell(R)} (x,r)$. 

Recall the constraint on $\rho$, \eqref{e:rho}, and consider a constant $\sigma$ (let it be a power of $2$), so that
\begin{align} \label{e:sigma}
    \frac{1}{200\sqrt{n}} \min\ck{\eta_1, \alpha_1} \ell(R) \leq \sigma \leq \frac{1}{100\sqrt{n}}  \min\ck{\eta_1,\alpha_1} \ell(R).
\end{align}
Then we put
\begin{align}
    & \Delta_{\sigma}(B_6):= \ck{ I \in \Delta_{j(\sigma)} \, |\, I \cap B_6 \neq \emptyset};\label{e:delta6}\\
  & \cC_{\sigma}^1(B_6) := \ck{ I  \in \Delta_\sigma(B_6) \, |\, I \cap E_R \neq \emptyset }; \label{e:cCB6}\\
  & \cC_{\sigma}^2(B_6) := \ck{ I \in \Delta_\sigma(B_6) \, |\, \mbox{ there exists a } J \in \cC_\sigma^1(B_6) \mbox{ with } I \cap J \neq \emptyset}.
\end{align}
Finally we put
    \begin{align}
        & V^1 := \bigcup_{I \in \cC^1_{\sigma}(B_6)} I  \enskip \enskip \mbox{ and}\label{e:V1}\\
        & V^2 := \bigcup_{I \in \cC^2_{\sigma}(B_6)} I. \label{e:V2}
    \end{align}
    %\begin{figure}[hbt!]
 %\centering
 %\includegraphics[scale=0.5]{Esigma.png}
 %\caption{How I imagine $V^1$.}
%\end{figure}
  %  \michele{Perhaps a better definition would be to have $V^2$ to wrap around $V^1$ without ever enclosing it.}
Note that for any cube $I \in \cC_R(B_6)$, there exists a cube $J \in \cC_{\sigma}(B_6)$ so that $J \supset I$. %\michele{Is this important?}
\begin{lemma}
%\michele{It is also true that $E_R \cap B_6 \subset V^2$}
With the notation above, we have that
\begin{align}
    & B_6\cap E \subset V^2 \subset B_7 \mbox{ and } \label{e:Ta}\\
    & \dist(y, E) \leq \alpha_1 \ell(R) \mbox{ for all } y \in V^1.  \label{e:Tb}
\end{align}
\end{lemma}
\begin{proof}
The first inclusion in \eqref{e:Ta} is immediate. To see the second one, note that for any point $y \in V^2$, we have that $\dist(y, V^1) \leq \sqrt{n} \rho$. In turn, any point in $V^1 \setminus B_6$ can be at most $\sqrt{n}\rho$ away from $\partial B_6$. Hence, by the choice of $\sigma$ in \eqref{e:sigma}, we see that if $y \in V^2\setminus B_6$, $\dist(y, \partial B_6) < \frac{1}{10} \eta_1 \ell(R)$, and so \eqref{e:Ta} will be satisfied. Similarly for \eqref{e:Tb}: first, if $y \in V^1$, then $\dist(y, E_R) \leq \rho \leqt{\eqref{e:rho}} \frac{1}{1000\sqrt{n}} \ell(R)$. On the other hand, if $y' \in E_R$, then we have that $\dist(y', E) \leq \tau \ell(R)$ (this follows from Lemma \ref{l:IandQ}). But also $\tau << \min\ck{\eta_0,\alpha_0}$ (by \eqref{e:tau}) and thus $\tau \leq \alpha_1$ (using \eqref{e:alpha}). Therefore, letting $y' \in E_R$ to be such that $\dist(y, E_R) \sim |y-y'|$, we obtain
\begin{align*}
    \dist(y, E) \leq |y-y'| + \dist(y', E) \leq \rho + \tau \ell(R) \leq \alpha_1 \ell(R). 
\end{align*}
\end{proof}
We are now ready to fix the class of subsets upon which the said functional will be allowed to act. 
We set
\begin{align}
    \dF_0 \label{e:F_0}
\end{align}
to be the class of subsets $F$ of $\R^n$ such that
\begin{align}
    & F \mbox{ is closed (in the topology of $\R^n$).} \label{e:F_01}\\
    & F \subset V^2 \label{e:F_02}\\
    & F = F^* \cup L. \label{e:F_03}
\end{align}
Here $L$ denotes any subset of Hausdorff dimension smaller or equal than $d-1$; by $F^*$ we mean a finite union of $d$-dimensional faces of cubes coming from $\Delta_{\rho}$. We will call $F^*$ the \textit{coral} part of $F$. 
In other words the class $\dF_0$ is composed by subsets that are built out of a finite number of $d$-faces coming from cubes in $\Delta_\rho$. 

Let us consider a subclass of $\dF_0$: we set
\begin{align} \label{e:dF}
    \dF := \ck{ F \in \dF_0 \, |\,  F= \vp_1(E_\rho \cap V^2)},
\end{align}
where $\{\vp_1\}_{0 \leq t \leq 1}$ is a family of Lipschitz mappings on $\R^n$ such that
\begin{align}
    & \vp_t(V^2) \subset V^2 \mbox{ for all } t \in [0,1];  \label{e:vpV2a} \\
    & t \mapsto \vp_t(y) \mbox{ is continuous for all } y \in \R^n; \label{e:vpV2b} \\
    & \vp_t(y) = y \mbox{ for } t=0 \mbox{ and for } y \in \R^n \setminus V^2; \label{e:vpV2c} \\
    & \dist(\vp_t(y), E_R) < \alpha_1 \ell(R) \mbox{ for } y \in E_\rho \cap V^2 \mbox{ and all } t \in [0,1]; \label{e:vpV2d}\\
    & \vp_1(y) \in V^1 \mbox{ for } y \in E_\rho \cap V^2.\label{e:vpV2e}
\end{align}
\begin{lemma}\label{l:dF}
We have that $E_\rho \cap V^2 \in \dF$. In particular, the class $\dF$ is nonempty. 
\end{lemma}
\begin{proof}
We just take the trivial deformation $\vp_t(y)=y$ for all $y$ and $t$, so that \eqref{e:vpV2a}, \eqref{e:vpV2b} and \eqref{e:vpV2c} hold immediately. Moreover, by construction we have that all points in $E_\rho$ are contained in a cube from $\cC_{R, \rho}$. The side length of these cubes is (much) less than $\alpha_1 \ell(R)$ and they must touch $E$. Hence $\dist(y, E_R) \leq \tau \ell(R)$ and so \eqref{e:vpV2d} is satisfied. As for condition \eqref{e:vpV2e} is concerned, we see that if $y \in E_\rho \cap V^2$, then by definition of $E_\rho$ and $\cC_{R, \rho}$ in \eqref{e:E-rho} and \eqref{e:cC-R-rho}, we see that $y$ must lies in a cube which belongs to $\cC_\sigma^1(B_6)$ (from the definition of $\sigma$ in \eqref{e:sigma}), and thus it must be in $V^1$.
\end{proof}

Let now define the aforementioned functional. For some $c_2<1$ to be chosen later, we put
\begin{align}\label{e:M}
M=\frac{C_3}{c_2\,\delta_1},    
\end{align}
where recall that $C_3$ is the Ahlfors regularity constant of $E_R$ (as fixed in Notation \ref{n:C3}).
Then we set
\begin{align}\label{e:J}
    J(F) := \hd(F \cap E_\rho) + M\, \hd(F \setminus E_\rho) \mbox{ for } F \in \dF. 
\end{align}
Note that $J(F)= J(F^*)$ (with notation as in \eqref{e:F_03}), and there is only a finite number of sets like $F^*$. Thus there exists a set $\wt F \in \dF$ such that 
\begin{align*}
    J(\wt F) = \min_{F \in \dF} J(F). 
\end{align*}

Note that, for a set $F \in \dF$ trying to keep $J(F)$ small, it will be very expensive to have a large portion which does not intersect $E_\rho$, as $M$ can be quite large. This is the reason why we expect the minimiser $\wt F$ to have a large intersection with $E_\rho$. This also implies that a minimiser of $J$ also will lie close to $E_R$.
\begin{lemma} \label{l:large-intersection}
%\michele{The proof of this lemma is very similar to the one given by David (perhaps I could omit it).}
Let $\wt F$ be a minimiser of $J$ \textup{(}as in \eqref{e:J}\textup{)} in $\dF$. Then 
\begin{align} \label{e:L-Int}
    \hd(E_\rho \cap \wt F) \geq C \,\delta_1\ell(R)^d.
\end{align}
\end{lemma}
Once again, the proof below follows that of David in \cite{david04}. We include it for completeness. 
\begin{proof}
Because $\wt F \in \dF$, then $\wt F = \vp_1(E_\rho \cap V^2)$, where $\{\vp_t\}$ satisfies \eqref{e:vpV2a}-\eqref{e:vpV2e}. We want to check that this specific one parameter family $\vp_t$ satisfies also the conditions for the deformations used for STC (see Definition \ref{d:TND}). Note that  $\{\vp_t\}$ satisfies \eqref{e:vp1}, \eqref{e:vp2} and \eqref{e:vp3}, since from \eqref{e:Ta}, we have that $V^2 \subset B(x,r)$. We want to check that  \eqref{e:TND3} holds, that is, that  
\begin{align} \label{e:TND3b}
    \dist(\vp_t(y), E_R) \leq \alpha_1 \ell(R) \mbox{ for } t \in [0,1] \mbox{ and } y \in E_\rho \cap B(x,r).
\end{align}
So, let $y \in E_\rho \cap B(x,r)$. If $y \notin V^2$, then $\vp_t(y)=y$ by \eqref{e:vpV2c} and so \eqref{e:TND3} is satisfied (recall \eqref{e:rho}). If $y \in V^2 \cap E_\rho$, then by \eqref{e:vpV2e}, $\vp_t(y)$ must lie in $V^1$, and hence be at most $\sigma$ far away from $E_R$ (by construction); but $\sigma < \alpha_1 \ell(R)$, and so \eqref{e:TND3b} holds.

Thus $\{\vp_t\}$ is a one parameter family of Lipschitz deformations which satisfies the requirements stated in the definition of STC (see Definition \ref{d:TND}). Recall that $E_\rho$ to satisfies the STC (at scale $\ell(R)$); we therefore have the lower bound \eqref{e:STC-E-rho}, i.e.
\begin{align*}
    \hd(\vp_1(E_\rho \cap B(x,r))) \geq \delta_1 \ell(R)^d + \hd\ps{E_\rho \cap A_{\wt \eta_1 \ell(R)}(x,r)}.
\end{align*}
Now, the family $\{\vp_t\}$ which we are considering, not only satisfies \eqref{e:vp3}, but also \eqref{e:vpV2c}, and so, in particular, 
\begin{align*}
    \vp_1\ps{E_\rho \cap B(x,r)} & = \vp_1\ps{(V^2 \cap E_\rho) \cup (E_\rho \cap (B(x,r) \setminus V^2))}\\
    & = \vp_1(E_\rho \cap V^2) \cup \ps{E_\rho \cap (B(x,r) \setminus V^2)},
\end{align*}
recalling that by definition (see \eqref{e:Ta}) $V^2 \subset B(x,r)$. Also, note that 
\begin{align} \label{e:Ja}
    E_\rho \cap (B(x,r) \setminus V^2) \subset A_{\wt\eta_1 \ell(R)}(x,r) \cap E_\rho;
\end{align}
indeed, using  $B_6 \cap E_\rho \subset V^2$, we see that $E_\rho \cap (B(x,r) \setminus V^2) \subset E_\rho \cap (B(x,r) \setminus B_6)$, and (recalling \eqref{e:Bj}), $B(x,r) \setminus B_6 \subset A_{\wt \eta_1\ell(R)}(x,r)$. Thus we have
\begin{align*}
     \hd\ps{\vp_1(E_\rho \cap V^2)} + \hd\ps{A_{\wt \eta_1 \ell(R)}(x,r)\cap E_\rho} \geq \delta_1 \ell(R)^d + \hd\ps{E_\rho \cap A_{\wt \eta_1 \ell(R)}(x,r)}
\end{align*}
and so
\begin{align}\label{e:Jb}
    \hd\ps{\vp_1(E_\rho \cap V^2)} \geq \delta_1\ell(R)^d. 
\end{align}
In particular, from the definition of $\dF$, this inequality holds for any $F \in \dF$. 
Recall now that we decided that $\wt F$ was a minimiser of $J$ (as defined in \eqref{e:J}). Thus we have that
\begin{align}\label{e:Jc}
    & J(\wt F) \leqt{\text{Lemma } \ref{l:dF} } J(E_\rho \cap V^2) = \hd\ps{E_\rho \cap V^2}\\
    & \leqt{\eqref{e:Ta}} \hd\ps{E_\rho \cap B(x,r)} \leqt{\text{Lemma } \ref{l:Erho-ADR}} C_3 \ell(R)^d. 
\end{align}
Moreover, by definition of $J$, 
\begin{align} \label{e:Jd}
    \hd\ps{\wt F \setminus E_\rho} \leq \frac{J(\wt F)}{M} \leqt{\eqref{e:Jc}} \frac{C_3}{M}\ell(R)^d \eqt{\eqref{e:M}} c_2\,\delta_1 \ell(R)^d.
\end{align}
But then we have that 
\begin{align}
    \hd\ps{\wt F \cap E_\rho} = \hd(\wt F) - \hd(\wt F \setminus E_\rho) \geqt{\eqref{e:Jb}, \eqref{e:Jd}} \frac{\delta_1 \ell(R)^d}{2}.
\end{align}
This proves the Lemma.
\end{proof}
%\michele{So here the point is to have a minimiser that intersects (with large intersections) the our set $E_R$.}

%\michele{Write that this section is basically the same as the corresponding section in David's paper.}

==> 08b-2-AlmgrenQM.tex <==
\subsection{Almgren quasiminimality of $\wt F$.} Roughly speaking, a set $S$ in $\R^n$   is a quasiminimiser of the $d$-dimensional Hausdorff measure $\hd$ if, whenever we deform $S$ in a suitable way, the $d$-measure of such deformations does not shrink too much. Quasiminimality is a form of stability: the set maintain its Hausdorff dimension under a suitable class of perturbations. Heuristically, this is the reason why we need to transfer the topological condition from $E$ to an Ahlfors regular set: in this case, modulo technicalities, quasimininality roughly coincides with our topological condition.

We now recall from \cite{david-semmes00} the precise definitions to make this notion precise. Let $U$ be an open set in $\R^n$ and fix two constants 
\begin{align}\label{e:QMconst}
    1 \leq k < \infty \mbox{ and } 0 < \delta \leq + \infty. 
\end{align}
Let $S \subset U$ be so that
\begin{align} \label{e:QMa}
    S \neq \emptyset \mbox{ and } \overline{S} \setminus S \subset \R^n \setminus U.
\end{align}
Assume also that 
\begin{align} \label{e:QM-finite}
    \hd(S \cap B) < +\infty \mbox{ for all balls } B \subset U.     
\end{align}
Now, let us make precise what we mean by `deformations' or `perturbations'. Given a set $S$, deformations of $S$ will be sets of the form $\phi(S)$, where 
\begin{align}\label{e:QM-Lip}
    \phi: \R^n \to \R^n \mbox{ is Lipschitz }
\end{align}
and satisfies the following properties. 
\begin{align}
    & \diam\ps{ W \cup \phi(W)} \leq \delta \mbox{ where } W := \ck{ x \in \R^n \, |\, \phi(x) \neq x}; \label{e:QM-W} \\
    & \dist\ps{W \cup \phi(W) , \R^n \setminus U} > 0; \label{e:QM-dist}\\
    & \phi \mbox{ is Lipschitz-homotopic to the identity}. \label{e:QM-homo}
\end{align}
The last requirement means that there exists a continuous map 
\begin{align*}
    h : \R^n \times [0,1] \to \R^n
\end{align*}
such that $h(x, 0) = x$ and $h(x, 1) = \phi(x)$ for all $x \in \R^n$, such that $h(\cdot, t): \R^n \to \R^n$ is Lipschitz for all $t \in [0,1]$, and such that
\begin{align*}
    \diam(\widehat W) < \delta \mbox{ and } \dist( \widehat W, \R^n \setminus U ) >0,
\end{align*}
where 
\begin{align*}
    \widehat W := \bigcup_{t \in [0,1]} W_t \cup \phi_t(W_t), \enskip \phi_t(x) = h(x,t) \mbox{ and } W_t:= \ck{x \in \R^n \, |\, \phi_t(x) \neq x }.
\end{align*}

\begin{definition}
Let $0<d< n$; let $U \subset \R^n$ be an open set and fix two constant $k, \delta$ as in \eqref{e:QMconst}. We say that $S \subset U$ is a \textit{$(U, k, \delta)$-quasiminimizer} for $\hd$ if $S$ satisfies \eqref{e:QMa}, \eqref{e:QM-finite} and 
\begin{align}
    & \hd(S \cap W) \leq k \hd\ps{\phi(S \cap W)}\label{e:QMmain} \\
    & \mbox{for all Lipschitz mappings } \phi \mbox{ which satisfy } \eqref{e:QM-W}, \eqref{e:QM-dist} \mbox{ and } \eqref{e:QM-homo}.\nonumber
\end{align}
\end{definition}

\begin{lemma}\label{l:quasiS}
The set 
\begin{align}
    S:= \wt F \cap B_2
\end{align}
is a $(B_2, k, \delta)$-quasiminimizer for $\hd$, where
\begin{align}
    k = C\,4^{nd}M, 
\end{align}
(here $C$ is a geometric constant), and
\begin{align}
    \delta = c_3 \min\ck{\alpha_1, \eta_1} \ell(R).
\end{align}
Here $0< c_3<1$ is a parameter that we will fix later. 
\end{lemma}

We will need the following lemma from \cite{david04}. We tailor it to our current notation.  
\begin{lemma}[{\cite{david04}, Lemma 5.8}]\label{l:retraction}
Let $V^1$ be a finite union of dyadic cubes belonging to $\Delta_\sigma$, where $\sigma$ should be thought of as in \eqref{e:sigma}. There exists a $4^n$-Lipschitz function $h$, defined on 
\begin{align} \label{e:h1}
    V^1_+ := \ck{ y \in \R^n \,|\, \dist(y, V^1) \leq \frac{\sigma}{4}}
\end{align}
and such that
\begin{align}
    & h(V^1_+) \subset V^1 \label{e:h2}\\
    & h(y) = y \mbox{ for } y \in V^1, \label{e:h3}
\end{align}
and 
\begin{align}
    |h(y) - y| \leq n^{1/2} \sigma.
\end{align}
\end{lemma}
Recall that we want to show that $\wt F$ is a quasiminimal set for $\hd$.
Here is the idea to do so. We want to look at $\hd(\phi(\wt F \cap W))$; what we know about $\wt F$ which makes us hope that it may well be a quasiminimal set is that $\wt F$ is a minimiser of the functional $J$ as defined in \eqref{e:J}. We want to use this information. In other words, we would like to say that $\phi(\wt F)$ is a competitor of $\wt F$ belonging to the class $\dF$. Unfortunately, this is not true, in the sense that $\phi(\wt F)$ may lie outside $V^1$, and this is not permitted (see \eqref{e:vpV2e}). What we can do however, is first to retract $\phi(\wt F)$ (which we will call $F_1$) back into $V^1$ (using the map $h$ from Lemma \ref{l:retraction}); let us set $F_2:=h(F_1)$. Next, we want to project $F_2$ onto some $d$-dimensional skeleton so that it belongs to $\dF_0$ (as defined in \eqref{e:F_0}). This projection will happen in two steps, with two corresponding maps; we will denote the images so obtained by $F_3$ and then $F_4$; this latter one will be the needed competitor. The last step will be to show that these distortions of $\phi(\wt F)$ don't increase the size of $\phi(\wt F)$ too much. In this way, first by the minimising property of $\wt F$ we will obtain a bound like $\hd(\wt F) \leq M \hd(F_4) $ and then, by this last step, a bound similar to $\hd(F_4) \leq C \hd(\phi(\wt F))$ and thus establishing quasiminimality.

\subsubsection{Constuction of $F_1$ and $F_2$}
Let us get started: we want to deform $\wt F$ with Lipshitz maps $\phi$ as in \eqref{e:QM-Lip}. Pick one such Lipshitz deformation $\phi$. We are interested in those points $y \in W \cap \wt F$, i.e. those points which are actually being moved by $\phi$. But by \eqref{e:QM-W}, we must have that $|\phi(y)-y| \leq \delta$. We put
\begin{align}
    \delta= c_3 \min\ck{\alpha_1, \eta_1} \ell(R), 
\end{align}
where $c_3$ is a small parameter to be chosen soon. The rationale to choose $c_3$ is that we want $ \phi(\wt F)$ to lie in $V^1_+$, so that we may apply Lemma \ref{l:retraction} and send $\phi(\wt F)$ back into $V^1$. Recall that $V^1_+$ is the set of points lying at most $\sigma/4$ far away from $V^1$; recall also that $\wt F= \vp_1(E_\rho \cap V^2) \subset V^1$ by \eqref{e:dF} (the way $\dF$ was defined) and the property of $\{\vp_t\}$, \eqref{e:vpV2e}. Hence for an appropriate choice of $c_3$, say $c_3 = \frac{1}{300 \sqrt{n}}$ (see \eqref{e:sigma}) we have that if $y \in W \cap \wt F$, then
\begin{align}
    \phi(y) \in V^1_+.
\end{align}
We set 
\begin{align}
    & F_1 := \phi(\wt F) \mbox{ and }\label{e:F1} \\
    & F_2 := h(F_1) = h(\phi(\wt F)). \label{e:F2} 
\end{align}
In particular, $F_2 \subset  V^1$.

\subsubsection{Construction of $F_3$}
We want to project $F_2$ back into a $d$-dimensional skeleton, since this is a requirement to belong to $\dF_0$ (and so eventually to $\dF$). By definition of $\dF_0$, we will be projecting onto the $d$-skeleton of cubes coming from $\Delta_{\rho}$.   

We will use the following Lemma, which is taken from \cite{david-semmes00}.

\begin{lemma}[{Lemma 11.14, \cite{david-semmes00}.}] \label{l:FF2}
Let $j \in \Z$ and let $A$ be a compact subset of $\R^n$ such that $\hd(A)<\infty$. Denote by $N(A)$ the union of all the cubes $I \in \Delta_j$ that touch a cube in $\Delta_j$ which intersects $A$. Then there is a Lipschitz mapping $f: \R^n \to \R^n$ with the following properties.
%\michele{Need to define some notaion here}
\begin{align}
    & f(x) = x \mbox{ for } x \in \R^n \setminus N(A); \label{e:FF2a}\\
    & f(x) = x \mbox{ for all } x \in \mathcal{S}_{j,d}; \label{e:FF2b} \\
    & f(A) \subset \mathcal{S}_{j,d}; \label{e:FF2c}\\
    & f(I) \subset I \mbox{ for all } I \in \Delta_j; \label{e:FF2d} \\
    & \hd\ps{f((A \cap I) \setminus \dS_{j,d})} \leq C \,\hd\ps{(A \cap I) \setminus \dS_{j,d}} \mbox{ for all } I \in \Delta_j. \label{e:FF2e}
\end{align}
\end{lemma}
Recall the definition of $\dS_{j,d}$ in \eqref{e:Sjd}. 

We now apply Lemma \ref{l:FF2} with \begin{align*}
    j=-j(\rho) \mbox{ and } A = F_2= h(\phi(\wt F)), 
\end{align*}
and thus we set
\begin{align} \label{e:F3}
    F_3= f(F_2)= (f \circ h \circ \phi)(\wt F). 
\end{align}

\begin{remark}\label{r:rem-A}
Let us note a couple of facts. First, we see that if $y \in \wt F \setminus W$, then $\phi(y)=y$ (by definition of $W$, as in \eqref{e:QM-W}); but, still with the same $y$, also $h(\phi(y))=h(y)=y$, since $y \in V^1$ already, and $h$ does not move such points (as in \eqref{e:h3}), and further, $f(h(\phi(y)))= f(y) =y$ by \eqref{e:FF2b}, since $y \in \wt F$, and therefore it belongs to the $d$-face of some cubes from $\Delta_\rho$. 
\end{remark}
\begin{lemma}
With the notation as above,  we have
\begin{align} \label{e:dim}
    \dim \ps{F_3 \setminus \dS_{-j(\rho), d}} \leq d-1. 
\end{align}
\end{lemma}
%\michele{This proof is ok as long as $\wt F$ is coral.}
\begin{proof}
By Remark \ref{r:rem-A}, we already know that $f(h(\phi(\wt F \setminus W)))= \wt F \setminus W \subset \dS_{-j(\rho), d}$. On the other hand, we must have that $f(h(\phi(\wt F \cap W))) \subset \dS_{-j(\rho), d}$ by \eqref{e:FF2c}. Thus the Lemma follows. 
\end{proof}

\subsubsection{Construction of $F_4$ and $F_4 \in \dF$}
Note that $F_3$ is not necessarily a union of full $d$-dimensional faces: the projection $f$ is into and not necessarily onto. 
\begin{lemma}
There exists a Lipschitz map $\pi: \R^n \to \R^n$ so that $\pi(F_3)$ is precisely the union of those $d$-dimensional faces which were contained in $F_3$. 
\end{lemma}
\begin{proof}
See \cite{david04}, pages 211-212. The idea of the proof is to consider those faces $T$ which intersect $F_3$ on a set of positive $d$-dimensional measure but that are not contained in $F_3$. On these faces, exactly because they are not contained in $F_3$, we can define a Lipschitz map $\pi$ which sends whatever lies of $F_3$ in one such face to its $(d-1)$-dimensional boundary. The result, $F_4$, will be a set of full $d$-faces plus a set of dimension smaller or equal to $d-1$.
\end{proof}
We now set 
\begin{align}
    F_4 := \pi(F_3).
\end{align}
\begin{lemma}
With notation as above,
\begin{align}
    F_4 \in \dF.
\end{align}
\end{lemma}
\begin{proof}
Once again, see \cite{david04}, pages 212 to 215. 
\end{proof}
%\michele{Add some details?}
Hence $F_4$ is a valid competitor in $\dF$ of $\wt F$. But $\wt F$ is a minimiser of the functional $J$ in this class, and therefore we have the inequality
\begin{align} \label{e:F4-F}
    J(\wt F) \leq J (F_4). 
\end{align}
We will use this inequalty in the following subsection to finally prove that $\wt F$ is also a quasiminimiser of $\hd$. 

\subsubsection{$\wt F$ is a quasiminimiser}
First, note that $F_4 \subset F_3$, except perhaps from a set of dimension smaller than, or equal to, $d-1$. Thus, using also \eqref{e:F4-F}, we have that
\begin{align*}
    J(\wt F) \leq J(F_3). 
\end{align*}
Recall the definition of $W$ in \eqref{e:QM-W} and that of $J$ in \eqref{e:J}. Writing $\wt F = \ps{\wt F \cap W} \cup \ps{\wt F \setminus W}$, and using the additivity of $\hd$, we have
\begin{align}
    J(\wt F) = J(\wt F \cap W) + J(\wt F \setminus W). 
\end{align}
Let us set 
\begin{align*}
    \Phi(y) = \ps{f \circ h \circ \phi} (y).
\end{align*}
With this notation we see that $F_3= \Phi(\wt F)$ (this is just \eqref{e:F3}). Moreover, recall from Remark \ref{r:rem-A}, that $\Phi(\wt F) = \Phi(\wt F \cap W) \cup \Phi(\wt F \setminus W)$, and in turn, that $\Phi(\wt F \setminus W) = \wt F \setminus W$, and thus $J(\Phi(\wt F \setminus W)) = J(\wt F \setminus W)$, which is immediate from the definition of $J$ as in \eqref{e:J}. In particular we get that
\begin{align*}
    J(F_3) & = J(\Phi(\wt F ))  \\
    & \leq J\ps{\Phi(\wt F \cap W)} + J\ps{\Phi(\wt F \setminus W)} \\
    & = J\ps{\Phi(\wt F \cap W)} + J\ps{\wt F \setminus W}. 
\end{align*}
We thus
\begin{align*}
   J(\wt F)=  J(\wt F \cap W) + J(\wt F \setminus W) \leq J(\Phi(\wt F \cap W)) + J(\wt F \setminus W), 
\end{align*}
which, subtracting $J(\wt F \setminus W)$ from both sides, gives,
\begin{align*}
    J(\wt F \cap W) \leq J(\Phi(\wt F \cap W)).
\end{align*}
But note that, by the definition of the functional $J$ in \eqref{e:J}, \begin{align*}
    & \hd(\wt F \cap W) \leq J(\wt F \cap W) \leq J(\Phi(\wt F \cap W)) \\
    & = \hd(\Phi(\wt F \cap W)\cap E_\rho) + M \hd(\Phi(\wt F \cap W) \setminus E_\rho) \leq M \hd(\Phi(\wt F \cap W)).
\end{align*}
That is, 
\begin{align} \label{e:QMd}
    \hd(\wt F \cap W) \leq M \, \hd(\Phi(\wt F \cap W)).
\end{align}
Note that \eqref{e:QMd} resembles the comparison estimate \eqref{e:QMmain}: we need to swap $\Phi$ with $\phi$. To do so, we need to show that up constants, the maps $f$ and $h$ did not increase the mass of $\phi(\wt F \cap W)$. 
Let us worry about $f$ first. We write
\begin{align}
    & A_1 := h(\phi(\wt F \cap W)) \cap \dS_{-j(\rho),d}\,; \\
    & A_2 := h(\phi(\wt F \cap W)) \setminus \dS_{-j(\rho),d}\, .
\end{align}
Now, because $f(y) = y $ whenever $y \in \dS_{-j(\rho), d}$, we immediately have that
\begin{align} \label{e:QMi}
    \hd(f(A_1)) = \hd(A_1).
\end{align}
Let us look at $A_2$. Because of \eqref{e:FF2d} and the fact that dyadic cubes have bounded overlap, we can write
\begin{align*}
    \hd\ps{f(A_2)} \leq \sum_{I \in \Delta_{-j(\rho)}} \hd(f(A_2 \cap I)) \leq C \sum_{I \in \Delta_{-j(\rho)}} \hd(f(\overline{A_2} \cap I \setminus \dS_{-j(\rho),d} )).
\end{align*}
To estimate this last sum, we use \eqref{e:FF2e}:
\begin{align*}
   &  C \sum_{I \in \Delta_{-j(\rho)}} \hd(f( \overline{A_2} \cap I \setminus \dS_{-j(\rho),d} )) \nonumber \\
   &\leq C' \sum_{I \in \Delta_{-j(\rho)}} \hd(\overline{A_2} \cap I \setminus \dS_{-j(\rho),d})\nonumber\\
   & \leq C'\hd\ps{\overline{ h(\phi(\wt F \cap W))} \setminus \dS_{-j(\rho), d}}.
\end{align*}
Putting together these estimates, we see that
\begin{align} \label{e:QMf}
\hd(\Phi(\wt F \cap W)) \leq \hd(A_1) + C'\hd(\overline{ h(\phi(\wt F \cap W))} \setminus \dS_{-j(\rho), d}).
\end{align}
\begin{lemma}
With the notation as above, we have
\begin{align} \label{e:QMg}
    \dim\ps{\overline{h(\phi(\wt F \cap W))} \setminus (h(\phi(\wt F \cap W)) \cup \dS_{-j(\rho), d})} \leq d-1.
\end{align}
\end{lemma}
\begin{proof}
See the proof of equation 5.60 in \cite{david04}.
\end{proof}
Using \eqref{e:QMg}, we then can write
\begin{align}
    & \hd(A_1) + C' \hd(\overline{h(\phi(\wt F \cap W))} \setminus \dS_{-j(\rho),d}) \nonumber\\
    &
    \leq \hd(A_1) + C' \hd(h(\phi(\wt F \cap W)) \setminus \dS_{-j(\rho),d}\nonumber \\
    & = \hd(A_1) + C' \hd(A_2) \nonumber\\
    & \leq C' \hd(h(\phi(\wt F \cap W))).  \label{e:QMh}
\end{align}
Hence, \eqref{e:QMf} and \eqref{e:QMh} tell us that
\begin{align} \label{e:QMm}
     \hd(\Phi(\wt F \cap W)) \leq C'\hd(h(\phi(\wt F \cap W))).
\end{align}
Now note that because $\pi$ is Lipschtz with constant $4^n$ as for Lemma \ref{l:retraction}, we immediately see that
\begin{align} \label{e:QMl}
    \hd(h \circ \phi(\wt F \cap W)) \leq 4^{nd}\hd(\phi(\wt F \cap W)).
\end{align}
The two estimates \eqref{e:QMm} and \eqref{e:QMl} together show that $\wt F \cap B_2$ is a $(B_2, k, \delta)$-quasiminimal set (with $B_2$ as defined in \eqref{e:Bj}, $k= 4^{nd} C' M$ and $$\delta= c_3 \min\ck{\alpha_1, \eta_1} \ell(R).$$





==> 08c-2-URofF.tex <==
\subsection{A uniformly rectifiable set covering the minimising set $\wt F$.}
In this short subsection, we will use the main result of \cite{david-semmes00}, to show that $\wt F$ can be locally covered by a uniformly rectifiable set.
\begin{lemma}\label{l:UR-cover}
With notation as above \textup{(}in particular recall the definition of $B_1$ in \eqref{e:Bj}\textup{)}, we have that
\begin{align*}
    \wt F \cap B_1 \subset Z, 
\end{align*}
where $Z$ is a uniformly $d$-rectifiable set. 
\end{lemma}

Let us recall the main result in \cite{david-semmes00}. 
\begin{theorem}[{\cite{david-semmes00}, Theorem 2.11}] \label{t:UR}
    Let $U$ be an open set in $\R^n$, and suppose that $S$ is a $(U, k, \delta)$-quasiminimizer for $\hd$. Let $S^*$ be the support in $U$ of the restriction of $\hd$ to $S$. Then for each $x \in S^*$ and radius $R_0$ which satisfy
    \begin{align}
        0<R_0< \delta \mbox{ and } B(x, 3R_0) \subset U,
    \end{align}
    there is a compact, Ahlfors $d$-regular set $Z$ such that
    \begin{align}
        S^* \cap B(x,R_0) \subset Z \subset S^* \cap B(x,2R_0)
    \end{align}
    and
    \begin{align}
        Z \mbox{ is uniformly rectifiable and contains big pieces of Lipschitz graphs.}
    \end{align}
    The constants for the Ahlfors regularity and for the uniform rectifiability of $Z$ depend only on $n$ and $k$.
\end{theorem}
\begin{proof}[Proof of Lemma \ref{l:UR-cover}]
Recall that $\wt F$ is a minimiser of the functional $J$ over $\dF$, see definitions \eqref{e:J} and \eqref{e:dF}.
By Lemma \ref{l:quasiS}, we know that $S= \wt F \cap B_2$ is a $(B_2, k, \delta)$-quasiminimizer for $\hd$. Also recall that
\begin{align*}
    B_2=B\ps{x, r- \frac{8}{10} \eta_1 \ell(R) } \mbox{ (see \eqref{e:Bj})},
\end{align*}
that $k = C4^{nd}M$, and $\delta= c_3 \min\{\alpha_1, \eta_1\} \ell(R)$. Then, making $c_3$ smaller if needed, we see that for all points $y \in \wt F \cap B_1$, we have 
\begin{align}
    B(y, 3\delta) \cap \wt F^* \subset B_2,
\end{align}
where recall that $\wt F^*$ is the coral part of $\wt F$ (see \eqref{e:F_03}).
By Theorem \ref{t:UR}, we see that there exists a uniformly rectifiable set $Z_y$ so that
\begin{align} \label{e:Zy}
    \wt F^* \cap B(y, \delta/2) \subset Z_y \subset \wt F^* \cap B(y, \delta),
\end{align}
since we can chose $R_0 \geq \delta/2$.
Now, clearly
\begin{align*}
    \bigcup_{y \in B_1\cap \wt F} B(y, \delta/2) \supset \wt F \cap B_1. 
\end{align*}
Moreover, we can find a finite subfamily of balls $\{B(y_j, \delta/2)\}_{j=0}^N$ such that
\begin{align}\label{e:fin-balls}
    \wt F \cap B_1 \subset \bigcup_{i=0}^N B(y_i, \delta/2) 
\end{align}
and 
\begin{align*}
    N \leq C = C(n, \eta_1). 
\end{align*}
To see this, recall that $r(B_1)= r-9/10\eta_1 \ell(R)$. This, by the choice of $r=r_2$ in \eqref{e:TND-r_2}, and choosing the constant $C$ in \eqref{e:eta} appropriately, gives that $r(B_1) \leq \ell(R)/2$. Hence, since $\delta=c_3\min\{\alpha_1, \eta_1\}$, we need at most $C$ balls in \eqref{e:fin-balls}, where $C$ depends only on $n, \alpha_1$ and $ \eta_1$. Now, for this each one of these balls, we take the corresponding uniformly rectifiable set $Z_{y_i}$ as in \eqref{e:Zy}, and we set
\begin{align}\label{e:Zx}
    Z_x := \bigcup_{i=0}^N Z_{y_i}.
\end{align}
Then $Z_x$ is a uniformly rectifiable set (with uniform constant now depending on $N$, and thus $\alpha_1$ and $\eta_1$) so that
\begin{align*}
    \wt F^* \cap B_1 \subset \bigcup_{i=0}^N B(y_i, \delta/2) \cap \wt F^* \subset \bigcup_{i=0}^N Z_{y_i} = Z_x. 
\end{align*}
This proves the lemma. 
\end{proof}

\begin{remark}
A short summary of what has been done so far will be useful to the reader in the subsequent section. 

We started off with a surface $E$ satisfying the topological condition \eqref{e:TC} with some prescribed parameters $r_0,\, \alpha_0, \, \eta_0$ and $\delta_0$. We took the corona construction from Lemma \ref{l:corona}, and we showed that TC on $E$ implies a skeletal topological condition on all the approximating $E_R$ in the coronisation (Section \ref{s:TC-STC}, Lemma \ref{l:TC-STC}). Next, we constructed a further approximating Ahlfors regular set $E_{R, \rho}$ (see \eqref{e:E-rho}), to then show that \textit{for any point} $x \in R$ (see the choice of $x_2$ in \eqref{e:TND-x}), there is a $(B_2, k, \delta)$-quasiminimiser set $\wt F= \wt F(R, x)$ such that, first, 
\begin{align} \label{e:wtF-Erho}
    \hd(\wt F \setminus E_\rho) \leq c_2 \delta_1 \ell(R)^d,
\end{align}
| this is equation \eqref{e:Jd}); and second, that there exists a uniformly $d$-rectifiable set $Z_x$ so that
\begin{align} \label{e:B1F-Zx}
    B_1 \cap \wt F^* \subset Z_x;
\end{align}
| this is Lemma \ref{l:UR-cover}.
\end{remark}
\begin{lemma} \label{l:UR-large-int}
Let $R \in \Top(k_0)$. Then there exists a uniformly $d$-rectifiable set $Z_R$ and a set $\wt F_R$ which is a the union of a uniformly finite family of quasiminimal sets so that, 
\begin{align} \label{e:UR-largint-1}
    \hd(\wt F_R \cap E_{R, \rho}) \geq \delta_0 \ell(R)^d,
\end{align}
and,
\begin{align} \label{e:UR-largint-2}
    \hd(\wt F_R \setminus E_{R, \rho}) \leq c_2 \delta_1 \ell(R)^d;
\end{align}
and,
\begin{align} \label{e:UR-largint-3}
     \wt F_R \subset Z_R.
\end{align}
\end{lemma}
\begin{proof}

Now, recall from \eqref{e:Bj}, that 
\begin{align*}
    B_1 = B\ps{x_2, r_2 - \frac{9}{10} \eta_1 \ell(R)},
\end{align*}
and also recall from \eqref{e:r-R}, that $r_2 > \eta_1 \ell(R)$. In particular we have that
\begin{align*}
    B(x, \eta_1\ell(R)/10) \subset B_1.
\end{align*}
Note that to cover $R$, we need at most $N'\sim_n \eta_1^{-n}$ balls centered on $R$ and with radius $\eta_1 \ell(R)/10$. Pick one such collection that is also minimal, and thus of bounded overlap. Let it be
\begin{align*}
    B^j := B(x_j, \eta_1 \ell(R)/10), \, x_j \in R, \, 1 \leq j \leq N'. 
\end{align*}
For each $1\leq j \leq N'$, there correspond a quasiminimal set $\wt F=\wt F(R, x_j)$ (and its coral part $\wt F^*$) satisfying \eqref{e:wtF-Erho}, and a corresponding uniformly $d$-rectifiable set $Z_{x_j}$ satisfying \eqref{e:B1F-Zx}.
We now set 
\begin{align}
    \wt F_R := \bigcup_{j=1}^{N'} \wt F(R, x_j),
\end{align}
and
\begin{align}
    Z_R := \bigcup_{j=1}^{N'} Z_{x_j}
\end{align}
It is then easy to see that \eqref{e:UR-largint-1}, \eqref{e:UR-largint-2} and \eqref{e:UR-largint-3} hold.

\end{proof}
\begin{corollary}
For $R \in \Top(k_0)$, let $Q \in \Tree(R)$. Then there exists a uniformly $d$-rectifiable set $Z_Q$ and a set $\wt F_Q$ which is the union of a uniformly finite family of quasiminimal sets so that $\hd(\wt F_Q \cap E_{R, \rho}) \geq \delta_0 \ell(Q)^d$, $\hd(\wt F_Q \setminus E_{R, \rho}) \leq c_2 \delta_1 \ell(Q)^d$ and $\wt F_Q \subset Z_Q$.
\end{corollary}
This follows immediately from the arguments that lead to the previous lemma. Indeed, the only property of $R$ that was used to show the existence of the quasiminimiser $\wt F_R$ was that $R$ satisfied the STC. However, any $Q \in \Tree(R)$ satisfies the same property, hence the Corollary. 
%\michele{\textbf{To Jonas:} I will change the quasiminimal arguments above so that this corollary is actually proven - it will be just a change of notation.}
\begin{lemma}
For each pair $(x,r) \in E_{R,\rho} \times (0, \ell(R))$, there exists a uniformly $d$-rectifiable set $Z_{x,r}$ such that 
\begin{align*}
    \hd(E_{R,\rho} \cap Z_{x,r} \cap B(x,r)) \geq \delta_0 r^d.
\end{align*}
The Ahlfors regularity,  uniform rectifiability and BPLG constants for the sets $Z_{x,r}$ are uniform in $(x,r)$.
\end{lemma}
\begin{proof}
If $x \in E_\rho$, then by the construction of $E_\rho$ (as in \eqref{e:cC-R-rho} and  \eqref{e:E-rho}), there exists a dyadic cube $I \in \cC_R$ such that $\dist(x, \partial_d I) < \ell(I)$. Recall also that for each $I \in \cC_R$, there exists a surface cube $Q_I \in \Tree(R)$ such that $\dist(Q_I, I) \leq c \tau^{-1} \ell(I)$ and $\ell(I) \leq \ell(Q_I) \leq c' \tau^{-1} \ell(I)$. This cube is given by Lemma \ref{l:I-QI}.

Now, take two constants $C$, $C'$ to be fixed below, depending on the constants $c, c'$.
\begin{enumerate}
    \item Suppose first that \begin{align*}
        C\tau^{-1}\ell(I) \leq r \leq C' \ell(Q_I).
    \end{align*}
    Choosing $C$ appropriately, we can insure that
    \begin{align*}
        B(x,r) \supset B_{Q_I}.
    \end{align*}
    But from Lemma \ref{l:UR-large-int}, we know that $$\hd(E_\rho \cap Z_{Q_I}) = \hd(E_\rho \cap Z_{Q_I} \cap B(x,r)) \geq \delta_1 \ell(Q)^d.$$ 
    Since $r \sim \ell(Q_I)$, where the constants behind $\sim$ depend on $C,C', c, c'$, then we conclude that there is an absolute constant $C''$ so that
    \begin{align*}
        \hd(E_\rho \cap Z_{Q_I} \cap B(x,r) ) \geq C'' \delta_0 r^d.
    \end{align*}
    This give the Lemma for this case.
     \item Suppose now that
     \begin{align*}
         0< r < C \tau^{-1} \ell(I). 
     \end{align*}
     Let $T$ be a $d$-face of $\partial_d I$, and let $T(r)$ be tile of $T$ containing $x$ and with
     
     \begin{align*}
         \ell(T(r)) \sim \min\ck{\frac{1}{10}r, \ell(I)}.
     \end{align*}
     Then clearly, 
     \begin{align*}
         T(r) \subset E_\rho \cap B(x,r) \mbox{ for all } r>0,
     \end{align*}
     and $T(r)$ is a uniform rectifiable set with constants independent of $r$. Now, note that if $C \tau^{-1} > r>\ell(I)$, 
     then 
     \begin{align*}
         \hd(E_\rho \cap T(r) \cap B(x,r)) \geq \hd(T(r)) = c \ell(I)^d \sim_{\tau, C, C'} r^d.
     \end{align*}
     On the other hand, if $0<r< \ell(I)$, we have
     \begin{align*}
         \hd(E_\rho \cap B(x,r) \cap T(r)) \geq \hd(T(r)) = c r^d.
     \end{align*}
     In any case, we found a unifromly rectifiable set which intersects $E_\rho$ with measure bounded below uniformly. This gives the Lemma in this case.
     \item Now, if $C' \ell(Q_I) < r < \ell(R)$, we can repeat the arguments of point (1) for some parent of $Q_I$ appropriately chosen. By construction, this parent will be belong to $\Tree(R)$, and thus the same estimates apply.
\end{enumerate}
\end{proof}
From the theory of uniformly rectifiable sets (see \cite{david-semmes93}), we deduce the following.
\begin{corollary}\label{c:UR-Erho}
With notation as above, $E_\rho = E_{R, \rho}$ is a uniformly $d$-rectifiable set with Ahlfors regularity, uniform rectifiability and BPLG constants dependent only on those of the intersecting UR sets $Z_{x,r}$.  
\end{corollary}

For future use, let us pin down an easy fact about the distance between $R \subset E$ and $E_{\rho}= E_{R, \rho}$. 
\begin{lemma}\label{l:Erho-dist}
For each $x \in S$, with $S \in \Stop(R)$, we have
\begin{align*}
    \dist(x, E_\rho) \leq C \ell(S). 
\end{align*}
\begin{proof}
Using again Lemma \ref{l:meta1}, we see that if $S \in \Stop(R)$, then there exists a cube $I_S \in \cC_R$ such that $\zeta_S \in I_S$ and $\ell(S) \sim \tau^{-1} \ell(I_S)$. Thus in particula, if $x \in S$, then $\dist(x, E_R) \lesssim \ell(S) \sim \tau^{-1} \ell(I_S)$. Further, by construction of $E_\rho=E_{R, \rho}$, we have that $E_R \subset E_\rho$. This proves the Lemma. 
\end{proof}
\end{lemma}

==> 09-2-beta-est.tex <==




\section{Estimates on the $\beta$ coefficients and the end of the proof} \label{s:beta-end}
In this section we give the final estimates on the Jones' $\beta$ coefficient which will prove Theorem \ref{t:main}.

Recall the notation $\dD(k_0)$ from Lemma \ref{l:corona}. Theorem \ref{t:main} will easily follow from the Lemma below.
\begin{lemma} \label{lemma:upper_beta_est}
Let $p=p(d)$ be as in \eqref{e:pd} and fix an arbitrary (but sufficiently large) integer $k_0>0$.
There exists a constant $C_0 \geq 1$ (independent of $k_0$) so that, with the above notation, 
\begin{align} \label{e:upper_beta_est}
    \sum_{\substack{Q \subset Q_0\\ Q \in \dD(k_0)}} \beta_E^{p,d}(C_0Q)^2\ell(Q)^d \leq C \hd(E \cap B_{Q_0}),
    \end{align}
where $C$ depends on $n, d$, but not on $k_0$. 
\end{lemma}

We will use the following lemma.
\begin{lemma}[{[AS1], Lemma 2.21}] \label{lemma:azzamschul}
Let $1 \leq p < \infty$ and $E_1, E_2 \subset \R^n$. Let $x \in E_1$ and fix $r>0$. Take some $y \in E_2$ so that $B(x,t) \subset B(y, 2t)$. Assume that $E_1, E_2$ are both lower content $d$-regular. Then
\begin{align*}
    \beta_{E_1}^{p,d} (x,t) \lesssim_c \beta_{E_2}^{p,d} (y, 2t) + \left( \frac{1}{t^d} \int_{E_1 \cap B(x, 2t)} \left(\frac{\dist (y, E_2)}{t} \right)^p \, d \hdc(y)\right)^{\frac{1}{p}}.
\end{align*}
\end{lemma}

Let us now get started. Recall that the definition of $\Forest(R)$ in \eqref{e:forest}.
\begin{sublemma} \label{lemma:betatree}
Let $p=p(d)$ be as in \eqref{e:pd} and fix an arbitrary integer $k_0>0$.
There exists a constant $C_0 \geq 1$ \textup{(}independent of $k_0$\textup{)} so that, with the above notation,
\begin{align} 
    \sum_{\substack{Q \in \Tree(R)\\ Q \in \dD(k_0)}} \beta_{E}^{p,d}(C_0Q)^2 \ell(Q)^d & \lesssim  \ell(R)^d,
\end{align}
where the constant behind the symbol $\lesssim$ depends on $n, d, C_0$, and the Ahlfors regularity constant of $E_R$, but not on $k_0$. 
\end{sublemma}



\begin{sublemma}\label{sl:treesum}
Let $R \in \Top(k_0)$. Then 
\begin{align}\label{e:treetilde}
    \sum_{P \in  \Tree(R)} \beta_E^{p, d}(P)^2 \ell(P)^d \lesssim \ell(R)^d.
\end{align}
\end{sublemma}
\begin{proof}
We want to apply Lemma \ref{lemma:azzamschul} with $E_1=E$ and $E_2 = E_{R, \rho}$. 
For $Q \in \dD$, recall that $\zeta_Q$ denotes the center of $Q$. By the definition of $ \Forest(R)$, we see that if $Q \in \Forest(R)$, then there must exists a dyadic cube $I \in \cC_R$ which meets $Q$. The $d$-skeleton $\partial_d I$ of $I$ is part of $E_{R, \rho}$. We see that $\ell(I) \lesssim \tau \ell(Q)$. Hence there exists a point $x_Q' \in E_{R, \rho}$ such that $|x_Q - x_Q'| \leq 4 \tau \ell(Q)$, and we obtain that
\begin{align*}
    B_Q := B(x_Q, \ell(Q)) \subset B(x_Q', 2 \ell(Q))=: B_Q'.
\end{align*}
 This implies that for each cube $Q \in  \Forest(R)$ the hypotheses of Lemma \ref{lemma:azzamschul} are satisfied (with $E_1 = E$ and $E_2 = E_{R, \rho}$); we may then write
\begin{align*}
    \sum_{\substack{P \in \Tree(R)\\ P \in \dD(k_0)}} \beta_{E}^{p, d} (C_0B_P)^2 \ell(P)^d  \lesssim \sum_{\substack{P \in \Tree(R)\\ P \in \dD(k_0)}} \beta_{E_{R, \rho}}^{p,d} (2C_0B'_P)^2 \, \ell(P)^d \\
    + \sum_{\substack{P \in  \Tree(R)\\ P \in \dD(k_0)}} \ps{\frac{1}{\ell(P)^d} \int_{2C_0 B_P\cap E} \ps{\frac{\dist(y, E_{R, \rho})}{\ell(P)}}^p \, d \hdc(y) }^{\frac{2}{p}}\, \ell(P)^d \\
    & := I_1 + I_2.
\end{align*}
First, let us look at $I_1$. We apply Theorem \ref{t:Christ} to $E_{R,\rho}$; let us denote the cubes so obtained by $\dD_{E_{R,\rho}}$. Note that for each $P \in \Forest(R)$ with $P \in \dD(k_0)$, $x_P'$ belongs to some cube $ P' \in \dD_{E_{R, \rho}}$ so that $\ell(P') \sim \ell(P)$; hence there exists a constant $C_4 \geq 1$ so that 
\begin{align*}
    2C_0 B'_P \subset C_4B_{P'}.
\end{align*}
This in turn implies that $\beta_{E_{R,\rho}}^{p,d}(2C_0 B'_P) \lesssim_{p,n,d,C_0,C_4} \beta_{E_{R,\rho}}^{p,d}(C_4 B_{P'})$. Hence, 
\begin{align}
    \sum_{\substack{ P \in \Tree(R) \\ P \in \dD(k_0)}} \beta_{E_{R,\rho}}^{p,d} (2C_0 B'_P)^2 \ell(P)^d \lesssim_{p,n,d,C_0, C_1} \sum_{\substack{P' \in \dD_{E_{R,\rho}} \\ \ell(P') \lesssim \ell(R) }} \beta_{E_{R,\rho}}^{p,d} (C_4 B_{P'})^2 \ell(P')^d. 
\end{align}
Since $E_{R,\rho}$ is uniformly rectifiable (by Corollary \ref{c:UR-Erho}), we immediately have that $I_1 \lesssim \ell(R)^d$. 
Let us now estimate $I_2$. 
 Now
let $y \in 2C_0R$; by Lemma \ref{l:Erho-dist}, there exists a cube $S \in \Stop(R)$ such that 
\begin{align} \label{eq:SS_distyER}
    \dist(y, E_{R,\rho}) \lesssim \ell(S);
\end{align}
We can estimate the integral in $I_2$ with \eqref{eq:SS_distyER} as follows.
\begin{align*}
    \int_{2C_0 B_P\cap E} \ps{\frac{\dist(y, E_{R,\rho})}{\ell(P)}}^p \, d \hdc(y) & \leq \sum_{P' \in \dN(P)} \int_{P'} \ps{\frac{\dist(y, E_{R,\rho})}{\ell(P)}}^p \, d \hdc(y)\\
   &  \lesssim \sum_{P' \in \dN(P)} \sum_{\substack{S \in \Stop(R) \\ S \subset P' }} \int_{S} \frac{\ell(S)^p}{\ell(P)^p}  \\
    & \lesssim \sum_{P' \in \dN(P)} \sum_{\substack{S \in \Stop(R) \\ S \subset P' }} \frac{ \ell(S)^{d+p}}{\ell(P)^{p}},
\end{align*}
and so 
\begin{align*}
    I_2 \lesssim \sum_{\substack{P \in \Tree(R)\\ P \in \dD(k_0)}}
    \sum_{P' \in \dN(P)} \sum_{\substack{S \in \Stop(R) \\ S \subset P' }} \frac{\ell(S)^{\frac{2d}{p} + 2}}{\ell(P)^{d(\frac{2}{p}-1) + 2}}.
\end{align*}
We now swap the sums (which are all finite), to obtain that
\begin{align}
    I_2 & \lesssim \sum_{\substack{S \in \Stop(R)}}  \ell(S)^{\frac{2d}{p} + 2} \sum_{\substack{P \in  \Tree(R) \\ \exists P' \in \dN(P):\, P' \supset S}}  \frac{1}{\ell(P)^{d(\frac{2}{p}-1) + 2}}\nonumber  \\
    & \lesssim_{d,n} \sum_{\substack{S \in \Stop(R)}} \ell(S)^{\frac{2d}{p} + 2} \sum_{\substack{P \in  \Tree(R) \\ \exists P' \in \dN(P):\, P' \supset Q}} \frac{1}{\ell(P)^{d(\frac{2}{p}-1) + 2}}. \label{e:estBeta1}
\end{align}
We see that the number of cubes $P \in  \Tree(R)$ of a given generation so that there exists a sibling $P' \in \dN(P)$ for which $P' \supset S$ is bounded above by a universal constant depending on $n$ and $C_0$. Thus 
 we can sum geometrically the interior series:
\begin{align*}
    \sum_{\substack{P \in  \Tree(R) \\ \exists P' \in \dN(P):\, P' \supset Q}} \frac{1}{\ell(P)^{d(\frac{2}{p}-1) + 2}} \lesssim_{n} \frac{1}{\ell(S)^{d(\frac{2}{p}-1) +2}}. 
\end{align*}
Therefore we obtain 
\begin{align*}
    \eqref{e:estBeta1} \lesssim \sum_{\substack{S \in \Stop(R) }}  \frac{\ell(S)^{d(\frac{2}{p}) +2 }}{\ell(S)^{d(\frac{2}{p}-1) + 2}} = \sum_{\substack{S \in \Stop(R)}} \ell(S)^d.
\end{align*}
This latter sum is bounded above by $C \ell(R)^d$. This concludes the proof of the lemma.
\end{proof}




\begin{proof}[Proof of Lemma \ref{lemma:upper_beta_est}]
Let $Q_0$ as above and let $R_0$ be the minimal cube in $\Top(Q_0)$ so that $Q_0 \subset R_0$. Then we write 
\begin{align}
    \sum_{\substack{Q \subset Q_0\\ Q \in \dD(k_0)}} \beta_E^{p,d}(C_0Q)^2 \ell(Q)^d & \lesssim \sum_{\substack{R \in \Top \\ R \subset Q_0}} \sum_{\substack{Q \in \Tree(R)\\ Q \in \dD(k_0)}} \beta_{E}^{p,d}(C_0Q)^2\ell(Q)^d \\
    & \enskip \enskip + \sum_{\substack{Q \in \Tree(R_0) \\ Q \subset Q_0 \\ Q\in \dD(k_0)}}  \beta_{E}^{p,d}(C_0 Q)^2\ell(Q)^d =: \Sigma_1 + \Sigma_2.
\end{align}
First, let us look at $\Sigma_2$: by the same argument of Lemma \ref{lemma:betatree}, we see that this sum is bound above by $\ell(Q_0)^d$. On the other hand, by Lemma \ref{lemma:betatree}, we see that 
\begin{align}
    \Sigma_1 \lesssim \sum_{\substack{R \in \Top \\ R \subset Q_0}} \ell(R)^d. 
\end{align}
Note that each $R \in \Top$ is the child of some stopped cube $R'$. Recall we stopped at a surface cube $R' \in \mathcal{D}$ whenever it happened that $R' \cap I$ and $\ell(I) \sim \ell(Q)$ for some $I \in \Badsh{}$. We can therefore associate to each $R \in \Top$ a bad dyadic cube $I$, and thus, by \eqref{e:Bad-est}, we have that
\begin{align}
    \sum_{\substack{R \in \Top  \\ R \subset Q_0}} \ell(R)^d \lesssim \sum_{\substack{I \in \Badsh{}\\ I \subset B_{Q_0}}} \ell(I)^d \lesssim \hd(E\cap B_{Q_0}).
\end{align}
The estimate in \eqref{e:Bad-est} is independent of $k_0$, so is the one we obtained here.
All in all, we see that, by lower $d$-regularity, 
\begin{align*}
    \Sigma_1 + \Sigma_2 \lesssim \ell(Q_0)^d + \hd(E \cap B_{Q_0}) \lesssim  \hd(E \cap B_{Q_0}).
\end{align*}

This concludes the proof of Lemma \ref{lemma:upper_beta_est}.
\end{proof}

\begin{remark} \label{rem:k0}
Note that the estimate in \eqref{e:upper_beta_est} is independent of $k_0$, and therefore holds for all $k_0 \in \mathbb{N}$. Hence we can sum over all cubes $Q \subset Q_0$ and we have the estimate
\begin{align} \label{e:k0}
    \sum_{Q \subset Q_0} \beta_E^{p, d}(C_0 Q)^2 \ell(Q)^d \lesssim C(n,d, C_0) \hd(E \cap B_{Q_0}).
\end{align}
\end{remark}

It follows from Theorem I in \cite{azzam-schul18} that 
\begin{align}
    \hd(E\cap B_{Q_0}) \lesssim 1+\sum_{\substack{Q \in \dD \\ Q \subset Q_0}} \beta_{E}^{d,p}(C_0 Q)^{2}\diam(Q)^{d}
\end{align}
This completes the proof of Corollary \ref{cor:main}.


==> 10-2-surface.tex <==
\section{Covering by stable surfaces} \label{s:Sigma}
In this section, we show that for any set $E$ which is lower content $d$-regular, there exists a stable $d$-surface $\Sigma$ such that $\Sigma \supset E$. In other words, we prove Corollary \ref{c:TST-lcr-stable}, which we rewrite here for convenience. 
\begin{corollary}
Let $E \subset \R^n$ be a lower content \textup{(}$d, \cc_1$\textup{)}-regular set. Let $Q_0 \in \dD$. For two parameter $0< \ve, \kappa< 1$, there exists a set $\Sigma= \Sigma(Q_0, \ve, \kappa)$ such that
\begin{enumerate}[leftmargin=1cm, label=\textup{(}\textup{\arabic*}\textup{)}] 
    \item $Q_0 \subset \Sigma$. 
    \item $\Sigma$ is a stable  $d$-surface with parameters  $r_0= \diam(Q_0)/2$,  $0< \eta_0 < 1/100$  and  $\alpha_0, \, \delta_0$  sufficiently small with respect to   $\ve$  and $
    \kappa$.  
    \item We have the estimate 
    \begin{align}
        {\rm diameter}(Q_0)^d + {\rm BETA}(Q_0)  \approx \hd(\Sigma),
    \end{align}
    where ${\rm BETA}(Q_0)$ is as in \eqref{e:BETA}
\end{enumerate}
\michele{Add constants dependence}
\end{corollary}

%Fix two parameters $\ve>0$ and $\tau>0$ and let $E \subset \R^n$ be a lower content $d$-regular set (with constant $c_0$). For a given integer $k_0 \in \N$, consider $\Top(k_0)$, that is, the coronisation of $E$ by Ahlfors regular set guaranteed by Lemma \ref{l:corona}. For each $R \in \Top(k_0)$, we run a stopping time within each $\Tree(R)$, as it was done is Section 10. However, we now change the stopping criterion, and we stop whenever a cube cannot be well approximated by $d$-dimensional planes. 
\noindent
Let us briefly sketch this construction. Fix Let $Q_0 \in \dD$ be a chosen Christ-David cube (if $E$ is bounded we can let $E=Q_0$). For two constants $\ve>0$ and $\Cc_0>1$, put
\begin{align*}
    & \BWGL(Q_0)= \BWGL(Q_0, \Cc_0, \ve) := \ck{ Q \in \dD(Q_0) \, |\, d_{\Cc_0 B_Q} (Q,L)> \ve \, \mbox{ for all } d-\mbox{planes} }.
    %\\
    %& \gBWGL(Q_0) = \gBWGL(Q_0, \Cc_0, \ve):= \dD(Q_0) \setminus \BWGL(Q_0). 
\end{align*}
\noindent
Pick now a further parameter $\kappa>0$ to be fixed below. If $Q \in \BWGL(Q_0)$, we find an integer $k(Q) \in \N$, so that $\frac{1}{2} \kappa \ell(Q) \leq 2^{-k(Q)} \leq 2 \kappa \ell(Q)$. We then set 
\begin{align*}
    \dS(Q):= \ck{ I \in \Delta_{k(Q)} \, |\, I \cap Q \neq \emptyset}, 
\end{align*}
and 
\begin{align*}
    E_Q := \bigcup_{I \in \dS(Q)} \partial_d I. 
\end{align*}
It is immediate that $E_Q$ is Ahlfors regular, with constants depending on $n$ and $\kappa$. 
We now define the covering surface: we put
\begin{align}
\label{e:Sigma} 
\Sigma = \Sigma(\ve, \kappa, Q_0) := Q_0 \cup \ps{ \bigcup_{Q \in \BWGL(Q_0)}  E_Q }.
\end{align}
%\begin{remark}
%Let us quickly remark that the surface constructed in \eqref{e:Sigma}\label{rem:Sigma-BAUP} satisfies the following. For some fixed $\ve>0$ and $\Cc_0>1$, we have that for each $x \in \Sigma$ and for each $0<r< \diam(\Sigma)/\Cc_0$, it holds that either there exists a plane $P_{x,r}$ with 
%$d_{x, Ar}(\Sigma, P) < \ve$ or there exists a family $\dF= \dF(x,r)$ of $d$-dimensional planes so that 
%$d_{x,Ar}\ps{\cup_{P \in \dF} P, \Sigma}< \ve$. This follows immediately by the construction of $\Sigma$.
%\end{remark}

\begin{lemma}\label{l:hd-Sigma-up}
Let $\Sigma= \Sigma(\ve, \kappa, Q_0)$ be as defined in \eqref{e:Sigma}. Then we have that
\begin{align*}
    \hd(\Sigma) \lesssim_{\cc_1, n,d} \, \hd(Q_0) + {\rm BWGL}(Q_0, \ve, \Cc_0). 
\end{align*}
\end{lemma}
\noindent
Recall the definition of ${\rm BWGL}(Q_0, \ve, \Cc_0)$ in \eqref{e:BWGL}.
\begin{proof}
 We have that
\begin{align*}
    \hd(\Sigma) & \leq \hd(Q_0) + \hd\ps{\bigcup_{Q \in \BWGL(Q_0)} E_Q} \\
    & \leq \hd(Q_0) + \sum_{Q \in \BWGL(Q_0)} \hd(E_Q) \\
    & \lesssim_{n,d, \kappa}   \hd(Q_0) +   \sum_{Q \in \BWGL(Q_0)} \ell(Q)^d.
\end{align*}
By definition
\begin{align*}
    \sum_{Q \in \BWGL(Q_0)} \ell(Q)^d = {\rm BWGL}(Q_0, \ve, \Cc_0).
\end{align*}
\end{proof}

\begin{lemma}\label{l:Sigma-TC}
Let $\ve, \kappa$ be positive \textup{(}small\textup{)} parameters. Then $\Sigma= \Sigma(\ve, \kappa)$ satisfies the topological condition \eqref{e:TC} with constants $r_0= \diam(\Sigma)/2\approx \diam(E)$, $0< \eta_0 < 1/100$ and $\alpha_0$ and $\delta_0$ sufficiently small depending only on $\ve, \kappa$.
\end{lemma}

\begin{proof}
Let $\Sigma$ be defined as in \eqref{e:Sigma}. We want to find parameter $r_0, \alpha_0, \delta_0$ and $\eta_0$ so that for all $\alpha_0$-ALD $\{\varphi_t\}$ and for all $x_0 \in \Sigma$ and $0<r<r_0$, we have that
\begin{align*}
    \hd(B(x, (1-\eta_0)r) \cap \varphi_1(\Sigma)) \geq \delta_0 r^d. 
\end{align*}
We immediately choose
\begin{align*}
    r_0 = \diam(\Sigma)/2.
\end{align*}
\noindent
Now, let $(x, r) \in \Sigma \times (0, r_0)$. Moreover, let $\delta_0$, $\alpha_0$ and $\eta_0$ be positive parameters to be fixed below.  We consider two separate cases. 
\begin{itemize}[leftmargin=0.5cm]
\item 
\underline{Case 1.}  Suppose first that $x \in E$. Let $\kappa_1>0$ be a parameter to be fixed below. Then there is a cube $Q_{x,r} \in \dD$ such that 
\begin{align}\label{e:Qxr-ball}
    & 10^{-3} \lambda \kappa_1 r \leq \ell(Q_{x,r}) \leq \kappa_1 r, \mbox{ and }
    B_{Q_{x,r}} \subset B(x,r).
\end{align}
Here recall that $\lambda$ is the parameter from the Christ-David cubes construction (Theorem \ref{t:Christ}); the constant $10^{-3}$ could be substituted with any other constant sufficiently small.
We consider three subcases, depending on what type of cube $Q_{x,r}$ is. 
\begin{enumerate}
    \item If 
    \begin{align*}
        Q_{x,r}  \in  \dD(Q_0)\setminus \BWGL(Q_0, \ve, \Cc_0).
    \end{align*}
then, by construction, $Q_{x,r}$ must satisfy the following. There exists a $d$-dimensional affine plane $L_{x,r}$ so that 
\begin{align*}
d_{\Cc_0 B_{Q_{x,r}}} (L_{x,r}, E) < \ve.
\end{align*}
Now, by Remark \ref{rem:Sigma-BAUP}, we can choose a subset of $\Sigma$,  denoted by $\Sigma'$, so that for each $x' \in \Sigma$, we can find a $d$-plane so that so that 
$d_{x', Ar} (P, \Sigma') < \ve$. We also make sure that the point $x \in \Sigma$ under consideration, also satisfies $x \in \Sigma'$. 
Next, we apply a result of David, Theorem 1.10 from \cite{david14}, to obtain a smooth surface $\wt \Sigma$, such that 
$\dist(x, \Sigma')< C \ve r$ for all $x \in \wt \Sigma$ and $\dist(x, \wt \Sigma) < C \ve r$ for all $x \in \Sigma'$.

Now, being a smooth surface, $\wt \Sigma$ satisfies local property of being linked to a $(n-d-1)$-dimensional sphere, as in the definition of Semmes surfaces in Definition \ref{def:semmes-surface}. This property is stable, thus holds for $\Sigma'$ at $x$. One can then use the proof of David of Lemma \ref{l:ss-top}, and the fact that $\Sigma' \subset \Sigma$, to obtain the lower bound
\begin{align*}
    \hd(\vp_1(E) \cap B(x, (1-\eta_0)r)) \geq \delta_0 r, 
\end{align*}
for any $\alpha_0$-ALD $\vp_t$,
with parameters depending on $\ve>0$.
\item Suppose now that 
\begin{align}\label{e:Qxr-Next}
    Q_{x,r} \in \mathscr{B}^\text{BWGL}(Q_0).
\end{align}
Then, by construction, there is a dyadic cube $I \in \dS(Q(x,r)) \cap \Delta_{k(Q)}$ such that $x \in I$ and $\frac{1}{2} \kappa\ell(Q) \leq \ell(I) \leq 2\kappa \ell(Q)$.
In particular, 
\begin{align*}
    \ell(I) \geq 10^{-4} \kappa_1 \kappa \lambda r. 
\end{align*}
Moreover, if we choose $\kappa_1$ appropriately (depending also on $0< \eta_0<1/100$), we can make sure that 
\begin{align*}
    E_Q \subset B(x, (1-\eta_0)r).
\end{align*}
Hence, if we choose
\begin{align*}
    \alpha_0 < 10^{-5} \lambda \kappa \kappa_1, 
\end{align*}
we get that
\begin{align*}
    \vp_1(\partial_d I) \subset N_{10^{-5} \tau \lambda \kappa r} (\partial I) \subset B(x,(1-\eta_0)r).
\end{align*}
Choosing $$0<\eta_0<1/100$$ (the precise upper bound for this parameter is not relevant here), we obtain that
\begin{align*}
    \hd(B(x,(1-\eta_0)r) \cap \vp_1(\partial_d I)) = \hd(\vp_1(\partial_d I)) \geq C (\kappa_1 \lambda \kappa)^d r^d
\end{align*}
If we now set
\begin{align*}
    \delta_0 = C (\kappa_1 \lambda \kappa)^d,
\end{align*}
and 
\begin{align*}
    \alpha_0 < 10^{-5}\kappa_1 \lambda \kappa,
\end{align*}
we obtain that, whenever $\vp_t$ is an $\alpha_0$-ALD,
\begin{align*}
    \hd(\vp_1(\Sigma) \cap B(x, (1-\eta_0)r)) \geq \hd(\vp_1(\partial_d I_Q)) \geq \delta_0 r^d.  
\end{align*}
\end{enumerate}
Hence we see that for $(x, r) \in E \times (0, \diam(\Sigma)/2)$, the topological condition \eqref{e:TC} is satisfied with constants $\alpha_0 = \min\{c \ve, 10^{-6}\tau \lambda \kappa\}$, $\delta_0 = \min\{c' \ve, C(\tau \lambda \kappa)^d$ and $0<\eta_0<1/100$.

\item \underline{Case 2.} If $x \in \Sigma \setminus E$, then by construction, 
\begin{align*}
    x \in E_Q \mbox{ for some } Q\in \mathscr{B}^\text{BWGL}(Q_0).
\end{align*}
In particular, $x \in \partial_d I$, for some $I \in \dS(Q)$.
We will consider two subcases. 
\begin{enumerate}
    \item Suppose that $0<r< C \ve^{-1} \ell(Q)$, for some constant $C$. Let $T_I$ be the $d$-dimensional face of $I$ containing $x$, and let $T(r)\subset T$ be a tile of $T$ of side length $10^{-1}\ve r$ which also contains $x$. If we choose $\alpha_0$ sufficiently small, say $\alpha_0 < 10^{-5} \ve $, and $0< \eta_0 < 1/100$, then we that for any $\alpha_0$-ALD $\vp_t$,
    \begin{align*}
        \vp_1(T(r)) \subset N_{\alpha_0 r}(T(r)) \subset B(x, (1-\eta_0)r),
    \end{align*}
    and thus 
    \begin{align*}
    \hd(\vp_1(\Sigma) \cap B(x, (1-\eta_0)r)) & \geq
    \hd(\vp_1(\partial_d I) \cap B(x,(1-\eta_0))) \\ & \geq \hd(\vp_1(T(r)) \cap B(x,(1-\eta_0)r))\\
    & = \hd(\vp_1(T(r))) \\
    & \geq (10^{-2}\ve)^d r^d.
    \end{align*}
    \item Suppose now that $C \ve^{-1}\ell(Q) \leq r \leq \diam(\Sigma)$. There exists a cube $\hat Q \in \dD$ so that $ \hat Q \supset Q$ and so that $r \sim \ell(\hat Q)$ (here we can choose the constant behind $\sim$ to depend on $\kappa_1$ and $\lambda$, as in \eqref{e:Qxr-ball}). Now, if $\hat Q \in \mathscr{G}^\text{BWGL}$, we can argue as Case 1, (1). If $\hat Q \in \mathscr{B}^{\text{BWGL}}(Q_0)$, we can argue as in Case 1, (2).
\end{enumerate}
\end{itemize}
We now choose the constants $\alpha_0$, $\delta_0$ and $\eta_0$ to be sufficiently small so that the upper bounds given in the various cases above hold, and the lemma is proven.  
\end{proof}

\begin{theorem}\label{t:Sigma}
Let $E \subset\R^n$ be a lower content $d$-regular set with constant $c_0$ and let $Q_0 \in \dD$. Given two parameters $0< \ve, \tau< 1$, there exists a set $\Sigma= \Sigma(\tau, \ve, Q_0)$ such that
\begin{enumerate}
    \item $Q_0 \subset \Sigma$.
    \item $\Sigma$ is a TC surface with constant $r_0= \diam(Q_0)$, $0<\eta_0<1/100$, and $\alpha_0$ and $\delta_0$ sufficiently small with respect to $\tau$ and $\ve$. 
    \item We have the estimate
    \begin{align*}
        \beta(Q_0)^2 + \diam(Q_0)^d \sim_{c_0, n, d, \ve} \hd(\Sigma). 
    \end{align*}
\end{enumerate}
\end{theorem}
\begin{proof}
We take $\Sigma$ to be the surface constructed in \eqref{e:Sigma}. It holds by definition that $Q_0 \subset \Sigma$. by Lemma \ref{l:Sigma-TC}, we see that also (2) is satisfied. We just need to check (3), but this is an easy consequence of Theorem \ref{t:main} and the Traveling Salesman theorem of Azzam and Schul. Indeed, from Theorem \ref{t:main}, we see that
\begin{align*}
    \beta(\Sigma)^2 + \diam(\Sigma)^d \lesssim C(\ve, \tau, n, d) \hd(\Sigma).
\end{align*}
On the other hand, using Lemma \ref{l:hd-Sigma-up} and the TST of Azzam and Schul, we have
\begin{align*}
    \hd (\Sigma) \lesssim_{c_0,n,d} \hd(Q_0) + \textrm{BWGL}_E(Q_0) \lesssim_{\ve,c_0, n,d} \beta_E(Q_0)^2 + \diam(Q_0)^d.
\end{align*}
By containment, we have $\beta(Q_0)^2 + \diam(Q_0)^d \lesssim \beta(\Sigma)^2 + \diam(\Sigma)^d$. This concludes the proof of Theorem \ref{t:Sigma}.
\end{proof}

==> 1000scarti.tex <==
To prove this Lemma we would like to use Lemma \ref{lemma:azzamschul} directly to bound the $\beta$ coefficients of $E$ in terms of those of $Z_R$, which we know that satisfy the Carleson packing property by virtue of being uniformly rectifiable. Unfortunately, however, $Z_R$ is not always as close to $E_R$ (and thus to $E$) as we would like it to be. We do the following. Set
\begin{align*}
    & \cG_{R, \rho} := \ck{I \in \cC_{R,\rho} \, |\, I \cap Z_R \neq \emptyset}, \mbox{ and } \\
    & \cB_{R,\rho} := \cC_{R,\rho} \setminus \cG_{R, \rho}. 
\end{align*}
Let $C_0$ be the inflation constant used for the $\beta$ numbers (see \eqref{i:C0}); for a cube $Q \in \dD$, we also put
\begin{align*}
    & \cC_{R}(Q) := \ck{ I \in \cC_R \, |\, I \cap 2C_0 Q \neq \emptyset};\\
    & \dZ_R (Q) := \ck{ I \in \cC_{R}(Q) \, |\, \mbox{ there exists a } J \in \cG_{R, \rho} \st J \cap I \neq \emptyset}.
\end{align*}
For a constant $0< c_4< 1$ to be fixed later, we define $\wt \Tree(R)$ to be the subfamily of cubes $Q \in \Tree(R)$, such that, first, 
\begin{align} \label{e:wtTree}
    \hd \ps{\bigcup_{ I \in \cC_R(Q) \setminus \dZ(Q)}} < c_4 \ell(Q)^d, 
\end{align}
and second, if $Q \in \wt \Tree(R)$, then all the cubes $Q'$ such that $Q \subset Q' \subset R$ also satisfy \eqref{e:wtTree}. 
We define $\wt \Forest(R)$ in the analogous manner.
Furthermore, we denote by 
\begin{align*}
    \wt \Stop(R)
\end{align*}
the family of minimal cubes in $\wt \Forest(R)$.
Finally, we put
\begin{align*}
    \Next_1(R) := \ck{ Q \in \Tree(R) \, |\, Q \in \Child(Q') \mbox{ for some } Q' \mbox{ minimal in } \wt \Forest(R)}.
\end{align*}
As convention and for future use, let us set $\Next_0(R)=\{R\}$. 
We denote the elements of $\Next_1(R)$ as $Q^1_i$, where $i \in \cI^1$ is some (finite) index set. 
For each $Q^1_i \in \Next_1(R)$, we run the stopping time algorithm as in Section \ref{s:ER}; we then construct $\wt E_{Q^1_i}$, $i \in \cI^1$, and the corresponding modification $E_{Q^1_i}$; we can then show that $E_{Q^1_i}$ satisfies the STC condition (just as it was done for $E_R$ in Section \ref{s:TC-STC}); hence we build the second approximating set $E_{Q_i^1, \rho}$, we show that it satisfies the STC (at scale $\ell(Q^1_i)$), as in Section \ref{s:E-rho-STC}, and hence obtain a uniform rectifiable set $Z_{Q^1_i}$ close to $E_{Q_i^1, \rho}$. For each $Q^1_i$, we defined $\wt \Tree(Q_i^1)$ and $\wt \Stop(Q_i^1)$ as above (with $Q_i^1$ instead of $R$) and then set
\begin{align*}
    \Next_1(Q_i^1) := \ck{ Q \in \Tree(Q_i^1) \, |\, Q \in \Child(Q') \mbox{ for some } Q' \mbox{ minimal in } \wt \Forest(Q_i^1)}.
\end{align*}
Next, we put
\begin{align*}
    \Next_2(R):= \bigcup_{i \in \cI^1} \Next_1(Q_i^1).
\end{align*}
Proceeding recursively in this fashion, we define
\begin{align*}
    \Next_{j+1}(R):= \bigcup_{i \in \cI^j} \Next_1(Q_i^j).
\end{align*}
Note that the procedure stops at some integer $K_R \in \N$, since $\Forest(R)$ is finite (and note that we always pick cubes from $\Forest(R)$). However, it will be important to obtain estimates independent of $K_R$.

\begin{sublemma}\label{sl:next1}
Let $Q_i^{j} \in \Next_j(R)$, for some $0\leq j \leq K_R$. Then 
\begin{align}
    \sum_{P \in \Next_1(Q_i^{j})} \ell(P)^d \lesssim \frac{1}{2} \ell(Q_i^j)^d.
\end{align}
\end{sublemma}
\begin{proof}
For this proof only, set $Q=Q_i^j$. Recall from the proof of Lemma \ref{l:large-intersection}, and in particular from \eqref{e:Jd}, that 
for each $\wt F$ constructed as above, we have that
\begin{align*}
    \hd(\wt F \setminus E_{Q, \rho}) \leq c_2 \delta_1 \ell(Q)^d.
\end{align*}
Note that, by the construction in \eqref{e:Zx}, 
\begin{align}
    Z_Q \subset \bigcup_{y \in E} B(y, \delta) \cap \wt F.\nonumber
\end{align}
We can have at most $\sim \frac{1}{\min\{\alpha_1, \delta_1\}}$ such balls $B(y, \delta)$ (by the choice of $\delta$). Hence, if we choose $c_2$ in \eqref{e:M} appropriately, we obtain that 
\begin{align}
    \hd(E_{Q, \rho} \setminus Z_Q) \leq 2 c_2 \ell(Q)^d. 
\end{align}
Now, by definition of $\Next_1(Q)$, we see that 
\begin{align}
    \ell(P)^d \leq \frac{1}{c_4} \hd\ps{\bigcup_{I \in \cC_{Q}(P) \setminus \dZ_Q(P)} \partial_d I} \nonumber
\end{align}
Recall that $\cC_Q(P) \setminus \dZ_Q(P)$ is the set of dyadic cubes $I$ in $\cC_Q$ so that, first $I \cap P \neq \emptyset$, and second, there does not exist a cube $J \in \cG_{Q, \rho}$ with $J \cap I \neq \emptyset$. Thus, we see that
\begin{align*}
    \bigcup_{I \in \cC_Q(P) \setminus \dZ_Q(P)} \partial_d I \subset \bigcup_{\{J \in \cB_{Q, \rho} \, |\, \exists I \in \cC_Q \st I \cap J \neq \emptyset \text{ and } I \cap P \neq \emptyset \}}  \partial_d J. 
\end{align*}
Therefore, because $\Next_1(Q)$ is a disjoint family, we have that
\begin{align*}
   & \sum_{P \in \Next_1(Q)}  \hd\ps{  \bigcup_{I \in \cC_Q(P) \setminus \dZ_Q(P)} \partial_d I } \\
   & \leq C \hd \ps{ \bigcup_{J \in \cB_{Q, \rho}} \partial_d J}\\
   & \leq \hd(E_{Q, \rho} \setminus Z_Q)\\
   & \leq c_2 \delta_1 \ell(Q)^d. 
\end{align*}
This in turn implies that
\begin{align}
    \sum_{P \in \Next_1(Q)} \ell(P)^d \leq C \frac{c_2 \delta_1}{c_4} \ell(Q)^d.
\end{align}
Choosing $c_2$ and $c_4$ appropriately, we obtain the lemma. 
\end{proof}
We now define one more family of cubes. Recall that for each $Q \in \wt \Stop(Q_i^j)$, there exists a dyadic cube $I_Q$ in $\cC_{Q_i^j}$ such that $x_Q \in I_Q$ and $\ell(I_Q) \sim \tau \ell(Q)$. We put
\begin{align*}
    \Approx(Q_i^j) := \ck{ S \in \dD \, |\, S \subset 2C_0 Q \mbox{ for some } Q \in \wt \Stop(Q_i^j) \mbox{ and } \ell(S) \sim \tau \ell(Q) }
\end{align*} 
It is clear that
\begin{align} \label{e:approx-cover}
2C_0 Q_j^i \subset \bigcup_{S \in \Approx(Q_i^j)} S.
\end{align}
The following lemma will be useful. 
\begin{lemma} \label{l:meta1}
 Let $Q$ be a minimal cube in $\wt \Tree(Q_i^j)$. Then there exists a dyadic cube $I_Q := I \in \cC_{Q_i^j}$ so that $I_Q \subset \frac{1}{2}B_Q$ and $\ell(I_Q) \sim \tau \ell(Q)$. 
\end{lemma}
\begin{proof}
   Let $x_Q$ be the center of $Q$. Then there exists a dyadic cube $I \in \cC_{Q_j^i}$ such that $x_Q \in I$; thus for $I$ we have $\dist(I, Q)=0$, and therefore $d_{Q_j^i}(I) \leq \dist(I, Q) + \ell(Q) = \ell(Q)$. In other words, when computing $d_{Q_j^i}(I)$, it suffices to minimise over all cubes $T$ such that 
   \begin{align*}
       \dist(I, T) + \ell(T) \leq \ell(Q).
   \end{align*}
   But note that since $Q$ is a minimal cube in $\wt \Tree(R)$, we must have that $T \subset Q^c$. Recall also that, by Theorem \ref{t:Christ}, $E \cap B(\zeta_Q, c_5 \ell(Q)) \subset Q$. If we let $\tau$ be small enough, we can insure that $I \subset B(\zeta_Q, \frac{c_5 \ell(Q)}{2})$; hence we see that \begin{align*}
        \dist(I, T) \gtrsim \ell(Q),
   \end{align*}
  and therefore $d_{Q_j^i}(I) \gtrsim \ell(Q)$. 
\end{proof}
\begin{lemma}\label{l:good-dist}
For a constant $C_4$ sufficiently large, if $Q \in \wt \Forest(Q_i^j)$ and $x \in 2C_0 Q$, then there exists a cube in $\Approx(Q_i^j)$ so that
\begin{align}\label{e:good-dist}
    \dist(x, Z_{Q_i^j}) \leq C_4 \ell(S). 
\end{align}
\end{lemma}

Before we prove this, let us prove the following other claim. 

\underline{Claim.} If $I \in \cC_{Q_i^j}$ and $I \cap Q \neq \emptyset$ for some $Q \in \wt \Stop(Q_i^j)$, then 
\begin{align}\label{e:claim1}
    \ell(I)\lesssim \tau \ell(Q).
\end{align}
To see this, recall that $\ell(I) \sim \tau d_{Q_i^j}(I) \leq \tau d_{Q_i^j}(x)$, whenever $x \in Q \cap I$. Moreover $d_{Q_i^j}$ is 1-Lipschitz, and so if $x_0$ is a point in $I_Q$ (where $I_Q$ is as in Lemma \ref{l:meta1}) so that $d_{Q_i^j}(I) \geq \frac{1}{2} d_{Q_i^j}(x_0)$, then
\begin{align*}
    \ell(I) \leq 2 \tau d_{Q_i^j}(x) \leq 4 \tau \ell(Q) + 2\tau d_{Q_i^j}(x_0) \leq 8 \tau \ell(Q).
\end{align*}
\begin{proof}[Proof of Lemma \ref{l:good-dist}]
Let $x \in 2C_0Q$. Then $x \in P\cap I$, where $P  \in \wt \Forest(Q_i^j)$ and $I \in \cC_{Q_i^j}$; also, $x \in S \in \Approx(Q_i^j)$ by the definition. By the claim above, we see that $\ell(I) \leq 20 C_0 \tau \ell(P)$. If $I \in \dZ(P)$, then we are done: if $y \in Z_{Q_i^j}\cap J$, where $J \in \cC_{Q_i^j, \rho}$ and $J \cap I \neq \emptyset$, then 
\begin{align*}
    |x-y| \leq 2 \ell(I),
\end{align*}
and thus $|x-y| \leq C(C_0) \tau \ell(P) \sim C(C_0) \ell(S)$.
Suppose on the other hand that the cube $I$ containing $x$ belongs to $\cC_{Q_j^i}(P) \setminus \dZ_{Q_i^j}(Q)$. Note that there must exists a cube $I' \in \dZ(P)$ with $\dist(I, I') \lesssim \tau \ell(P)$. Indeed, if not, we would have
\begin{align*}
    \hd \ps{ \bigcup_{I \in \cC_{Q_i^j}(P) \setminus \dZ_{Q_i^j}(P)} \partial_d I} \geq c_4 \ell(P)^d.
\end{align*}
But this contradicts the fact that $P \in \wt \Forest(Q_i^j)$. Hence using the fact that there exists a cube $I' \in \dZ_{Q_i^j}(P)$ with $\dist(I, I') \lesssim \tau \ell(P)$, we obtain \eqref{e:good-dist} also in this case.
\end{proof}


Thus we see that
\begin{align*}
    & \sum_{Q \in \Tree(R)} \beta_E^{p,d}(C_0 Q)^2 \ell(Q)^d\\
    & = \sum_{j=0}^{K_R} \sum_{Q \in \Next_j(R)} \sum_{P \in \wt \Tree(Q)} \beta_E^{p,d}(C_0 P)^2 \ell(P)^d \\
    & \leqt{\eqref{e:treetilde}} \sum_{j=0}^{K_R} \sum_{Q \in \Next_j(R)} C \ell(Q)^d.
\end{align*}
Note that for $0 \leq j \leq K_R$, we see that if we apply repeatedly Sublemma \ref{sl:next1}, we obtain
\begin{align*}
    & \sum_{Q \in \Next_j(R)} \ell(Q)^d = \sum_{Q \in \Next_{j-1}(R)} \sum_{P \in \Next_1(Q)} \ell(P)^d \\
    & \leq \sum_{Q \in \Next_{j-1}(R)} \frac{1}{2} \ell(Q)^d \\
    & = \sum_{Q \in \Next_{j-2}(R)} \sum_{P \in \Next_1(Q)} \frac{1}{2} \ell(P)^d \\
    & \leq \sum_{Q \in \Next_{j-2}(R)} \frac{1}{2^2} \ell(Q)^d \\
    & \vdots \\
    & \leq \frac{1}{2^j} \ell(R)^d.
\end{align*}
Hence we have that 
\begin{align*}
     \sum_{j=0}^{K_R} \sum_{Q \in \Next_j(R)} C \ell(Q)^d \leq \ell(R)^d \sum_{j=0}^{K_R} \frac{1}{2^j} \lesssim \ell(R)^d.
\end{align*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us now conclude the argument and show that \eqref{e:main} holds. 
Fix a ball $B$ centered on $E$, with radius $r_B$. By rescaling and translating, we can assume without loss of generality that the center of the ball is $0$ and that $r_B=1$. Let $Q_0 \in \dD$ be the maximal Christ-David cube so that $Q_0 \subset B(0,1)$ and $\ell(Q_0) \gtrsim 1$. 
We have that
\begin{align} \label{e:dyadic-christ}
    \sum_{\substack{I \in \Delta_0 \\ I \cap E \cap B(0,1) \neq \emptyset }}\beta_E^{p,d} (C_0 I)^2 \ell(I)^d  \lesssim_{n,C_0} 1+  \sum_{Q \subset Q_0} \beta_E^{p,d}(2 C_0 B_Q)^2 \ell(Q)^d;  
\end{align}
indeed, we can split the sum on the left hand side of \eqref{e:dyadic-christ} into two sums, one where we sum over all dyadic cubes which have sidelength larger that $\ell(Q_0)$, and a second one where we sum over dyadic cubes with $\ell(I) < \ell(Q_0)$. The first sum is bounded above by a universal constant depending on $n, d$ and $\rho$ (the parameter in the construction of the Christ-David cubes). 
For the second one, note that for each $I \in \Delta$ such that $I \cap E \neq \emptyset$ and $\ell(I)< \ell(Q_0)$, there exists a cube  $Q \in \dD, Q \subset Q_0$ such that $I \cap Q \neq \emptyset $ and $\ell(Q) \sim \ell(I)$. Therefore it is easy to see that $\beta_E^{p,d}(C_0 I) \lesssim_{n, d, C_0} \beta_E^{p,d}(2C_0 B_Q)$. Moreover, for a fixed $Q \in \mathcal{D}$, the number of dyadic cubes $I$ so that $I \cap Q \neq \emptyset$ and $\ell(I) \sim \ell(Q)$ is bounded above by a universal constant; with this, we obtain \eqref{e:dyadic-christ} and therefore the estimate 
\begin{align}
    \sum_{\substack{I \in \Delta_0 \\ I \cap E \cap B}} \beta_E^{p,d}(C_0 I)^2 \ell(I)^d \lesssimt{\eqref{e:dyadic-christ}, \eqref{e:k0}} 1 + \hd(E \cap B). 
\end{align}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For each $R \in \Top(k_0)$, we define a  $\wt \Tree(R)$, a subfamily of $ \Tree(R)$, as follows. First, we immediately put $R \in \wt \Tree(R)$; second, we add $Q \in \Tree(R)$ to $\wt \Tree(R)$ if, 
\begin{align} \label{e:wtTree}
     Q \in \cG^{\text{BWGL}}_{}(Q_0);
\end{align}
 and if $Q \in \wt \Tree(R)$, then all the cubes $Q'$ such that $Q \subset Q' \subset R$ also satisfy \eqref{e:wtTree}; third, if there exists a $Q' \in \Child(Q)$ so that $Q \notin \mathscr{good}^{\text{BWGL}}(Q_0)$, for some $Q \in \wt \Tree(R)$, then we ask that $\Child(Q) \subset \ps{\wt \Tree(R)}^c$.

 This guarantees that $\wt \Tree(R)$ is a stopping time region (see Definition \ref{d:stopping}).
In other words, $\wt \Tree(R)$ is a pruned version of $\Tree(R)$, where we cut whenever we found a cube $Q \in \cB^\text{BWGL}$. We also put
\begin{align*}
    \wt \Stop(R) := \ck{ Q \in \cD \, |\, Q \mbox{ minimal  in } \wt \Tree(R)}.
\end{align*}
Next we let
\begin{align}
\begin{aligned}[t]
   \Next_1(R):= 
   \Big\{
 Q \in \Tree(R) \, | &\, Q \in \Child(Q')\\
 & \mbox{ for some } Q' \mbox{ minimal in } \wt \Tree(R) 
  \Big\}
 \end{aligned}
\end{align}
Set $\Next_0(R)= \ck{R}$. Denote each element of $\Next_1(R)$ by $Q^1_i$, for $i \in \cI^1$, some index set; furthermore for each $i \in \cI^1$, we run a stopping algorithm again, stopping whenever we meet a cube in $\cB^\text{BWGL}_\cD$, or we reach the bottom of $\Tree(R)$. In other words, for $i \in \cI^1$, we let $ \wt \Tree(Q_i^1)$ to be the subfamily of cubes in $\Tree(R)$, such that 
\begin{align*}
    & Q \subset Q^1_i \\
    & Q \in \cG_\cD^\text{BWGL}Q_0) \mbox{ and } \\
    & \wt \Tree(Q^1_i) \mbox{ is coherent}.
\end{align*}
We let $\wt \Stop(Q_i^1)$ denote the minimal cubes in $\wt \Tree(Q_i^j)$. Further, we set
\begin{align*}
    \Next_1(Q_i^1):= 
   \Big\{
 Q \in \Tree(R) \, | &\, Q \in \Child(Q')\\
 & \mbox{ for some } Q' \mbox{ minimal in } \wt \Tree(Q_i^1) 
  \Big\}
\end{align*}
and finally
\begin{align*}
    \Next_2(R) := \bigcup_{i \in \cI^1} \Next_1(Q_i^1).
\end{align*}
Proceeding inductively in this fashion, we define
\begin{align*}
    \Next_{j+1}(R):= \bigcup_{i \in \cI^j} \Next_1(Q_i^j).
\end{align*}
This process terminates at some integer $K_R$ since $\Tree(R)$ is finite. We also set
\begin{align*}
    \Next(R) := \bigcup_{i=1}^{K_R} \Next_j(R). 
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%
Before proving this, however, let us state following two technical lemmas. Their proofs are standard, but we include them in the appendix for completeness.
\begin{lemma} \label{l:meta1} Let $S$ be a cube in $\wt \Stop(Q)$ for some $Q \in \Next(R)$, $R \in \Top(k_0)$. Then there exists a dyadic cube $I_S := I \in \cC_{Q}$ so that $I_S \subset \frac{1}{2}B_S$ and $\ell(I_S) \sim \tau \ell(S)$.
\end{lemma}

\begin{lemma}\label{l:I-QI}
Let $I \in \cC_Q$ for $Q \in \Next(R)$, $R \in \Top(k_0)$. Then there exists a cube $Q_I \in \wt \Tree(Q)$ so that 
\begin{align*}
    & \ell(I) \leq \ell(Q_I) \leq c \tau^{-1} \ell(I); \\
    & \dist(I, Q_I) \leq c \tau^{-1} \ell(I). 
\end{align*}
\end{lemma}





%%%%%%%%%%%%%%
First, we set $k_0^*$ to be the minimal integer so that a non trivial corona decomposition $\Top(k_0^*)$ exists so that for any $x_1 \in E$, we can find an $R \in \Top(k_0^*)$ with $x_1 \in R$ and $\frac{\ell(R)}{4} \leq \frac{r_0}{1000}$. Note that then, any corona decomposition $\Top(k_0)$, with $k_0 \geq k_0^*$, will satisfy such requirements. 
\begin{remark}
Note that such a $k^*_0$ is not guaranteed to exists. However, in this case, the following would hold: we can find a cube $R \in \dD$ such that given any cube $Q \in \dD(R)$, $Q$ cannot satisfy \eqref{e:ST-cond}. This implies that $R$ is Ahlfors regular for all the scales smaller that $\ell(R)$. Hence we can always construct a skeletal approximation $E_R$, and this approximation will be good (in the sense of \eqref{e:adr-corona}) up to an arbitrary small scale of our choice. In particular, we can decompose $R$ into a family $\dR:= \{R'\}_{R' \subset R}$ so that
\begin{align*}
    & R = \bigcup_{R'\in \dR} R' \mbox{ and } \\
    & \frac{\ell(R')}{4} \leq r_0/1000. 
\end{align*}
The corresponding approximating sets $E_{R'}$, $R \in \dR$, will have the same properties as those constructed in Lemma \ref{l:corona}.
\end{remark}





%%%%%%%%%%%%


\begin{lemma}\label{l:reifenberg}
Fix $\epsilon >0$ and let $E \subset \R^n$. If for each $(x,r) \in E \times (0,\diam(E))$ there exists a $d$-dimensional plane $P$ with
\begin{align} \label{e:l-reifenberg1}
    d_{x,r}(E, P) < \ve, 
\end{align}
then there are constants $\alpha_0,\delta_0, \eta_0$ which depend only on $\ve$, $n$ so that for any $\alpha_0$-ALD $\vp_t$, we have
\begin{align*}
    \hd(\vp_1(E) \cap B(x, (1-\eta_0)r)) \geq \delta_0 r^d. 
\end{align*}
\end{lemma}
The proof of this follows quite quickly from two observation. First, note that if there exists a $d$-plane $P$ so that $ d_{x,r} (E, P) < \epsilon$, then the image of $E$ under an $\epsilon$-ALD will satisfy $d_{x,r} (\vp_1(E),P) < 2 \epsilon$. Indeed, recall that if $\vp_t$ is an $\epsilon$-ALD, then \eqref{e:vp4} tell us that 
\begin{align}
    \dist(\vp_t(y), E)\leq \epsilon r \mbox{ for all } 0 \leq t \leq 1 \mbox{ and } y \in B(x,r)\cap E.
\end{align}
Second, it is easy to see that if a pair $(x,r) \in E \times \R_+$ satisfies $d_{x,r}(E, P)< 2\ve$ for some $d$-plane $P$, then $d_{x,r/2}(E, P) < 4 \ve$ and so $\hd(E \cap B(x,(1-\eta_0)r)) \geq  c(\epsilon) r^d$, where $c(\epsilon)<1$ is a positive constant which depends only of $n, d$ and $\epsilon$, and $\eta_0$ is a positive constant that can be chosen to be smaller that $1/100$, say. In particular, these parameters do not depend on the set $E$. For a proof of this, see Lemma 13.2 in
\cite{david-toro12}. 
Putting together these two facts, we immediately see that the topological condition TC is satisfied. 

==> 20-problems.tex <==
\section{Follow up problems}
Let us consider some problems that one can think about, coming from this paper. 
 First, one notices that the following are immediate corollary of the main results together with the Analyst's travelling salesman of Azzam and Schul. 
 
    \textbf{Corollary 1.} If $\Gamma$ is a David surface, and if its Hausdorff measure is finite, then $\Gamma$ is rectifiable. 
    
    \textbf{Corollary 2. } If moreover $\Gamma$ is upper regular, then $\Gamma$ is uniformly rectifiable.
    
\begin{enumerate}
    \item The most interesting, but very vague possible application is to Favard length. The Favard length conjecture says that if 
    $\int |\Pi_V(E \cap B)| d V > C$ for a constant $C>0$, then $\mathcal{H}^1(E \cap B \cap F) \geq C'$, where $F$ is a Lipschitz graph, and $C'$ is a constant depending on $C$. 
    
    The intuition on why this could somewhat related to David surfaces is the following: suppose that we can find an allowed lipschitz deformation $\vp$ for which the Hausdorff measure of $E \cap B$ drops below the threshold. This means that there has to be some big hole. Moreover, we can compose this Lipschitz allowd deformation with a Federer-Fleming projection. This will imply that the FF projection will have small measure. The question then becomes 

\end{enumerate}

==> Commands.tex <==
%Alphabets
\def\dA{{\mathcal{A}}}
\def\dB{{\mathcal{B}}}
\def\dC{{\mathcal{C}}}
\def\dF{{\mathcal{F}}}
\def\dG{{\mathcal{G}}}
\def\dN{{\mathcal{N}}}
\def\dS{{\mathcal{S}}}

\def\bA{{\mathbb{A}}}
\def\bB{{\mathbb{B}}}
\def\bC{{\mathbb{C}}}
\def\bD{{\mathbb{D}}}
\def\bR{{\mathbb{R}}}
\def\bS{{\mathbb{S}}}
\def\bO{{\mathbb{O}}}
\def\bE{{\mathbb{E}}}
\def\bF{{\mathbb{F}}}
\def\bH{{\mathbb{H}}}
\def\bI{{\mathbb{I}}}
\def\bT{{\mathbb{T}}}
\def\bZ{{\mathbb{Z}}}
\def\bP{{\mathbb{P}}}
\def\bN{{\mathbb{N}}}
\def\bQ{{\mathbb{Q}}}
\def\bK{{\mathbb{K}}}
\def\bG{{\mathbb{G}}}
\def\va{{\textbf{a}}}
\def\vb{{\textbf{b}}}
\def\vc{{\textbf{c}}}
\def\vx{{\textbf{x}}}
\def\vu{{\textbf{u}}}
\def\vv{{\textbf{v}}}
\def\vw{{\textbf{w}}}
\def\vy{{\textbf{y}}}

\def\RP{\bR P}


\def\nrj{{\mathcal{E}}}
\def\cA{{\mathscr{A}}}
\def\cB{{\mathscr{B}}}
\def\cC{{\mathscr{C}}}
\def\cD{{\mathscr{D}}}
\def\cE{{\mathscr{E}}}
\def\cF{{\mathscr{F}}}
\def\cG{{\mathscr{G}}}
\def\cH{{\mathscr{H}}}
\def\cI{{\mathscr{I}}}
\def\cJ{{\mathscr{J}}}
\def\cK{{\mathscr{K}}}
\def\Layer{{\rm Layer}}
\def\cM{{\mathscr{M}}}
\def\cN{{\mathscr{N}}}
\def\cO{{\mathscr{O}}}
\def\cP{{\mathscr{P}}}
\def\cQ{{\mathscr{Q}}}
\def\cR{{\mathscr{R}}}
\def\cS{{\mathscr{S}}}
%\def\cT{{\mathscr{T}}}
\def\Up{{\rm Up}}
\def\cU{{\mathscr{U}}}
\def\cV{{\mathscr{V}}}
\def\cW{{\mathscr{W}}}
\def\cX{{\mathscr{X}}}
\def\cY{{\mathscr{Y}}}
\def\cZ{{\mathscr{Z}}}


\def\sA{\mathfrak{A}}
\def\sB{\mathfrak{B}}
\def\sC{\mathfrak{C}}
\def\sD{\mathfrak{D}}
\def\sE{\mathfrak{E}}
\def\sF{\mathfrak{F}}
\def\sG{\mathfrak{G}}

\def\sL{\mathfrak{L}}
\def\sM{\mathfrak{M}}
\def\sP{\mathfrak{P}}
\def\sQ{\mathfrak{Q}}
\def\sR{\mathfrak{R}}
\def\sS{\mathfrak{S}}
\def\sU{\mathfrak{U}}
\def\sX{\mathfrak{X}}
\def\sZ{\mathfrak{Z}}
\def\one{\mathds{1}}
\def\sign{\mbox{sign }}

\def\largetheta{\Theta_}


%Random shortcut symbols
\def\ve{\epsilon} % needed to  unite between \epsiln and \ve because we were not consistent
\def\vp{\varphi}
\def\sothat{\mathop\mathrm{ s.t. }}
\renewcommand{\d}{{\partial}}
\def\lec{\lesssim}
\def\gec{\gtrsim}
\def\into{\rightarrow}
\def\Lap{\triangle}






\def\ext{\mathop\mathrm{ext}} 	
\def\spn{\mathop\mathrm{span}} 	
\DeclareMathOperator{\diam}{diam}
\def\Cap{\mathop\mathrm{Cap}} 					% capacity 
\def\Osc{\mathop\mathrm{Osc}}					%oscillation 
\def\Tan{\mathop\mathrm{Tan}} 					%tangent measures
\def\BMO{\mathop\mathrm{BMO}} 					%BMO
\def\Lip{\mathop\mathrm{Lip}} 						%lipschitz constant 
\def\Mod{\mathop\mathrm{Mod}} 					%modulus
\def\co{\mathop\mathrm{co }}						%smallest convex set, i.e. the convex hull
\def\cco{\overline{\mathop\mathrm{co}}\;} 				%smallest closed convex set			
\def\dim{\mathop\mathrm{dim}} 					%dimension	
\def\dist{\mathop\mathrm{dist}} 						%distance
\def\id{\mathop\mathrm{id}}						%identity
\def\Int{\mathop\mathrm{Int}} 						%Interior
\def\ker{\mathop\mathrm{ker }}						%kernel
\def\supp{\mathop\mathrm{supp}}					%support
\def\wk{\mathop\mathrm{wk }} 						%weak as in weak topologies
\def\loc{\mathop\mathrm{loc}}						%locally
\def\cof{\mathop\mathrm{cof }} 						%cofactor
\DeclareMathOperator*{\esssup}{ess\,sup}			%essential supremum
\DeclareMathOperator*{\essinf}{ess\,inf}				%essential infimum
\renewcommand{\div}{\mathop\mathrm{div }}			%divergence

%Brackets
\newcommand{\ps}[1]{\left( #1 \right)}
\newcommand{\bk}[1]{\left[ #1 \right]}
\newcommand{\ck}[1]{\left\{#1 \right\}}
\newcommand{\av}[1]{\left| #1 \right|}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\cnj}[1]{\overline{#1}}
\newcommand{\isif}[1]{\left\{\begin{array}{cc} #1
\end{array}\right.}
\newcommand{\nrm}[1]{\left|\left| #1 \right|\right|}
\newcommand{\ob}{\overbrace}
\newcommand{\ub}{\underbrace}
\newcommand{\fr}[2]{\frac{#1}{#2}}

%\def\barintgerm_#1{\mathchoice
%{\mathop{\vrule width 6pt height 3 pt depth -2.5pt
%\kern -8.8pt \intop}\nolimits_{#1}}%
%{\mathop{\vrule width 5pt height 3 pt depth -2.6pt
%\kern -6.5pt \intop}\nolimits_{#1}}%
%{\mathop{\vrule width 5pt height 3 pt depth -2.6pt
%\kern -6pt \intop}\nolimits_{#1}}%
%{\mathop{\vrule width 5pt height 3 pt depth -2.6pt \kern -6pt
%\intop}\nolimits_{#1}}}


\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$ }
\vcenter{\hbox{$#2#3$ }}\kern-.58\wd0}}
\def\ddashint{\Xint=}
\def\avint{\Xint-}
%
%\newcommand{\avint}{\Xint} %average integral, thanks Jason A

%Linear Algebra and Optimization
\newcommand{\vctr}[1]{\left(\begin{array}{c} #1 \end{array}\right)}
\newcommand{\mtrx}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}

\def\grad{\nabla}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{xca}[theorem]{Exercise}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\numberwithin{equation}{section}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\SH}{\mathcal{S}}
\newcommand{\haus}[2]{\mathscr{H}^{#1}_{#2}}
%\newcommand{\diam}{\mathrm{\, diam}}
\newcommand{\psicar}{\psi^{h, \mathscr{F}}}
\newcommand{\F}{\mathscr{F}}
%\newcommand{\supp}{\mathrm{supp }}
\newcommand{\Sp}{S^{n-1}}
\newcommand{\Lloc}{L^1_{\mathrm{loc}}}
%\newcommand{\sign}{\mbox{sgn}}
\newcommand{\dxdt}{\frac{dtdx}{t}}
\newcommand{\dtdx}{\frac{dxdt}{t}}
\newcommand{\hde}{\mathcal{H}^d|_E}
\newcommand{\lip}{\mathrm{Lip}}
\newcommand{\hd}{\mathcal{H}^d}
\newcommand{\hm}[1]{\mathcal{H}^{#1}}
\newcommand{\hdc}{\mathcal{H}^d_\infty}
\newcommand{\Tn}{\mathrm{Tn}}
\newcommand{\thetamax}{\theta_{\mbox{max}}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\interior}{\mathrm{Int}}
\newcommand{\bil}{\mbox{bil}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\conesindex}{K(i,j,h,q,k)}
\newcommand{\cones}{\mathrm{Cn}}
\newcommand{\lipcones}{\Gamma_{i,j, \mathbf{N}}^{k, h}}
\newcommand{\grass}{G(d, d+1)}
\newcommand{\bubbles}{B(i,j,h,q,k)}
\newcommand{\betae}[1]{\beta_E^{#1, d}}
\newcommand{\spt}{\mathrm{spt}}
\newcommand{\dt}{\frac{dt}{t}}
\newcommand{\dr}{\frac{dr}{r}}
\newcommand{\wt}{\widetilde}

\newcommand{\cubes}{\mathcal{D}}
\newcommand{\mucubes}{\mathcal{D}_\mu}
\newcommand{\Badsh}{\text{BAD}}
%tools
\newcommand{\eqt}[1]{\ensuremath{\stackrel{#1}{=}}}
\newcommand{\leqt}[1]{\ensuremath{\stackrel{#1}{\leq}}}
\newcommand{\leqref}[1]{\ensuremath{\stackrel{\text{\eqref{#1}}}{\leq}}}
\newcommand{\geqref}[1]{\ensuremath{\stackrel{\text{\eqref{#1}}}{\geq}}}
\newcommand{\equref}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\lesssimt}[1]{\ensuremath{\stackrel{#1}{\lesssim}}}
\newcommand{\gtrsimt}[1]{\ensuremath{\stackrel{#1}{\gtrsim}}}

%Families symbols
 \def\Bad{\mathrm{Bad}}
\def\Top{\textrm{Top}}
\def\Stop{\textrm{Stop}}
\def\Tree{\textrm{Tree}}
\def\Next{\mathrm{Next}}

\newcommand{\ds}{d_{\bS^1}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}



==> TND1.tex <==





















\subsection{A uniformly rectifiable set close to $E_R$}
\begin{lemma}
For $R \in \Top$, there exists a set $F_R$ which is uniformly rectifiable and lie close to $E_R$ 
\end{lemma}

This lemma will follow from the main result of \cite{david-semmes00}, and from the construction of the approximating set $E_R$. 
\begin{theorem}[{\cite{david-semmes00}, Theorem 2.11}] \label{t:UR-QM}
    Let $U$ be an open set in $\R^n$, and suppose that $S$ is a $(U, k, \delta)$-quasiminimizer for $\hd$. Let $S^*$ be the support in $U$ of the restriction of $\hd$ to $S$. Then for each $x \in S^*$ and radius $R$ which satisfy
    \begin{align}
        0<R< \delta \mbox{ and } B(x, 3R) \subset U,
    \end{align}
    there is a compact, Ahlfors $d$-regular set $Z$ such that
    \begin{align}
        S^* \cap B(x,R) \subset Z \subset S^* \cap B(x,2R)
    \end{align}
    and
    \begin{align}
        Z \mbox{ is uniformly rectifiable and contains big pieces of Lipschitz graphs.}
    \end{align}
    The constants for the Ahlfors regularity and for the uniform rectifiability of $Z$ depend only on $n$ and $k$.
\end{theorem}
By Lemma \ref{l:quasiS}, we know that $S= \wt F \cap B_2$ (recall that $\wt F$ is a minimiser of the functional $J$ over $\dF$, see definitions \eqref{e:J} and \eqref{e:dF}) is a $(B_2, k, \delta)$-quasiminimizer for $\hd$. Also recall that
\begin{align*}
    B_2=B\ps{x, r- \frac{8}{10} \eta_1 \ell(R) } \mbox{ (see \eqref{e:Bj})},
\end{align*}
that $k = C4^{nd}M$, and $\delta= c_1 \min\{\alpha_1, \eta_1\} \ell(R)$. Then, choosing $c_1$ appropriately 



\section{$\beta$ number estimates}
if $\cC$ are the Christ-David cubes, we write $\cD_0= \{Q_0\}$. For an positive integer $k_0$, we also write $\cD(k_0)= \bigcup_{k=0}^{k_0} \cD_{k}$.
\begin{lemma} \label{lemma:upper_beta_est}
Let $p=p(d)$ be as in \eqref{e:pd} and fix an arbitrary integer $k_0>0$.
There exists a constant $C_0 \geq 1$ (independent of $k_0$) so that, with the above notation, 
\begin{align} \label{e:upper_beta_est}
    \sum_{\substack{Q \subset Q_0\\ Q \in \cD(k_0)}} \beta_E^{p,d}(C_0Q)^2\ell(Q)^d \leq C \hd(E \cap B_{Q_0}),
    \end{align}
where $C$ depends on $n, d$, but not on $k_0$. 
\end{lemma}

We will use the following lemma. 
\begin{lemma}[{[AS1], Lemma 2.21}] \label{lemma:azzamschul}
Let $1 \leq p < \infty$ and $E_1, E_2 \subset \R^n$. Let $x \in E_1$ and fix $r>0$. Take some $y \in E_2$ so that $B(x,t) \subset B(y, 2t)$. Assume that $E_1, E_2$ are both lower content $d$-regular. Then
\begin{align*}
    \beta_{E_1}^{p,d} (x,t) \lesssim_c \beta_{E_2}^{p,d} (y, 2t) + \left( \frac{1}{t^d} \int_{E_1 \cap B(x, 2t)} \left(\frac{\dist (y, E_2)}{t} \right)^p \, d \hdc(y)\right)^{\frac{1}{p}}.
\end{align*}
\end{lemma}
First, let us define a further family of cubes. For a cube $R \in \Top$, we set
\begin{align}
     \widetilde \Stop(R) := \left\{ \mbox{maximal } Q \in \mathscr{D}  \, |\, \exists I \in \cC_R \mbox{ s.t. } I \cap Q \neq \emptyset \mbox{ and } \ell(I) \sim \ell(Q)\right\}.
\end{align}
Note that 
\begin{align} \label{eq:SS_tildestopcover}
    \bigcup_{Q \in \wt \Stop(R)} Q \supset R.
\end{align}
Indeed, if $y \in R$, then there exists a cube $I \in \cC_R$ so that $y \in I$, and a cube $Q \in \wt \Stop(R)$ with $I \cap Q\neq \emptyset$ and $\ell(I) \sim \ell(Q)$. If $y \notin Q$, then its parent cube will contain $y$.
\begin{lemma} \label{lemma:betatree}
Let $p=p(d)$ be as in \eqref{e:pd} and fix an arbitrary integer $k_0>0$.
There exists a constant $C_0 \geq 1$ \textup{(}independent of $k_0$\textup{)} so that, with the above notation,
\begin{align} 
    \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \beta_{E}^{p,d}(C_0Q)^2 \ell(Q)^d & \lesssim  \ell(R)^d,
\end{align}
where the constant behind the symbol $\lesssim$ depends on $n, d, C_0$, and the Ahlfors regularity constant of $E_R$, but not on $k_0$. 
\end{lemma}
\begin{proof}
Fix $R \in \Top$. For $Q \in \Tree(R)$, choose $x_Q' \in E_R$ to be the closest point to $x_Q$. By \eqref{e:adr-corona}, there exists a constant $C_0 \geq 1$ so that $|x_Q- x_Q'| \leq C_0 \ell(Q)$; let $B'_Q= B(x_Q', \ell(Q))$. We apply Lemma \ref{lemma:azzamschul} to estimate 
\begin{align*}
    \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \beta_{E}^{p, d} (C_0B_Q)^2 \ell(Q)^d  \lesssim \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \beta_{E_R}^{p,d} (2C_0B'_Q)^2 \, \ell(Q)^d \\
    + \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \ps{\frac{1}{\ell(Q)^d} \int_{2C_0 B_Q\cap E} \ps{\frac{\dist(y, E_R)}{\ell(Q)}}^p \, d \hdc(y) }^{\frac{2}{p}}\, \ell(Q)^d \\
    & := I_1 + I_2.
\end{align*}

\michele{Added above.}

We first look at $I_1$. We apply Theorem \ref{theorem:Christ_cubes} to $E_R$; let us denote the cubes so obtained by $\cD_{E_R}$. Note that for each $Q \in \Tree(R)$ with $Q \in \cD(k_0)$, $x_Q'$ belongs to some cube $\wt Q \in \cD_{E_R}$ so that $\ell(\wt Q) \sim \ell(Q)$; hence there exists a constant $C_1 \geq 1$ so that 
\begin{align}
    2C_0 B'_Q \subset C_1B_{\wt Q}.
\end{align}
This in turn implies that $\beta_{E_R}^{p,d}(2C_0 B'_Q) \lesssim_{p,n,d,C_0,C_1} \beta_{E_R}^{p,d}(C_1 B_{\wt Q})$. Hence, 
\begin{align}
    \sum_{\substack{ Q \in \Tree(R) \\ Q \in \cD(k_0)}} \beta_{E_R}^{p,d} (2C_0 B'_Q)^2 \ell(Q)^d \lesssim_{p,n,d,C_0, C_1} \sum_{\substack{\wt Q \in \cD_{E_R} \\ \ell(\wt Q) \lesssim \ell(R) }} \beta_{E_R}^{p,d} (C_1 B_{\wt Q})^2 \ell(\wt Q)^d. 
\end{align}
Since $E_R$ is uniformly rectifiable by Theorem \ref{theorem:Dav88}, we immediately have that $I_1 \lesssim \ell(R)^d$. 
Let us now estimate $I_2$.
If $y \in R$, we claim that there exists a cube $S \in \wt \Stop(R)$ such that 
\begin{align} \label{eq:SS_distyER}
    \dist(y, E_R) \lesssim \ell(S);
\end{align}
indeed, $y \in R$ implies by \eqref{eq:SS_tildestopcover} that that there exists a cube $S \in \wt \Stop(R)$ containing $y$. Moreover, there exists a dyadic cube $I \in \cC_R$ with $I \cap S \neq \emptyset$ and $\ell(I) \sim \ell(S)$. Then there exists a point $y' \in S\cap I$, and further a point $y'' \in \partial_d I \subset E_R$. Hence \eqref{eq:SS_distyER} holds.
We can now estimate the integral in $I_2$ with \eqref{eq:SS_distyER} as follows.
\begin{align*}
    \int_{2C_0 B_Q\cap E} \ps{\frac{\dist(y, E_R)}{\ell(Q)}}^p \, d \hdc(y) & \lesssim \sum_{\substack{S \in \widetilde \Stop(R) \\ S \cap 2C_0B_Q \neq \emptyset }} \int_{S} \frac{\ell(S)^p}{\ell(Q)^p}  \\
    & \lesssim \sum_{\substack{S \in \widetilde \Stop(R) \\ S \cap 2C_0B_Q \neq \emptyset }} \frac{ \ell(S)^{d+p}}{\ell(Q)^{p}},
\end{align*}
and so 
\begin{align*}
    I_2 \lesssim \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \sum_{\substack{S \in \widetilde \Stop(R) \\ S \cap 2C_0B_Q\neq \emptyset }} \frac{\ell(S)^{\frac{2d}{p} + 2}}{\ell(Q)^{d(\frac{2}{p}-1) + 2}}.
\end{align*}
Clerly, since $S \cap 2C_0 B_Q \neq \emptyset$, we must have that $\dist(x_Q, S) \leq 2C_0 \ell(Q)$. Moreover, by Lemma \ref{lemma:SS_prop2} and the definition of $\wt \Stop(R)$, we have that 
\begin{align}
    \ell(S)  \sim \ell(I) \sim_{\tau} d_{\Stop(R)}(I)  \leq \ell(Q) + \dist(I, Q) \leq 3C_0 \ell(Q)
\end{align}
whenever $S$ intersects $2C_0 B_Q \cap E$.
Then we see that the number of cubes $Q \in \Tree(R)$ of a given generation so that $S \cap 2C_0 B_Q \neq \emptyset$ is bounded above by a universal constant depending on $n$ and $C_0$. Thus we can write
\begin{align}
    & \sum_{Q \in \Tree(R)} \sum_{\substack{ S \in \widetilde \Stop(R)\\ S \cap 2C_0 B_Q \neq \emptyset}} \frac{\ell(S)^{\frac{2d}{p} + 2}}{\ell(Q)^{d(\frac{2}{p}-1) + 2}} \nonumber\\
    & \lesssim \sum_{\substack{S \in \widetilde{\Stop}(R)\\ S \cap  2C_0B_R \neq \emptyset}} \sum_{\substack{Q \in \Tree(R) \\ S \cap 2C_0 B_Q \neq \emptyset}} \frac{\ell(S)^{\frac{2d}{p} + 2}}{\ell(Q)^{d(\frac{2}{p}-1) + 2}} \label{e:estBeta1}
\end{align}
Using the remark above, we can sum geometrically the interior series:
\begin{align*}
    \sum_{\substack{Q \in \Tree(R) \\ S \cap 2C_0 B_Q \neq \emptyset}} \frac{1}{\ell(Q)^{d(\frac{2}{p}-1) + 2}} \lesssim_{n} \frac{1}{\ell(S)^{d(\frac{2}{p}-1) +2}}. 
\end{align*}
Therefore we obtain 
\begin{align*}
    \eqref{e:estBeta1} \lesssim \sum_{\substack{S \in \wt \Stop(R) \\ S \cap 2C_0B_R \neq \emptyset}}  \frac{\ell(S)^{d(\frac{2}{p}) +2 }}{\ell(S)^{d(\frac{2}{p}-1) + 2}} = \sum_{\substack{S \in \wt \Stop(R) \\ S \cap 2C_0B_R  \neq \emptyset}} \ell(S)^d.
\end{align*}
This latter sum is bounded above by $C \ell(R)^d$ by the Ahlfors regularity of $\cC_R$. This concludes the proof of the lemma.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:upper_beta_est}]
Let $Q_0$ as above and let $R_0$ be the minimal cube in $\Top(Q_0)$ so that $Q_0 \subset R_0$. Then we write 
\begin{align}
    \sum_{\substack{Q \subset Q_0\\ Q \in \cD(k_0)}} \beta_E^{p,d}(C_0Q)^2 \ell(Q)^d & \lesssim \sum_{\substack{R \in \Top \\ R \subset Q_0}} \sum_{\substack{Q \in \Tree(R)\\ Q \in \cD(k_0)}} \beta_{E}^{p,d}(C_0Q)^2\ell(Q)^d \\
    & \enskip \enskip + \sum_{\substack{Q \in \Tree(R_0) \\ Q \subset Q_0 \\ Q\in \cD(k_0)}}  \beta_{E}^{p,d}(C_0 Q)^2\ell(Q)^d =: \Sigma_1 + \Sigma_2.
\end{align}
First, let us look at $\Sigma_2$: by the same argument of Lemma \ref{lemma:betatree}, we see that this sum is bound above by $\ell(Q_0)^d$. On the other hand, by Lemma \ref{lemma:betatree}, we see that 
\begin{align}
    \Sigma_1 \lesssim \sum_{\substack{R \in \Top \\ R \subset Q_0}} \ell(R)^d. 
\end{align}
Note that each $R \in \Top$ is the child of some stopped cube $R'$. Recall we stopped at a surface cube $R' \in \mathcal{D}$ whenever it happened that $R' \cap I$ and $\ell(I) \sim \ell(Q)$ for some $I \in BAD$. We can therefore associate to each $R \in \Top$ a bad dyadic cube $I$, and thus, by \eqref{e:Bads-est}, we have that
\begin{align}
    \sum_{\substack{R \in \Top  \\ R \subset Q_0}} \ell(R)^d \lesssim \sum_{\substack{I \in \Badsh{}\\ I \subset B_{Q_0}}} \ell(I)^d \lesssim \hd(E\cap B_{Q_0}).
\end{align}
The estimate in \eqref{e:Bads-est} is independent of $k_0$, so is the one we obtained here.
All in all, we see that, by lower $d$-regularity, 
\begin{align*}
    \Sigma_1 + \Sigma_2 \lesssim \ell(Q_0)^d + \hd(E \cap B_{Q_0}) \lesssim  \hd(E \cap B_{Q_0}).
\end{align*}

\michele{I think I sorted this out. However, can you actually sum over all dyadic cube in $\Delta$, or just the ones with $\ell(I) \leq 1$? Because if we are summing over all dyadic cubes (and so also the ones with a huge sidelength, we can't really use the trivial bounde $\beta \lesssim 1$. So that's why I used $\Delta_0$, i.e. the family of all dyadic cubes with sidelength from 1 and below.}

This concludes the proof of lemma \ref{lemma:upper_beta_est}.
\end{proof}

\begin{remark} \label{rem:k0}
Note that the estimate in \eqref{e:upper_beta_est} is independent of $k_0$, and therefore holds for all $k_0 \in \mathbb{N}$. Hence we can sum over all cubes $Q \subset Q_0$ and we have the estimate
\begin{align} \label{e:k0}
    \sum_{Q \subset Q_0} \beta_E^{p, d}(C_0 Q)^2 \ell(Q)^d \lesssim C(n,d, C_0) \hd(E \cap B_{Q_0}).
\end{align}
\end{remark}
Let us now conclude the argument and show that \eqref{e:Semmes-beta} holds. 
Fix a ball $B$ centered on $E$, with radius $r_B$. By rescaling and translating, we can assume without loss of generality that the center of the ball is $0$ and that $r_B=1$. Let $Q_0 \in \cD$ be the maximal Christ-David cube so that $Q_0 \subset B(0,1)$ and $\ell(Q_0) \gtrsim 1$. 
We have that
\begin{align} \label{e:dyadic-christ}
    \sum_{\substack{I \in \Delta_0 \\ I \cap E \cap B(0,1) \neq \emptyset }}\beta_E^{p,d} (C_0 I)^2 \ell(I)^d  \lesssim_{n,C_0} 1+  \sum_{Q \subset Q_0} \beta_E^{p,d}(2 C_0 B_Q)^2 \ell(Q)^d;  
\end{align}
indeed, we can split the sum on the left hand side of \eqref{e:dyadic-christ} into two sums, one where we sum over all dyadic cubes which have sidelength larger that $\ell(Q_0)$, and a second one where we sum over dyadic cubes with $\ell(I) < \ell(Q_0)$. The first sum is bounded above by a universal constant depending on $n, d$ and $\rho$ (the parameter in the construction of the Christ-David cubes). 
For the second one, note that for each $I \in \Delta$ such that $I \cap E \neq \emptyset$ and $\ell(I)< \ell(Q_0)$, there exists a cube  $Q \in \cD, Q \subset Q_0$ such that $I \cap Q \neq \emptyset $ and $\ell(Q) \sim \ell(I)$. Therefore it is easy to see that $\beta_E^{p,d}(C_0 I) \lesssim_{n, d, C_0} \beta_E^{p,d}(2C_0 B_Q)$. Moreover, for a fixed $Q \in \mathscr{D}$, the number of dyadic cubes $I$ so that $I \cap Q \neq \emptyset$ and $\ell(I) \sim \ell(Q)$ is bounded above by a universal constant; with this, we obtain \eqref{e:dyadic-christ} and therefore the estimate 
\begin{align}
    \sum_{\substack{I \in \Delta_0 \\ I \cap E \cap B}} \beta_E^{p,d}(C_0 I)^2 \ell(I)^d \lesssimt{\eqref{e:dyadic-christ}, \eqref{e:k0}} 1 + \hd(E \cap B). 
\end{align}
It follows from Theorem I in \cite{AS18} that 
\begin{align}
    \hd(E\cap B) \lesssim 1+\sum_{Q\in \Delta \atop Q\cap E\cap B\neq\emptyset}\beta_{E}^{d,p}(C_0 Q)^{2}\diam(Q)^{d}
\end{align}
All in all, we obtain \eqref{e:Semmes-beta} and therefore the main theorem.

\michele{Note that our trees are only in $\cD(k_{0})$, and so we aren't actually summing the betas over all cubes, so Lemma 5.1 doesn't immediately give 1.9. However, the constants will be independent of $k_0$, and so we need to give an estimate that accounts for this but then send $k_0$ to infinity.}






One can see that a set satisfying Condition B is just a Semmes $d$-surface with $d=n-1$. It is also not hard to show that such sets are lower $d$-content regular. 

\begin{corollary}
Let $E\subseteq \R^{n}$ be a Semmes $d$-surface. Then for any ball $B$ centered on $E$, and $C_0>1$ sufficiently large, 
\begin{equation}
 \cH^{d}(E\cap B) 
\sim_{C_{0},n,c,p} r_B^d+\sum_{\substack{Q\in \Delta \\ Q\cap E\cap B\neq\emptyset}}\beta_{E}^{{d},p}(C_0 Q)^{2}\ell(Q)^{d}
\label{e:Semmes-beta}
\end{equation}
\end{corollary}
\begin{lemma}
Semmes surfaces satisfy \eqref{e:TC}.
\end{lemma}

\begin{lemma}
Reifenberg flat surfaces satisfy \eqref{e:TC}.
\end{lemma}

==> biblio.tex <==
\begin{thebibliography}{20}

\bibitem[AS18]{azzam-schul18}
Azzam~J, Schul~R. An analyst’s traveling salesman theorem for sets of dimension larger than one. Mathematische Annalen. 2018 Apr 1;370(3-4):1389-476.

\bibitem[AV19]{azzam-villa19}
Azzam~J, Villa~M.  Quantitative Comparisons of Multiscale Geometric Properties. arXiv preprint arXiv:1905.00101. 2019 Apr 30.

\bibitem[BJ97]{bishop-jones97}
Bishop CJ, Jones PW. Wiggly sets and limit sets. Arkiv for Matematik. 1997 Oct 1;35(2):201-24.

\bibitem[C90]{christ90}
Christ M. A T(b) Theorem with remarks on analytic capacity and the Cauchy integral. \textit{Colloquium Mathematicum}, 1990.

\bibitem[Dav04]{david04}
David~G. Hausdorff dimension of uniformly non flat sets with topology. Publicacions matematiques. 2004 Jan 1:187-225.
 \bibitem[Dav14]{david14}
 David~G. Approximation of a Reifenberg-flat set by a smooth surface. Bulletin of the Belgian Mathematical Society-Simon Stevin. 2014;21(2):319-38.
 
 
\bibitem[Dav06]{wavelets}
David G. Wavelets and singular integrals on curves and surfaces. Springer; 2006 Nov 14.

\bibitem[Dav88]{Dav88}
G.~David.
\newblock Morceaux de graphes lipschitziens et int\'egrales singuli\`eres sur
  une surface.
\newblock {\em Rev. Mat. Iberoamericana}, 4(1):73--114, 1988.

\bibitem[DS91]{david-semmes91}
David G, Semmes S. Singular integrals and rectifiable sets in $\R^n$: Au-dela des graphes lipschitziens. Soci\'{e}t\'{e} math\'{e}matique de France; 1991.


\bibitem[DS93]{david-semmes93}
David~G, Semmes~S. \textit{Analysis of and on uniformly rectifiable sets}. American Mathematical Soc.; 1993.

\bibitem[DS00]{david-semmes00}
David~G, Semmes~S. Uniform rectifiability and quasiminimizing sets of arbitrary codimension. American Mathematical Soc.; 2000.

\bibitem[DT12]{david-toro12}
David~G, Toro~T. Reifenberg parameterizations for sets with holes. American Mathematical Soc.; 2012.

\bibitem[Fa90]{fang}
Fang~X. The Cauchy Integral of Calder\'{o}n and Analytic Capacity. PhD dissertation
(1990).

\bibitem[GM05]{garnett-marshall}
Garnett~JB, Marshall~DE. \textit{Harmonic measure}. Cambridge University Press; 2005.

\bibitem[H05]{heinonen}
Heinonen~J. \textit{Lectures on Lipschitz analysis}. University of Jyv\"{a}skyl\"{a}; 2005.

\bibitem[HM12]{hm12} 
Hyt\"{o}nen T, Martikainen H. Non-homogeneous Tb theorem and random dyadic cubes on metric measure spaces. \textit{Journal of Geometric Analysis}. 2012 Oct 1;22(4):1071-107.

\bibitem[J90]{jones90}
Jones~P.W. Rectifiable sets and the traveling salesman problem. Inventiones Mathematicae. 1990 Dec 1;102(1):1-5.

\bibitem[J91]{jones91}
Jones~P.W. The traveling salesman problem and harmonic analysis. Publicacions Matemàtiques. 1991 Jan 1;35(1):259-67.

\bibitem[Mat95]{mattila}
Mattila~P. \textit{Geometry of sets and measures in Euclidean spaces: fractals and rectifiability}. Cambridge university press; 1999 Feb 25.

\bibitem[Oki92]{oki92}
Okikiolu~K. Characterization of subsets of rectifiable curves in Rn. Journal of the London Mathematical Society. 1992 Oct 1;2(2):336-48.

\bibitem[S95]{semmes}
Semmes SW. Finding structure in sets with little smoothness. InProceedings of the International Congress of Mathematicians 1995 (pp. 875-885). Birkhauser, Basel.

\bibitem[Sch07]{schul07}
Schul~R. Subsets of rectifiable curves in Hilbert space-the analyst's TSP. Journal d'Analyse Mathematique. 2007 Dec 1;103(1):331-75.

\end{thebibliography}


==> scarto.tex <==

Given a Christ-David cube $Q_0 \in \dD$, set 
\begin{align*}
    \BWGL(Q_0)= \BWGL(Q_0, \ve, \Cc_0) := \{Q \in \dD(Q_0) \, |\, d_{\Cc_0 B_Q}(Q, L) > \ve \quad \mbox{ for all } \quad d\mbox{-planes}\}. 
\end{align*}
Given a cube $R \in \dD \setminus \BWGL(Q_0)$, 
we define tree (or stopping-time region)  $\Tree(R)$ by adding $Q \in \dD(R)$ to $\Tree(R)$ if any of the following conditions hold true:
\begin{enumerate}[leftmargin=0.5cm]
    \item $R = Q$.
    \item A child of $Q$ belongs to $\Tree(R)$.
    \item For any sibling $Q'$ of $Q$ (including $Q$), $\inf_P d_{\Cc_0 B_{Q'}}(P, E) < \ve$, where the infimum in taken over all $d$-planes $P$. 
\end{enumerate}

\noindent
We put
\begin{align*}
    \cP^R := \left\{x_Q \, |\, Q \in \Tree(R)\right\}. 
\end{align*}


%We recur to the same smoothing procedure we used in Lemma \ref{l:corona}. For $Q \in \dD\setminus \BWGL(Q_0)$ and $\Tree(Q)$ as above, and $x \in \R^n$ and $P \in \dD$,
%\begin{align*}
%    & d_Q (x):= \inf_{R \in \Ss(Q)} \left(\ell(R) + \dist(x, R)\right) \quad \mbox{ and} \\
%    & d_Q(P) := \inf_{x \in P} d_Q(x).
%\end{align*}
%We let $C_5>10$ be a possibly large constant  and  $\tau_1>0$ a possibly small one. They both will be fixed later. With these at hand, set  
%\begin{align}
%    & E_0^Q := \{ x \in C_5B_Q \, |\, d_Q(x)= 0\}; \\
%    & U^Q := \bigcup\{ x \in R \, |\, \ell(R)=\ell(Q) \mbox{ and } R \cap C_5 B_Q \cap R \neq \emptyset\};\\
%    & \Ww^Q := \{ R \in \dD(Q_0) \mbox{ and } R \cap U^Q \neq \emptyset \, |\, R \, \, \mbox{ is maximal w.r.t } \, \, \ell(R) < \tau_1 d_Q(R)\}.
%\end{align}
%Finally, we define
%\begin{align}\label{e:wtTree}
 %   \wt{\Tree}(Q) := \{ R \in \dD(Q_0) \mbox{ and } C_5 B_Q \cap R \neq \emptyset \, |\, R \subsetneq S \mbox{ for any } S \in \Ww^Q \}.
%\end{align}
%\noindent
%Recall from Theorem \ref{t:Christ} that any cube $R \in \dD$ has sidelength $\ell(Q) = 5 \lambda^{k (R)}$, where $\lambda>0$ is some small constant (e.g. $1/1000$) and $k(R) \in \N$. 
%For any integer $m$ we choose another integer $k(m)$ so that $5 \lambda^{k(m)} \leq r_m \leq 5 \lambda^{k(m)-1}$, where $r_m=10^{-m}$. We call $m_Q$ the integer for which $5\lambda^{k(m_Q)} \leq r_{m_Q} \leq 5 \lambda^{k(m_Q)-1}$. We might rescale so that $m_Q=0$. With this, we firstly put $\dN_{m_Q}^Q := \{x_Q\}$. Secondly we set\footnote{It might happen that $k(m)= k(m')$ for some $m\neq m'$ but this has no relevance.}
%\begin{align*}
    %\Tree(Q)_m := \dD_{k(m)} \cap \Tree(Q) \mbox{ for any  } m >0,
%\end{align*}
Let $m_0 \in \N$ be such that $\ell(R) \approx_\lambda r_{m_0}= 10^{-m_0}$ (recall that $\lambda$ is a parameter in Theorem \ref{t:Christ}). By re-scaling, we may and will assume that $m_0=0$.   Then for each $m \geq 1$ we construct a maximal $r_m$-separated net\footnote{Given a metric space $(X,d)$ and a $\delta>0$, a $\delta$-separated net $\dN$ is subset of $X$ satisfying $d(x,y) \geq \delta$ for any $x,y \in \dN$. $\dN$ is a \textit{maximal} $\delta$-separated net if for all $z \in X \setminus \dN$, there exists an $x \in \dN$ such that $d(x,z) < \delta$.} for $\cP_R$, 
which we call $\dN^R_m= \{x_{j, m}\}_{j \in J_m^R}$, for some index set $J_m^R$.  

\begin{lemma}\label{l:dt-lemma1}
Keep the notation as above. The collection $\{N_m^R\}_{m=0}^\infty$ satisfies the conditions a), b) and c) of Theorem \ref{t:david-toro}.
\end{lemma}
\begin{proof}
\textbf{Condition a).} There is only one point in $\dN_{0}^R=\{x_j^{0}\}$, namely $x_R$. We associate to $x_R$ the plane $P=:P^0$ such that $d_{\Cc_0 B_R}(E, P) < \ve$. That $x_R \in P^0$ is true by definition of $d_{\Cc B_R} (\cdot, \cdot)$. 

\bigskip



\noindent
\textbf{Condition b).} For each $m \geq 1$ and $j \in J_m^R$ we are required to associate a plane $P=P_j^m$ so that $x_j^m \in P_j^m$. We consider two cases: 1) if we can find a Christ-David cube $Q \in \Tree(R)$ so that  
\begin{align}\label{e:dt-10}
    B_Q \subset B(x_j^m, r_m) \subset \Cc_0 B_Q,
\end{align}
then we set $P_j^m = P_Q'$, where $P_Q'$ is the translation of $P_Q$ and $P_Q$ is a plane so that $d_{\Cc_0 B_Q}(P_Q, E) \approx \inf_P d_{\Cc_0 B_Q}(P, E)$. 2) If no such a cube exists, we find the minimal cube $Q \in \Tree(R)$ so that $B(x_j^m, r_m) \subset \Cc_0 B_Q$ and we put $P_j^m = P_Q'$, where again $P_Q'$ is the translate to $x_j^m$ of $P_Q$. 

\bigskip

\noindent
\textbf{Condition c).} For $m \geq 1$, let $x_j^m \in \dN_m^Q=\{x_j^m\}_{j \in J_m^R}$. We are required to find an $i \in J_{m-1}$ so that $x_j^m \in B(x_{i}^{m-1}, 2r_{m-1})$. Again, we have two cases: 1) if $x_j^m \in \dN_{m-1}^R$, then we are done. 2) If $x_j^m \notin \dN{m-1}^R$, then, by the maximality of $\dN_{m-1}^R$, there exists a point $y \in \dN_{m-1}^R$ so that $|y-x_j^m| < r_{m-1}$, and therefore $x_j^{m} \in B(y, 2r_{m-1})$. 

\end{proof}

\noindent


%\begin{lemma}[\cite{azzam2018analyst}, Lemma 2.11 (eq. 2.28), Lemma 2.14 (eq. 2.32), Lemma 2.16 (eq. 2.36)]
%Let $E \subset \R^n$ be a lower content $(d, \cc_1)$-regular set. Let $B$ be a ball centered on $E$ and $P$ a $d$-plane such that $d_{B}(E, P)< \ve$. Then any ball $B' \subset B$ centered on $E$ and such that $d_{B'}(E, P') < \ve$ for some $d$-plane $P$, we have
%\begin{align*}
  %  d_{B'}(P, P') \lesssim_{d, \cc_1} \ve. 
%\end{align*}
%\end{lemma}



In fact, the above mentioned lemmas from \cite{azzam2018analyst} are more general, but we adapted their statements to our current needs. 
\begin{lemma}
Keep the notation from Lemma \ref{l:dt-lemma1}. 
There exists an absolute constant $C$ (which might depend on $d, \cc_1$) so that condition \eqref{e:DT4} in Theorem \ref{t:david-toro} holds with $\ve' = C \ve$. In particular, choosing a sufficiently small $\ve$ in Subsection \ref{ss:construction-of-Sigma}, we can insure that $\ve' = V\ve < \ve_0$.
\end{lemma}
\begin{proof}
Fix $m, j \in J_m^R$. Let $\ell \in \N$ and $i \in J_\ell^R$ be so that 
\begin{align*}
    |m-\ell|< 2 \quad \mbox{ and } \quad x_j^m \in 100B_i^\ell.
\end{align*}

\end{proof}






\newcommand{\xjm}{x_j^m}







For each $Q \in \cF$, consider a smooth cut off function $\wt \psi_Q$ so that $\1_{\Cc_0/2 B_{Q}} \leq \psi_Q \leq \1_{\Cc_0 B_Q}$. Furthermore, for each $Q$ we put
\begin{align}
    \psi_{Q} = \frac{\wt \psi_Q}{\sum_{S \in \cF} \wt \psi_S}.
\end{align}
The family $\{\psi_Q\}_{Q \in \cF}$ is a partition of unity subordinated to the family of balls $\{\Cc_0 B_Q\}_{Q \in \cF}$. Now, recall that for each $Q \in \cF$, we chose (\eqref{e:dt-caseb}, Case b)) a `zeroth' plane $P_0^Q$ satisfying $d_{\Cc_0B_Q}(E, P_0^Q) < \ve$ (as in \eqref{P_0}). Then for each $Q \in \cF$, we denote by $A_Q$ the affine function $P_0 \to P_0^\perp$ whose graph is $P_0^Q$. Further, recall from Theorem \ref{t:david-toro} (1), and from our construction, that for each $Q \in \cF$, $\Sigma^Q=g(P_0^Q)$, with $g: \R^n \to \R^n$ a H\"{o}lder map. Now set
\begin{align*}
    h_Q= g_Q \circ A_Q: P_0 \to P_0^Q \to \Sigma^Q,
\end{align*}
and finally define, for $p \in P_0$, 
\begin{align*}
    h(p):= \sum_{
    
    
    
    
    
Fix a cube $Q_0 \in \dD$ and a plane $P_0$ which minimises $d_{\Cc_0 B_{Q_0}}(E,P)$. We consider the family $\cF$ of maximal cubes $Q \in \dD(Q_0)$ so that $\inf_P d_{\Cc_0B_Q}(E, P) < \ve$. Then since $\sum_{Q \in \BWGL(Q_0, \ve)} \ell(Q)^d< + \infty$, we must have that 
\begin{align}\label{cheap-cover}
    \bigcup_{Q \in \cF} \Cc_0 B_Q \supset Q_0.
\end{align}
For each $Q \in \cF$, we consider a dyadic cubes $I_Q$ so that $I_Q \subset B_Q \subset 3I_Q$. Set
\begin{align}
    \cI_Q := \{ I \in \Delta \, |\, \ell(I) = \ell(I_Q) \mbox{ and } I \cap \cC_0 B_Q \neq \emptyset\}. 
\end{align}
Finally we put
\begin{align*}
    \Sigma^0:= \bigcup_{Q \in \cF} \bigcup_{I \in \cI_Q} \partial_d I. 
\end{align*}
Note that
\begin{align*}
    \hd(\Sigma^0) \lesssim_{d,n} \sum_{Q \in \cF} \sum_{I \in \cI_Q} \ell(Q)^d \lesssim_{d,n, \Cc_0, \cc_1} \sum_{Q \in \cF} \hd(Q) \lesssim_{d,n, \Cc_0, \cc_1} \hd(Q_0).  
\end{align*}
\begin{lemma}
Let $\Sigma_0$ as defined above. There exists a constant $\gamma_0$ such that the following holds true. For all pairs $(x,r) \in Q_0 \cup \Sigma^0 \times (\ell(Q), \ell(Q_0)]$, we can find a ball $B$ centered on $Q_0 \cup \Sigma^0$, with $B\subset B(x,r)$ and $r_B \geq \gamma_0 r$ such that 
\begin{align}
    \hd(B(x_B, (1-\eta_0)r(B)) \cap \vp_1(E)) \geq \delta_0 r^d.
\end{align}
\end{lemma}
\begin{proof}
Let $Q_* \in \cF$ be a Christ-David cube with minimal sidelength in $\cF$. Choose $\gamma_0>0$ to be the maximal number such that $\ell(Q_*) \geq \gamma_0 \ell(Q_0)$. 

Let $x,r$ as in the statement of the lemma. Suppose first that $x \in Q_0$. Then, using \eqref{cheap-cover}, $x \in \cC_0 B_Q \cap Q_0$ for som
